Intelligent problem-solving as integrated hierarchical reinforcement learning

According to cognitive psychology and related disciplines, the development of complex problem-solving behaviour in biological agents depends on hierarchical cognitive mechanisms. Hierarchical reinforcement learning is a promising computational approach that may eventually yield comparable problem-solving behaviour in artificial agents and robots. However, to date the problem-solving abilities of many human and non-human animals are clearly superior to those of artificial systems. Here, we propose steps to integrate biologically inspired hierarchical mechanisms to enable advanced problem-solving skills in artificial agents. Therefore, we first review the literature in cognitive psychology to highlight the importance of compositional abstraction and predictive processing. Then we relate the gained insights with contemporary hierarchical reinforcement learning methods. Interestingly, our results suggest that all identified cognitive mechanisms have been implemented individually in isolated computational architectures, raising the question of why there exists no single unifying architecture that integrates them. As our final contribution, we address this question by providing an integrative perspective on the computational challenges to develop such a unifying architecture. We expect our results to guide the development of more sophisticated cognitively inspired hierarchical machine learning architectures.

==> abstract.tex <==
\begin{abstract}
According to \rev{cognitive psychology}{R3-\ref{rev:r3:final_edit}} and related disciplines, the development of complex problem-solving behaviour in biological agents depends on hierarchical cognitive mechanisms.
\rev{Hierarchical reinforcement learning is a promising computational approach that may eventually yield comparable problem-solving behaviour in artificial agents and robots. 
However, to date the problem-solving abilities of many human and non-human animals are clearly superior to those of artificial systems.
\rev{Here, we propose steps to integrate biologically inspired hierarchical mechanisms to enable advanced problem-solving skills in artificial agents.}{R3-\ref{rev:r3:clarify_contrib}}
Therefore, we first review the literature in \rev{cognitive psychology}{R3-\ref{rev:r3:final_edit}} to highlight the importance of  compositional abstraction and predictive processing.
Then we relate the gained insights with contemporary hierarchical reinforcement learning methods.
Interestingly, our results suggest that all identified cognitive mechanisms have been implemented individually in isolated computational architectures, raising the question of why there exists no single unifying architecture that integrates them.
As our final contribution, we address this question by providing an integrative perspective on the computational challenges to develop such a unifying architecture.
We expect our results to guide the development of more sophisticated cognitively inspired hierarchical machine learning architectures.}{E-\ref{rev:editor:abstract}}
\end{abstract}

==> all_table.tex <==

% \cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}

\begin{table*}[!ht]
{\sffamily 
% The full Excel table is here: \url{https://1drv.ms/x/s!AkFdeL8LlTTlip9lJdytKEfulJ6wdg?e=Fh2nYr}
  \centering
  \captionsetup{singlelinecheck = false, justification = raggedright}
\caption{Abilities, mechanisms and prerequisites of recent hierarchical reinforcement learning  approaches.}
\vspace{-10pt}
  \scriptsize
\rowcolors{2}{TableRowColor}{TableRowColor}
  \begin{tabular}{R{.14\textwidth}  C{.05\textwidth}  C{.06\textwidth}  C{.08\textwidth}  C{.055\textwidth}  C{.055\textwidth}  C{.08\textwidth}  C{.08\textwidth}  C{.08\textwidth}  C{.08\textwidth} }

\arrayrulecolor{black}            
  \rowcolor{TableRowColor}
            & \multicolumn{3}{ c  }{\scshape \large Abilities} & \multicolumn{4}{ c  }{\scshape \large Mechanisms} & \multicolumn{2}{ c }{\scshape \large Prerequisites} \\

\rowcolor{TableRowColor}
  {\scshape \large Approach} & Few-shot problem-solving & Transfer learning --------------- \begin{minipage}{.06\textwidth} N: near \\ F: far \end{minipage} \newline & Decision-time planning ------------------ \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline &  \multicolumn{2}{ c }
   {
  \begin{minipage}{.13\textwidth} {\centering \vspace{5pt} Sensorimotor abstraction \\ --------------------------- \\} B: basic \\ I: inference-fitted \\ C: compositional \\ \hspace{2pt}  ( actions )~~~~~~~~~ ( states )\end{minipage} 
   } & 
   Intrinsic motivation ------------------- \begin{minipage}{.1\textwidth}C: curiosity \\D: diversity \\SG: subgoals\\[0pt]  \end{minipage} &
   Mental simulation ------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline & 
    \newline Forward model -------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline & 
   Inverse model / policy ------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline \\\hline

\arrayrulecolor{white}

\citetsupp{Akrour2018_RL_StateAbstraction} & - & - & - & I,C & I & - & - & - & H,L\\\hline
\citetsupp{Arulkumaran2016_Classifying_Options_for_Deep_RL} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Bacon2017_OptionCritic} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{barreto2020fast} & (X) & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Beyret2019_DotToDot} & - & - & - & C & - & - & - & - & H,L\\\hline
\citetsupp{Blaes2019_CWYC} & - & - & H & I & - & C, SG & H & H,L & L\\\hline
\citetsupp{Chuck2020_HyPe} & - & - & - & I & - & C & - & - & H,L\\\hline
\citetsupp{Dietterich2000_StateAbstraction_MAXQ} & - & - & - & I & I,C & SG & - & - & H,L\\\hline
\citetsupp{Eppe2019_planning_rl} & - & - & H & I,C & I,C & SG & H & H & L\\\hline
\citetsupp{Eysenbach2019_DiversityFunction} & - & N & - & I & - & D & - & - & H,L\\\hline
\citetsupp{Frans2018_MetaLearningHierarchies} & (X) & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Ghazanfari2020_AssociationRules} & - & - & - & I & I & - & - & - & H,L\\\hline
\citetsupp{Ghosh2019_ActionableRep} & - & - & - & I & I & SG & - & - & H,L\\\hline
\citetsupp{Haarnoja2018_LatentSpacePoliciesHRL} & - & - & - & I & - & SG & - & - & H,L\\\hline
% \citetsupp{Hafez2020_dual-system} &  &  &  &  &  &  &  &  & \\\hline
\citetsupp{Han2020_hierarchicalSelfOrga} & X & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Heess2016_transferModulControl} & X & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Hejna2020_MorphologicalTransfer} & X & F & - & C & - & - & - & - & H,L\\\hline
\citetsupp{jaderberg2019human} & - & N & - & I & I & SG,(D) & - & - & H,L\\\hline
\citetsupp{Jiang2019_HRL_Language_Abstraction}  & X & N & - & I,C & B & - & - & - & H,L\\\hline
\citetsupp{Kulkarni2016_HDQN} & - & - & - & I & I,C & SG & - & - & H,L\\\hline
\citetsupp{Levy2019_Hierarchical} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Li2017_efficient_learning} & - & - & H & I,C & - & - & H,L & H,L & H,L\\\hline
\citetsupp{Li2020_SubPolicy} & X & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Lyu2019_SDRL} & - & - & H & I & I,C & SG & H & H & L\\\hline
\citetsupp{Ma2020_MultiAgentHRL} & - & - & H & I & I & - & H & H & L\\\hline
\citetsupp{Machado2017_PVF_Laplace_OptionDiscovery} & - & - & - & I & I & D & - & - & H,L\\\hline
\citetsupp{Nachum2018_HIRO} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Oh2017_Zero-shotTaskGeneralizationDeepRL} & X & N & - & I,C & I & SG & - & - & H,L\\\hline
\citetsupp{Qiao_2020_HRL-Driving} & - & - & - & I & - & SG & - & - & H,L\\\hline
\citetsupp{Qureshi2020_CompAgnosticPol}	& -	& F& 	-& 	I,C	&-& 	SG,D& 	-& 	-& 	H,L \\\hline
\citetsupp{Rafati2019_model-free_rep_learning} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Rasmussen2017_NeuralHRL} & - & N & - & I,(C) & I & SG & - & - & H,L\\\hline
\citetsupp{Riedmiller2018_SAC-X} & - & - & - & I & - & SG & - & - & H,L\\\hline
\citetsupp{Roeder2020_CHAC} & - & - & - & C & - & C,SG & - & - & H,L\\\hline
\citetsupp{Saxe2017_HRL_Multitask_LMDP} & - & - & - & I,C & - & SG & - & - & H,L\\\hline
\citetsupp{Schaul2013_Better_Generalization_with_Forecasts} & - & - & - & I & I,C & - & - & - & H,L\\\hline
\citetsupp{Shankar2020_MotorPrimitives} & - & - & - & I & - & D & - & - & H,L\\\hline
\citetsupp{Sharma2020_DADS} & X & N & H & I & - & D & H & H & L\\\hline
\citetsupp{silver2016mastering} & - & - & H & I & I & - & H & H & L\\\hline
\citetsupp{Sohn2018_Zero-ShotHRL} & X & N & - & I,C & I & SG & - & - & H,L\\\hline
\citetsupp{sutton2011horde} & - & (N) & - & - & I & - & L & L & L\\\hline
\citetsupp{Tessler2017_LifelongHRLMinecraft} & (X) & N & - & I,C & - & - & - & - & H,L\\\hline
\citetsupp{Vezhnevets2017_Feudal} & - & - & - & I & I & - & - & - & H,L\\\hline
\citetsupp{Vezhnevets2020_OPRE} & - & - & - & I,C & I,C & -  & - & - & H,L\\\hline
\citetsupp{Wu2019_ModelPrimitives}	& -	& N	& -	& I	& -	& -	& L	& L	& H,L \\\hline
\citetsupp{Wulfmeier2020_HierachicalCompositionalPolicies} & - & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Yamamoto2018_RL_Planning} & - & - & H & I,C & - & SG & H & H & L\\\hline
\citetsupp{Yang2018_PEORL} & - & - & H & I & - & SG & H & H & L\\\hline
\citetsupp{Yang2018_HierarchicalControl} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Zhang2020_AdjancentSubgoals} & - & - & - & C & - & SG & - & - & H,L\\\hline
  \end{tabular}
 \normalsize
    \label{tab:hrl_properties}
}
\end{table*}



==> cogShortNew.tex <==
\begin{figure*}[ht!]
    \centering
        \includegraphics[width=\textwidth,trim={0pt 1cm 0pt 0pt},clip]{pics/Figure2.pdf}
    \caption{
    % \rev{\textbf{Prerequisites, mechanisms, and features of biological problem-solving agents.}}{E-\ref{rev:ed:figure_captions}}
    \textbf{Prerequisites, mechanisms, and features of biological problem-solving agents.}
    \emph{Forward-} and \emph{inverse models} are prerequisites for higher-order mechanisms and abilities.
    \emph{Compositional abstractions} allow the agent to decompose a problem into reusable substructures, e.g., by learning which part of an object is easily graspable, such as the stem of a glass.
    \emph{Intrinsic motivation} applied with the help of forward models can drive an agent to interact with its environment in an information-seeking, epistemic way, e.g., by eliciting interactions with the glass to learn more about its properties.
    \emph{Mental simulations} enable the exploration of hypothetical state-action sequences, e.g., by imagining how the hand position will evolve while reaching for the glass.
    %These mechanisms form the foundation for more complex problem solving abilities:
    Given these mechanisms, an agent can flexibly achieve desired goal states via hierarchical, compositional \emph{goal-directed planning}, e.g., planning to drink from the glass by first suitably grasping and then appropriately transporting it.
    Compositional abstractions enable the agent to perform \emph{transfer learning}, e.g., by executing suitable grasps onto other objects with stem-like parts, such as the shown teapot. %i.e., the agent can use its knowledge from one task for a related problem
    In summary, these abilities enable \emph{few-shot problem-solving}.}
    \label{fig:cog_prereq}
\end{figure*}

\section{Neurocognitive foundations}
\label{sec:cognitive_background}
In the following, we propose that the complex problem-solving skills in biological agents can be distinctively characterised by particular cognitive abilities. 
In our perspective, these abilities depend on key cognitive mechanisms, including  abstraction, intrinsic motivation, and mental simulation.
% These mechanisms depend on certain neuro-functional prerequisites.
% \autoref{fig:cog_prereq} shows how complex structures as well as planning and reasoning abilities build upon forward and inverse models. 
% Together, cognitive abilities that we deem crucial for higher level intelligence become enabled, including few-shot problem solving and transfer learning. 
% Here we start with a characterization of these crucial cognitive abilities and then exhibit some of the key mechanisms and prerequisites needed to enable them. 
\autoref{fig:cog_prereq} outlines how these mechanisms may develop from forward and inverse models, as the fundamental neuro-functional prerequisites.
% Together, cognitive abilities that we deem crucial for higher level intelligence become enabled, including few-shot problem solving and transfer learning. 
% We start with a characterization of the crucial cognitive abilities and then exhibit the key mechanisms and prerequisites needed to enable them. 



\subsection{Cognitive abilities}
As distinct cognitive abilities, we focus on the following traits and properties.

\smallskip
\noindent
\textbf{Few-shot problem-solving} is the ability to solve unknown problems with few ($\lessapprox 5$) trials. 
Zero-shot problem-solving is a special case of few-shot problem-solving, where no additional training at all is required to solve a new problem.
% 
% We refer to the ability of solving unknown problems with few trials as few-shot problem-solving. 
% In many cases, agents are able to solve new problems without any trial and error at all (one-shot or zero-shot problem-solving).
% If a problem can be solved ``on sight'', i.e., without any trial and error, we speak about zero-shot or one-shot problem-solving\footnote{We use the terms zero-shot and one-shot problem-solving interchangeably}.
% For simple problems, few-shot problem-solving is trivial. For example, catching a ball is usually a purely reactive behaviour that builds on a direct neural mechanism to map the observation of the flying ball to appropriate motor commands. Such problems are solvable with current computational RL methods\cite{Li2018_DeepRL_Overview}. 
% It involves solving difficult problems that require, e.g., using tools in new contexts. 
For example, a crow can use a stick as a tool for a novel food-access problem without further training (see \autoref{fig:crow_probsolving}), given it has previously solved related problems \cite{Gruber2019_CrowMentalRep}.
%For example, consider the aforementioned problem-solving example of the  crow\cite{Gruber2019_CrowMentalRep} (see \autoref{fig:crow_probsolving}). The crow knows how to use a stick as a tool without any further training, because it has previously solved related problems.
% Here we are interested in the cognitive abilities that enable few-shot problem-solving for such advanced problems. 
We identify two abilities that are most central for such problem-solving, namely transfer learning and decision-time planning (see \autoref{fig:cog_prereq}). 

\smallskip
\noindent
\textbf{Transfer learning}
 allows biological agents to perform few-shot pro\-blem-solving by transferring the solution of a previously solved task to novel, but analogous, unseen tasks \cite{Perkins1992}. This significantly reduces and sometimes eliminates the number of trials to solve a problem. 


Such analogical reasoning is often considered as a critical cornerstone of human cognition.
For example, cognitive theory suggests that humans  understand mechanical systems by using analogous knowledge from other domains\cite{Hegarty2004_MechReasMentalSim}.
And education theory suggests that human transfer learning improves when explicitly trained to identify analogies between different problems\cite{Klauer1989_AnalogyTransfer}.
However, while humans seem skilful in applying analogies for problem-solving, it seems to be more difficult to discover new ones. 
For example, the phenomenon of functional fixedness describes the human problem-solving tendency to use objects only in the way they are traditionally used \cite{Duncker1945}.

\smallskip
\noindent
\textbf{Goal-directed planning.}
Behaviour is traditionally divided into two categories: Stimulus-driven, habitual behaviour and goal-directed, planned behaviour\cite{Dayan2009, Dolan2013, ODoherty:2017}.
Habitual behaviour refers to forms of reflexive control that are strongly automated, computationally efficient, and mainly learned from past reinforcements \cite{Dolan2013}.
% Stimulus-response theories suggest that  most behaviour is learned from past reinforcements \cite{Dolan2013}.
One of the first critics of this approach was Tolman, who showed that rats can find rewards in a maze faster when they have visited the maze before, even if their previous visit had not been rewarded \cite{Tolman1930,Butz:2002c}.
The results suggest that the rats form a representation, or cognitive map, of the maze, which enables them to plan their behaviour once a reward was detected.
Advances in AI and cognitive science have influenced one another to understand goal-directed planning.
An influential model for action control was the TOTE model \cite{Miller:1960}, where actions are selected based on an iterative, hierarchical feedback loop. Herein, a desired anticipated state is compared to the current sensory state to select the next action.
Similar to TOTE, many recent theories view planning as a hierarchical process with different levels of abstraction \cite{Botvinick2014, Tomov2020, Wiener2003}.

But what kind of information is considered while planning?
Ideomotor theories of action generation \cite{Stock2004_Ideomotor} suggest that anticipated action effects determine action selection.
Accordingly, the theory of event coding \cite{Hommel2001} claims that representations of actions and their effects are stored in a common code, whereby action effect anticipations can directly activate corresponding actions \cite{Hommel2001}.
Various experimental evidence supports this link between action generation and effect prediction \cite{Hommel2001, Hoffmann:2003, Kunde:2007}.
Our supplementary \autoref{box:appendix:automatization} describes how the continuous learning of action-effect associations questions the traditional dichotomy between planned and habitual behaviour\cite{Dolan2013}.

\subsection{Cognitive mechanisms for transfer learning and planning}
The previous paragraphs discussed how transfer learning and planning enable intelligent few-shot problem-solving. But what enables transfer learning and planning? 
Our survey suggests three critical mechanisms for transfer learning and planning, namely sensorimotor abstraction, intrinsic motivation, and mental simulation.


\textbf{Sensorimotor abstraction.}
According to theories of embodied cognition, abstract mental concepts are inferred from our bodily-grounded sensorimotor environmental interaction experiences \cite{Barsalou2008_GroundedCognition,Butz2017_MindBeing,Butz2016,Pulvermuller:2010}. 
Herein, we differentiate between \emph{action abstraction} and \emph{state abstraction}.
Action abstractions refer to a temporally extended sequence of primitive actions, sometimes also referred to as options\cite{Sutton1999_options} or movement primitives\cite{Flash2005_AnimalMotorPrimitives, Schaal_2006}.
For example, \emph{transporting an object} is as an action abstraction since it is composed of a sequence of more primitive actions, such as \textit{reaching} and \textit{lifting} (see \autoref{fig:cog_comp}). 

State abstractions refer to reduced encodings of (parts of) the environment, where irrelevant details are abstracted away.
Accordingly, state abstractions may decompose a scene into task-critical aspects, such as graspability, containment, or hollowness.
For example, both \textit{wine glasses} and \textit{tea pots} have the property of being a \textit{container} and being \textit{graspable} (see \autoref{fig:cog_comp}).
Meanwhile, a \textit{container} implies \textit{hollowness}, etc.---illustrating the hierarchical and \textbf{compositional} nature of such abstractions. 
Cognitive linguistics and related fields suggest that abstractions benefit from compositionality \cite{Feldman2009_neural_ECG}. 
Formally, expressions are compositional if they are composed of sub-expressions and rules to determine the semantics of the composition. 
The language of thought theory\cite{Fodor:2001} transfers the compositionality principle from language to abstract mental representations, claiming that thought must also be compositional. 
For example, humans can easily imagine previously unseen images by composing their known constituents from linguistic descriptions \cite{Frankland2020_SearchLoT}, even fantastic ones: think of how a pink dragon riding a skateboard would look like. 

It is still being debated whether the abstract mental representations are encoded as local symbols or by means of distributed encodings \cite{Hummel2011_Symbols_Neural}, but in both cases there is evidence for the existence of combinatorial generalisation.
For example, \citet{Haynes2015_CompositionalNeuroRep} show that the neural codes in the ventrolateral prefrontal cortex, which encode compound behavioural rules, can be decomposed into neural codes that encode their constituents.


For sensorimotor abstractions, the rules of composition need to be flexibly inferred by our minds to form plausible environmental scenarios in accordance with our world knowledge \cite{Butz2016,Gaerdenfors:2014,Lakoff1999}.
Such \emph{common sense compositionality} makes abstractions applicable in meaningful manners. 
The filling in of an abstract component (e.g., the  target of a grasp) is constrained towards applicable objects (e.g., a graspable object such as a teapot), as depicted in \autoref{fig:cog_comp}.
From an algorithmic perspective, common sense compositionality brings enormous computational benefits:
Abstractions, e.g., a grasping-encoding, are more economical if they can be applied in various situations, e.g. for different grasping targets.
Common sense compositionality essentially simplifies the identification of analogies by enabling mappings between representations, an advantage well-known in cognitive theories of creativity and concept blending\cite{Eppe2018_AIJ_Blending,Turner2014} (cf. supplementary \autoref{box:appendix:compositionality-example}).


\begin{figure}
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/Figure3a.pdf}
\hspace{-0.8cm}\begin{minipage}[b][0.3cm][t]{0.3cm}(a.)\end{minipage} 
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/Figure3b.pdf}
\hspace{-0.8cm}\begin{minipage}[b][0.3cm][t]{0.3cm}(b.)\end{minipage} 
\end{minipage}
\hfill
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/Figure3c.pdf}
\hspace{-0.8cm}\begin{minipage}[b][0.3cm][t]{0.3cm}(c.)\end{minipage} 
\end{minipage}
\caption{
\textbf{Compositional action and state abstractions.}
% \rev{\textbf{Compositional action and state abstractions.}}{E \ref{rev:ed:figure_captions}} 
\textbf{a},  \emph{Action abstractions} describe a sequence of more primitive actions. \textbf{b}, \emph{State abstractions} encode certain properties of the state space. \textbf{c}, Their \emph{compositionality} enables their general application, by instantiating abstract definitions (the graspable target of reaching), with a specific object (teapot).}
\label{fig:cog_comp}
\end{figure}


\smallskip
\noindent
\textbf{Intrinsic motivation} affects goal-directed reasoning by setting intrinsically motivated goals.  
From a cognitive development perspective, the term \emph{intrinsic motivation} was coined to describe the ``inherent tendency to seek out novelty, [...] to explore and to learn''\cite{RyanDeci2000}.
Here, \emph{intrinsic} is used in opposition to extrinsic values, which are rather associated with the satisfaction of needs or the avoidance of undesired outcomes \cite{Friston2015}.
Intrinsic motivations induce a general exploratory behaviour, curiosity, and playfulness.
Curiosity refers to information gain-oriented exploratory behaviour\cite{Berlyne1966, Loewenstein1994, Oudeyer2007}.
Curiosity is closely related to playfulness, where novel interactions are tried-out in a skill-improvement-oriented manner. Playfulness can be observed in certain intelligent animal species, such as dogs and corvids\cite{Pisula2008}.

\smallskip

\noindent
\textbf{Mental simulation} describes the ability of an agent to anticipate the dynamics of its environment on various representational levels. 
For example, \emph{motor-imagery} is deemed to enable athletes to improve the execution of challenging body movements (e.g. a backflip) by mentally simulating the movement\cite{Jeannerod1995_MentalImageryMotor}, and engineers can rely on mental simulation when developing mechanical systems \cite{Hegarty2004_MechReasMentalSim}. 
Several researchers suggest that mental simulation also takes place on higher reasoning levels. For example, \citet{Kahnemann1982_MentalSim}, \citet{Wells1989_MentalSimCausality}, and later \citet{Taylor1998_MentalSim} report how mental simulation improves planning of future behaviour on a causal conceptual level. 

\smallskip

\subsection{Forward-inverse models as functional prerequisites}

Sensorimotor abstraction, intrinsic motivation, and mental simulation are complex mechanisms that demand a suitable neuro-functional basis. 
We propose that this essential basis is constituted by forward and inverse models \cite{Stock2004_Ideomotor}. 
Forward models predict how an action affects the world, while inverse models determine the actions that need to be executed to achieve a goal.

\smallskip
\noindent
\textbf{Forward-inverse models for mental simulation.}
To perform mental simulation, an agent needs a forward model to simulate how the dynamics of the environment behave, possibly conditioned on the agent's actions.
However, the prediction of all consequences of all possible actions quickly becomes computationally intractable. 
Hence, action-selection requires more direct mappings from state and desired inner mental state to potential actions. 
This can be accomplished by an inverse model or behaviour policies, which generate candidate actions for accomplishing a current goal.

\smallskip

\noindent
\textbf{Forward-inverse models for intrinsic motivation.}
Forward and inverse models are also needed for intrinsic motivation. 
\rev{For example, the learning progress of internal forward models has been demonstrated to be useful for modeling curiosity as an intrinsic reward signal\cite{Kaplan:2004, Schmidhuber2010, Oudeyer2007}.}{R2-\ref{rev:r2:clarify_pred_errors}}
Friston et al.~propose that intrinsically motivated behaviour emerges when using forward models to apply \emph{active inference}\cite{Friston2011, Friston2015}, i.e., the process of inferring actions to minimise expected free energy.
The authors argue that active inference can lead to epistemic exploration, when an agent acts out different behaviour to reduce the uncertainty about their forward predictions \cite{Friston2015, Oudeyer2018_CompuCuriosityLearning}.
However, active inference and the free energy principle has been criticised as overly general, and its falsifiability has been questioned\cite{Colombo:2018}.

\smallskip
\noindent
\textbf{Forward-inverse models for abstraction and grounding.}
Various cognitive theories, including predictive coding\cite{Huang2011}, the free energy principle\cite{Friston2010}, and the Bayesian brain hypothesis\cite{Knill2004}, have viewed the brain as a generative machine, which constantly attempts to match incoming sensory signals with its probabilistic predictions\cite{Clark2013}.
Within these frameworks, prediction takes place on multiple processing hierarchies that interact bidirectionally:
Top-down information provides additional information to predict sensory signals, while bottom-up error information is used to correct high-level predictions \cite{Clark2016_SurfUncertainty}.
\citet{Butz2016} proposes that this hierarchical processing leads to the emergence of abstract, compositional encodings on higher processing levels, e.g., a container-concept, which enable predictions of lower-level features, e.g., the occlusion and transport of a contained object.
Event segmentation theory (EST)\cite{Zacks2007_EST}  makes the role of forward predictions for learning sensorimotor abstractions even more explicit:
According to EST, transient prediction errors are used to segment the continuous stream of experience into conceptual event-encodings, as detailed in the supplementary \autoref{box:appendix:EST}.








==> conclusionShort.tex <==
\section{Conclusion}
\label{sec:conclusion}
We provide an overview of the cognitive foundations of hierarchical problem-solving and how these are implemented in current hierarchical reinforcement learning architectures.
Herein, we consider few-shot problem-solving as the ultimate ability of intelligent beings that learn to solve causally non-trivial problems with as few trials as possible. 
As our main research question, we ask for the computational prerequisites and mechanisms to enable problem-solving for artificial computational agents on the level of intelligent animals. 
We further pose the challenge to integrate the different mechanisms. 

We appreciate that the cognitive theories we summarise are often contentious and controversial, as indicated in the \nameref{sec:cognitive_background} section. 
However, in our discussion, we show that the particular combination of the described theories have the potential to yield algorithmic synergies. 
% For instance, a forward model is highly synergistic because it enables intrinsic motivation, self-supervised abstraction, decision-time planning and background planning. 
% The abstract concept of a forward model that we describe in this article does not presuppose any hardware constraints. Therefore, the synergies it creates are agnostic to the underlying computational hardware and apply to \emph{in vivo} (biological) as well as to \emph{in silico} (computational) implementations. 
In other words, we reason that if a particular mechanism is useful for computational architectures, then it is likely to be beneficial for biological cognitive systems as well, and vice versa. 
In this way, cognitive sciences and artificial intelligence inspire each other, and they will hopefully converge to insights that are relevant for both fields and useful for the future of AI and humanity.
% Our article does not provide a solution to all problems of hierarchical reinforcement learning, but it provides guidelines and proposals for future research to address major remaining challenges. 

% Our research provides four main contributions. First, we performed a literature survey and a top-down structuring of cognitive abilities, mechanisms, and prerequisites for few-shot problem-solving (see \autoref{fig:cog_prereq}). Second, we reviewed recent hierarchical reinforcement learning architectures to identify whether and how the existing approaches implement the prerequisites, mechanisms, and abilities towards few-shot problem-solving (see \autoref{tab:hrl_properties}).
% Third, we identified four major shortcomings in state-of-the-art computational approaches, based on our review. 
% Fourth, we identified the underlying computational challenges that arise when integrating the cognitive mechanisms, and, as an outlook, we sketched-out proposals to address them.


% Three of these shortcomings are based on the lack of hierarchical forward models, but we also identify a lack of hierarchical reinforcement learning approaches that perform state abstraction, and we reveal a lack of approaches that exploit compositional representations. 
% The development of hierarchical forward models is particularly important because this potentially enables compositional abstraction to address the other gaps in the state of the art.
% In addition, hierarchical forward models are a critical prerequisite also for curiosity-driven intrinsic motivation and mental simulation.

% Nonetheless, we were able to identify several methods that address these gaps in the state of the art in isolation. 
% Not seeing any major reason why these approaches could not be integrated, we suggest that most of the tools to realise higher levels of intelligent behaviour in artificial agents have already been investigated. 
% The key is to combine them effectively. 
% This demonstrates significant potential to develop intelligent agents that can learn to solve problems on the level of intelligent biological agents.



==> glossary_box.tex <==
\begin{infobox}[Glossary]
\label{box:appendix:glossary}

\textbf{Decision-time planning } is a search process over different sequences of potential actions and consequently anticipated changes in the world.
The aim is to determine the best possible sequence of actions and immediate next action to reach a specified goal, to satisfy internal motivational drives, or to maximize a reward or minimize a cost function. 
% , where the agent predicts how the actions change the world. The purpose of decision-time planning is to determine the best possible next action with respect to a specific goal, intention, reward or cost function. 

\noindent \textbf{Background planning} refers to simulating the execution of actions, for the purpose of generating samples for training a behavioural policy. 
In contrast to decision-time planning, background planning does not necessarily happen just-in-time before action execution. It is rather similar to dreaming, in the sense that it simulates action executions to train a behaviour or policy during physically idle times. This reduces the amount of required real-world actions to train a policy, avoids catastrophic forgetting, and fosters selective knowledge consolidation.

\noindent \textbf{Intrinsic motivation}
describes a motivational system that rewards behaviour primarily based on internal goals rather than for some external rewards. 
Here, internal goals refer to all goals that highly depend on subjective, internal representations.
External rewards refer to all rewards found in the environment and are somewhat independent of the subject.
We consider the drive for exploration, curiosity, and playfulness intrinsic motivations. 

% \noindent \textbf{Inference-appropriate state abstraction}
% \noindent \textbf{Inference-fitted state abstraction}
\noindent \textbf{State abstraction}
refers to mapping a lower-level state representation to a higher-level representation.
For instance, high-dimensional raw sensor data are low-level partial state representations, which can be abstracted to high-level discrete symbolic representations\cite{Eppe2019_planning_rl} or low-dimensional continuous vectors produced by convolution and pooling layers in neural networks\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}.

\noindent \textbf{Action abstraction}
refers to the process of generalizing an action representation. 
For example, the index or label of a context-independent behavioural policy or movement primitive (e.g. \concept{grasp(object)} is an abstract action representation because it points to a much more specific low-level action model, namely the actual policy used to execute the context-specific low-level motor-commands. 

\noindent \textbf{Inference-fitted abstraction} is abstraction such that each representational layer is \emph{appropriate for the level of inference} to be performed on that layer. 
For example, many approaches based on convolutional neural networks are not inference-fitted because the same output of the convolution is passed to all hierarchical RL layers. Therefore, all hierarchical RL layers operate on the same preprocessed state representation, and it is unlikely that the representation is the best fit for all levels of inference.
In contrast, utilizing low-level raw sensor data as appropriate state representations for the low-level reinforcement learning layer and propositional symbolic high-level representations to perform high-level inference  with an action planner is inference-fitted: Here, the low-level control relies on low-level data while the high-level inference performs more effectively with high-level representations, which do not contain all the details of the low-level representation. 

\noindent \textbf{Compositional representations} are data structures that consist of sub-data structures that are subject to semantic rules, which specify how the sub-data structures may be combined. For example, this sentence itself is a data structure that consists of words and grammatical constructions, which are sub-data structures. The sentence is compositional because there exist grammatical rules that are necessary to understand the sentence. Another example for a compositional representation is a disentangled vector representation, where the individual slots of the vector represent individual properties (e.g. angle, colour, rotation or shape of an object). In this case, the semantic rules determine the meaning of each individual slot of the vector. 


\noindent \textbf{Mental simulation}
refers to the general ability to anticipate future states of the agent and its environment, where ``states'' can both refer to concrete observations but also to abstract properties of the environment. Note that the temporal reference ``future'' is relative to an assumed starting point in time and independent of the time when the mental simulation is performed. For example, an agent can perform counter-factual mental simulation to anticipate how a past starting state may have had developed differently if the agent had executed a hypothetical course of actions that is different from the actions it actually applied.

\noindent \textbf{Transfer learning}
is a broad term that generally refers to transferring knowledge acquired in a specific context to a new context. 
The term ``transfer'' is partially misleading in the sense that knowledge is usually not transferred between different agents, but rather re-applied in different contexts. Furthermore, transfer learning usually means that learned knowledge is transferred, and not that the transfer is learned. 
In robotic problem-solving, the context is usually a specific problem, and the knowledge is a computational model that provides a solution to it. In RL, the computational model is usually a learned policy, but it can also be a forward model or other data structures. 
For example, consider a policy that has been successfully trained to solve one or more source problems. If the same policy can be re-applied to solve a new unknown target problem the transfer is successful. 
\citet{Perkins1992} propose a distinction between near and far transfer. 
 Near transfer refers to the transfer of skills in similar domains and situations, e.g. using the knowledge from learning to grasp a glass to grasping other objects. Far transfer typically refers to the transfer of solutions between different situations via abstract analogies.

\noindent \textbf{Inductive bias}
refers to a set of assumptions to constrain a learning algorithm. 
% Typically, there are many possible solutions to a problem. With inductive biases, one can incentivize a learning algorithm ``to prioritize one solution (or interpretation) over another'' \cite{Battaglia:2018}. 
% Ideally, inductive biases encode knowledge about the problem and help the algorithm to generalize better to novel data.
Ideally, inductive biases encode general knowledge that is independent of the specific problem so solve, helping the algorithm to generalize better to novel data.
For example, curiosity and other intrinsic motivation models are inductive behavioural biases that potentially improve the data exploration of an agent. 
On the other hand, structural modularizations, convolution, and attention-based information processing, as well as regularization mechanisms are typical inductive learning biases.

\noindent \textbf{Event segmentation}
describes the process of identifying distinct events from a stream of continuous sensorimotor information. Very generally, an event can be any type of segment that is perceived to have a beginning and an end  \cite{Zacks2001_EventStructure}.
Moreover, an event can be typically characterised by distinct interaction dynamics, including particular spatial-relational, force or motor, and entity-respective properties \cite{Butz2016,Butz:2021} (cf. also \autoref{box:appendix:EST}). 

% \noindent \textbf{Epistemic drive}
% refers to the motivational drive of an agent to gain knowledge about itself and its environment. 

\noindent \textbf{Goal-Directed Behaviour}
refers to behaviour, possibly including the direction of attention and thought itself, towards goals. These goals may be activated by motivations, including extrinsic as well as intrinsic motivations, and related epistemic drives.
Goal-directed behaviour thus naturally influences both background planning and decision-time planning, by selectively reflecting on gathered experiences and actively reasoning and planning to solve current tasks respectively

% \noindent \textbf{Zero-shot, one-shot and few-shot problem-solving and learning}
% In machine learning literature, zero-shot learning usually refers to an architecture that can solve a new problem without any new training data.
% One-shot and few-shot learning requires one or only a few new training examples. 
% We adapt this terminology and use the terms zero-shot and few-shot problem-solving to refer to an agent that can solve a new problem without or with only a few any additional training trials. 
 \end{infobox}

==> hrlFinal.tex <==
\section{Computational realisations}
\label{sec:hrlFinal}

Computational hierarchical reinforcement learning (HRL) mechanisms (cf.~\autoref{fig:hrl}) are less integrated than those of biological agents. 
% There are promising developments to potentially overcome the existing limitations, but there are also shortcomings and challenges.
In the following, we summarize the state of the art of computational approaches in relation to the neurocognitive foundations. We provide an additional overview in the supplementary  \autoref{tab:hrl_properties}.

\begin{figure}
    \centering
    %trim={<left> <lower> <right> <upper>}
    %\includegraphics[width=\textwidth,trim={0pt 0pt 0pt 150pt},clip]{pics/HierarchicalArchitecture.pdf}
    \includegraphics[width=\textwidth]{pics/Figure4.pdf} %TODO use Figure_3_smaller.pdf if there is space
    \caption{
    \textbf{General hierarchical problem-solving architecture.}
    % \rev{\textbf{General hierarchical problem-solving architecture.}}{E \ref{rev:ed:figure_captions}} 
    A separate policy $\pi^i$ is used for each layer of abstraction. 
    Most existing computational HRL approaches focus on two layers, where the high-level action $a^1$ is either a behavioural primitive or a subgoal. % (an option or sub-policy), or a subgoal.
    The low-level actions $a^0$ are motor commands that affect the environment directly. }
    \label{fig:hrl}
\end{figure}

\subsection{Transfer learning and planning for few-shot abilities}
\label{sec:hrl:abilities}
Our survey of the neurocognitive foundations indicates that two foundational cognitive abilities for few-shot problem-solving are transfer learning and  planning. But how can we model these abilities computationally? 

\smallskip
\noindent
\textbf{Transfer learning} is natural for hierarchical architectures in the sense that they can potentially re-use general high-level skills and apply them to different low-level use cases, and vice versa. 
Therefore, a significant fraction of the existing transfer learning approaches build on learning re-usable low-level policies \cite{Eysenbach2019_DiversityFunction,Frans2018_MetaLearningHierarchies,Heess2016_transferModulControl,Jiang2019_HRL_Language_Abstraction,Li2020_SubPolicy,Qureshi2020_CompAgnosticPol,Sharma2020_DADS,Tessler2017_LifelongHRLMinecraft,Vezhnevets2016_STRAW}.
% Transfer learning may also involve the transfer of other data structures, such as predictive forward models\cite{Wu2019_ModelPrimitives}.
% \citet{Vezhnevets2016_STRAW} build on the automatic discovery of transferable macro-actions (plans) to solve problems in discrete 2D-environments, while  \citet{Jiang2019_HRL_Language_Abstraction} use natural language action representations to perform near transfer learning.
% \citet{Qureshi2020_CompAgnosticPol} build on re-usable low-level policies for goal-conditioned hierarchical reinforcement learning. 
% The policies are transferable between similar tasks, e.g. different locomotion tasks with the same agent.
Research has not only considered transfer learning between different tasks, but also between different robot and agent morphologies\cite{Devin2017_Transfer_RL,Frans2018_MetaLearningHierarchies,Hejna2020_MorphologicalTransfer}. 
% We classify these approaches as \emph{far} transfer because the entire sensorimotor apparatus changes, which places the agent in a far dissimilar context.
% Furthermore, the methods that feature such cross-morphological transfer also perform far transfer learning across different application domains. 
% \revv{
% For example, \citet{Frans2018_MetaLearningHierarchies} transfer navigation skills acquired in a discrete-space environment to a different continuous-space environment.}{R2-\ref{rev:r2:sugg:trans_learn_para}}
% All aforementioned near and far transfer approaches perform skill transfer implicitly, e.g, by re-using pre-trained policies and value functions, but without explicitly representing and learning the analogies between diferent tasks. 
% An exceptional approach that considers the analogies between representations in different tasks explicitly has been presented \citet{Oh2017_Zero-shotTaskGeneralizationDeepRL}. 
% The authors use vector embeddings to represent the representations. 
% The method has been extended in a later paper\cite{Sohn2018_Zero-ShotHRL}, where the high-level layer is implemented as a neural subtask graph solver that reasons over the preconditions, costs and rewards of subtasks to infer the optimal path over subtasks.

% In summary, the transfer-learning capabilities of hierarchical reinforcement learning methods are 
\smallskip
\noindent
\textbf{Planning} can be categorised into \emph{decision-time planning} and \emph{background planning}\cite{Hamrick2021_MBRL,Sutton:2018}. 
Decision-time planning refers to a search over sequences of actions to decide which action to perform next to achieve a specific goal.
The search is realised by simulating the actions with an internal predictive model of the domain dynamics.  
Decision-time planning enables zero-shot problem-solving because the agent only executes the planned actions if an internal prediction model verifies that the actions are successful.
Background planning refers to model-based reinforcement learning as introduced by \citet{Sutton1990_Dyna}. It is used to train a policy by simulating actions with a forward model.
This can improve the sampling efficiency, but not to the extent that it enables few-shot problem-solving.

Hierarchical decision-time planning is a well-known paradigm in classical artificial intelligence\cite{Nau2003_SHOP2}, but approaches that integrate it with hierarchical reinforcement learning are rare. 
Some approaches integrate action planning with reinforcement learning by using an action planner for high-level decision-making and a reinforcement learner for low-level motor control\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS}. 
% For example, \citet{Eppe2019_planning_rl} focus on integrating the discrete-space high-level representations for planning with continuous-space low-level representations for motor control. \citet{Ma2020_MultiAgentHRL} focus on multi-agent systems.
These approaches underpin that decision-time planning is especially useful for high-level inference in discrete state-action spaces. 
% However, we are aware of only one recent approach\cite{Botvinick2009_HierarchicalCognitionRL} that exploits predictive models for planning on both the high-level and low-level layer.
% % \footnote{Some approaches use the word ``planning'' to refer to a method that is different from the kind of planning that we consider here.} 
% The authors refer to this architecture as \emph{saltatory} model-based reinforcement learning with planning and they empirically demonstrate significant performance gains with their approach. 
% Additional still unexplored potential synergies become apparent when considering that action planning usually suffers from complexity issues due to the combinatorial explosion of possible state transitions. 
% A reinforcement learning policy can serve as a heuristics to propose candidate plans for a planner, so that the planner does not need to traverse the full search space.


% They either realize one-shot problem-solving by performing a very close transfer between similar problems within the same domain\cite{}, or they only support overly simplistic discrete-space environments\cite{}. 

\subsection{Mechanisms behind transfer learning and planning}
\label{sec:hrl:mechanisms}
Our summary of the cognitive principles behind transfer learning and planning reveals three important mechanisms that are critical for the learning and problem-solving abilities of biological agents, namely compositional sensorimotor abstraction, intrinsic motivation, and mental simulation.

\smallskip
\noindent
\textbf{Compositional sensorimotor abstraction and grounding.}
Hierarchical reinforcement learning (HRL) has a temporal and a representational dimension, and one can distinguish between action and state abstraction. 
The temporal abstraction of actions breaks down complex problems into a hierarchy of simpler problems. 
% The temporal dimension is an innate property of HRL because by definition it beaks down each high-level action or behaviour into low-level actions or behaviours. 
% The representational dimension is less clearly defined. 
% Another dimension of abstraction is representational abstraction. 
% However, temporal abstraction is not the only dimension of abstraction that helps to simplify problems. 
% Here, we are interested in a less investigated form of abstractions, namely representational abstraction. 
% Hierarchical reinforcement learning approaches also involve representational action abstraction. 
% One can distinguish the existing approaches into two different types of representational action abstraction.
The probably most influential method for representational action abstraction builds on behaviour primitives
% \cite{Bacon2017_OptionCritic,Dietterich2000_StateAbstraction_MAXQ,Frans2018_MetaLearningHierarchies,Kulkarni2016_HDQN,Li2020_SubPolicy,Li2017_efficient_learning,Ma2020_MultiAgentHRL,Machado2017_PVF_Laplace_OptionDiscovery,Qiao_2020_HRL-Driving,Shankar2020_MotorPrimitives,Sharma2020_DADS,Tessler2017_LifelongHRLMinecraft,Vezhnevets2020_OPRE}%
\cite{Bacon2017_OptionCritic,Dietterich2000_StateAbstraction_MAXQ,Frans2018_MetaLearningHierarchies,Kulkarni2016_HDQN,Li2020_SubPolicy,Shankar2020_MotorPrimitives,Sharma2020_DADS,Vezhnevets2020_OPRE}
, including options\cite{Sutton1999_options}, sub-policies, or atomic high-level skills.
Such behaviour primitives are represented in an abstract representational space, e.g. in a discrete finite space of action labels or indices (see \autoref{fig:options_behaviour_primitives}, a.). 
A more recent type of high-level action representations are subgoals in the low-level state-space \cite{Eppe2019_planning_rl,Ghazanfari2020_AssociationRules,Hejna2020_MorphologicalTransfer,Levy2019_Hierarchical,Nachum2018_HIRO,Rafati2019_model-free_rep_learning,Roeder2020_CHAC,Zhang2020_AdjancentSubgoals} (see \autoref{fig:options_behaviour_primitives}, b.).
Here, the agent achieves the final goal by following a sequence of subgoals.
Our supplementary \autoref{tab:hrl_properties} shows that  there is considerably less contemporary research on state abstraction than on action abstraction. 

\begin{figure}
    \centering
    %trim={<left> <lower> <right> <upper>}
    \includegraphics[width=.99\linewidth,trim={1.5cm 0cm 1.5cm 0.0cm},clip]{pics/Figure5.pdf}
    {\sf \footnotesize ~~~~~~~ (a.)    Behaviour primitives  ~~~~~~~~~~~~ (b.) Subgoals ~~~~~~~~~~~~ }
    \caption{
    % \rev{\textbf{Types of action abstractions.}}{E \ref{rev:ed:figure_captions}} %
    \textbf{Types of action abstractions.}
    \textbf{a}, With behaviour primitives, the agent determines the path to the final goal by selecting a sequence of high-level actions, but without specifying explicitly to which intermediate state each action leads. 
    \textbf{b}, With subgoals, the agent determines the intermediate states as subgoals that lead to the final goal, but without specifying the actions to achieve the subgoals.}
    \label{fig:options_behaviour_primitives}
\end{figure}
%



Many current reinforcement learning approaches based on visual input use convolutional neural networks to perform a rather generic form of  abstraction, where all hierarchical layers use the same abstract visual feature map\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}. 
A problem is that this does not appreciate that \emph{different levels of inference require different levels of abstraction}: For example,  for a transport task, the exact shape and weight of an object is only relevant for the low-level motor control. A high-level planning layer only requires abstract facts, such as whether the object is graspable or transportable.
Therefore, the representational state abstraction should fit the level of inference it is used for. We refer to such abstraction as \textbf{inference-fitted abstraction}. 
%
% Therefore, we consider only those approaches as representational abstraction methods that involve layer-wise abstraction. 
Inference-fitted abstraction has been tackled in existing HRL approaches, but many of them rely on manually defined abstraction functions\cite{Eppe2019_planning_rl,Kulkarni2016_HDQN,Ma2020_MultiAgentHRL,Toussaint2018}.
There exist only a few exceptions where state abstractions are derived automatically in hierarchical reinforcement learning%
% \cite{Ghosh2019_ActionableRep,Vezhnevets2017_Feudal,Vezhnevets2020_OPRE}
, e.g. through  clustering\cite{Akrour2018_RL_StateAbstraction,Ghazanfari2020_AssociationRules}, with feature representations\cite{Schaul2013_Better_Generalization_with_Forecasts}, or by factorisation \cite{Vezhnevets2020_OPRE}.
% Interestingly, non-hierarchical model-based reinforcement learning offers promising alternative prediction-based methods for state abstraction \cite{Hafner2020_Dreamer,Pathak2019_ICML_SelfSuperExploreDisa}, which show parallels to cognitive prediction-based abstraction theories. 
% However, these have not yet been applied in a hierarchical architecture. 

Cognitive science also suggests that \emph{compositionality} is an important property of abstract representations. 
For instance, a symbolic compositional action representation \concept{grasp(glass)} allows for modulating the action \emph{grasp} with the object \emph{glass}.
% In terms of reinforcement learning, compositionality implies that the meaning of a compositional action representation is determined by multiple constituent expressions and a set of rules to combine them. 
% For example, consider an action representation \concept{grasp(glass)}. 
% The expression consists of several sub-expression and symbols, i.e., an action type symbol (``\concept{grasp}'') a semantic patient symbol (``\concept{glass}''), and delimiter symbols (``('',``)''). There exist syntactic rules that determine that the semantic patient of the action is described by the expression within the delimiters and the action type is determined by the expression before the opening delimiter. Hence, the expression \concept{grasp(glass)} is \emph{syntactically compositional}. 
% This syntactic compositionality has the advantage that less atomic symbols are necessary to represent all possible combinations of action types and objects than the number of symbols that would be required if each composed action would be represented by one non-compositional atomic expression like \concept{``graspGlass''}). 
% For example, given $n_a=4$ action types \concept{``grasp'', ``push'', ``move'', ``release''}) and $n_o=4$ object types \concept{``glass'', ``cup'', ``tea pot'', ``spoon''}, the total number of symbols for compositional representations (e.g. \concept{grasp(glass)}) is $n_a + n_o = 8$, whereas the total number of symbols for non-compositional representations (e.g. \concept{graspGlass} is an atomic symbol) is $n_o \cdot n_a = 16$. 
% Similar advantages hold for compositional state representations (e.g. \concept{leftOf(cup,tea pot)}). 
Compositionality is also applicable to distributed numerical expressions, such as vector representations. For example, a vector $v_1$ is a compositional representation if it is composed of other vectors, e.g., $v_2$ and $v_3$, and if there is a vector operation $\circ$ that implements interpretation rules, e.g., $v_1 = v_2 \circ v_3$. 

There is significant cognitive evidence that compositionality improves transfer learning\cite{Colas2020_LanguageGroundingRL}. 
This evidence is computationally plausible when considering that transfer learning relies on exploiting analogies between problems, as described in the supplementary \autoref{box:appendix:compositionality-example}
% This lower number of possible analogy mappings of compositional representations implies better transferability. This has not yet been investigated empirically in reinforcement learning, but 
Other cognitively inspired computational methods, such as concept blending\cite{Eppe2018_AIJ_Blending}, provide further evidence that a lower number of possible analogy mappings improves transferability.
% , where two or more compositional concept representations are transferred into a new representation. 
% \begin{figure}
%     \centering
%     \includegraphics{pics/compTransfer.pdf}
%     \caption{Compositional representations improve transfer learning}
%     \label{fig:compTransfer}
% \end{figure}
Furthermore, the work by \citet{Jiang2019_HRL_Language_Abstraction} provides empirical evidence that compositional representations improve learning transfer. The authors use natural language as an inherently compositional representation to describe high-level actions in hierarchical reinforcement learning, and show that this natural language representation improves transfer learning performance compared to non-compositional representations.
%
% Few other researchers use compositional representations in hierarchical reinforcement learning. \citet{Saxe2017_HRL_Multitask_LMDP} compose high-level actions from concurrent linearly solvable Markov decision processes (LMDPs) to guarantee optimal compositionality. Their method successfully executes compositional policies that it has never executed before, effectively performing zero-shot problem-solving.
% Zero-shot problem-solving has also been demonstrated in other related articles that feature compositional action representations\cite{Isele2016_FeatureZeroShotTransfer,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}, but these works do not draw an explicit link between compositionality and zero-shot problem-solving.
% A few symbolic compositional state representations exist in hierarchical decision-making methods, but these rely on manually defined abstraction functions\cite{Eppe2019_planning_rl,Kulkarni2016_HDQN,Lyu2019_SDRL,Toussaint2018} or they are very general and feature compositionality only as an optional property\cite{Rasmussen2017_NeuralHRL}.
%

% There also exist hierarchical reinforcement learning approaches where sub-symbolic compositional representations are learned\cite{Devin2017_Transfer_RL,Qureshi2020_CompAgnosticPol,Schaul2013_Better_Generalization_with_Forecasts,Vezhnevets2020_OPRE}. 
% The compositionality of these representations is rather implicit and, with one exception \cite{Qureshi2020_CompAgnosticPol}, has not been investigated in the context of transfer learning. The exceptional approach by \citet{Qureshi2020_CompAgnosticPol} considers composable low-level policies and shows that compositionality significantly improves transfer between similar environments. 


\smallskip
\noindent
\textbf{Intrinsic motivation}
is a useful method to stabilise reinforcement learning by supplementing sparse extrinsic rewards with additional  domain-independent intrinsic rewards. 
% Intrinsic motivation is also commonly used to incentivize exploration.  
% Reinforcement learning typically models intrinsic motivation through intrinsic rewards. 
The most common method of HRL with intrinsic motivation is to provide intrinsic rewards when subgoals or subtasks are achieved%
% \cite{Blaes2019_CWYC, Cabi2017_intentionalunintentional,Eppe2019_planning_rl,Haarnoja2018_LatentSpacePoliciesHRL,Jaderberg2017_unreal,Kulkarni2016_HDQN,Lyu2019_SDRL,Oh2017_Zero-shotTaskGeneralizationDeepRL,Qureshi2020_CompAgnosticPol,Rasmussen2017_NeuralHRL,Riedmiller2018_SAC-X,Roeder2020_CHAC,Saxe2017_HRL_Multitask_LMDP,Sohn2018_Zero-ShotHRL,Yamamoto2018_RL_Planning,Yang2018_PEORL}.
\cite{Blaes2019_CWYC,Eppe2019_planning_rl,Haarnoja2018_LatentSpacePoliciesHRL,Kulkarni2016_HDQN,Lyu2019_SDRL,Oh2017_Zero-shotTaskGeneralizationDeepRL,Qureshi2020_CompAgnosticPol,Rasmussen2017_NeuralHRL,Riedmiller2018_SAC-X,Yang2018_PEORL}.

% }$^,$~ \cite{
Other approaches provide intrinsic motivation to identify a collection of behavioural primitives with a high diversity\cite{Blaes2019_CWYC, Eysenbach2019_DiversityFunction,Machado2017_PVF_Laplace_OptionDiscovery} and predictability\cite{Sharma2020_DADS}. 
This includes also the identification of primitives suitable for re-composing high-level tasks\cite{Shankar2020_MotorPrimitives}.

Another prominent intrinsic reward model that is commonly used in non-hierarchical reinforcement learning is based on surprise and curiosity\cite{Oudeyer2007,Pathak2017_forward_model_intrinsic,Schillaci2020_IntrinsicMotivation,Schmidhuber2010}. 
In these approaches, surprise is often modelled as a function of the prediction error of a forward model, and curiosity is realised by providing intrinsic rewards if the agent is surprised.
However, only \citet{Blaes2019_CWYC}, \citet{Colas2019_CURIOUS}, and \citet{Roeder2020_CHAC} use surprise in a hierarchical setting, showing that hierarchical curiosity leads to a significant improvement of the learning performance.
Hierarchical curiosity provides potential synergies because a curious high-level layer automatically acts as a curriculum generator for a low-level layer. For example, it can generate ``Goldilocks'' subgoals that are neither too hard nor too easy to achieve for the low-level layer. 
The difficulty is to identify these Goldilocks conditions and to find an appropriate balance between explorative and exploitative subgoals.

%Both approaches train a high-level layer to determine explorative subgoals in hierarchical reinforcement learning. 
% These approaches train a high-level layer to determine explorative subgoals in hierarchical reinforcement learning.
% In addition, \citet{Roeder2020_CHAC} also use surprise to supplement sparse reward for the low-level layer, and they show that hierarchical curiosity leads to a significant improvement of the learning performance.
% An alternative method to model curiosity is to perform hypothesis-testing for option discovery\cite{Chuck2020_HyPe}.

\smallskip
\noindent
\textbf{Mental simulation} enables an agent to anticipate the effects of its own and other actions. Therefore, it is a core mechanism to equip an intelligent agent with the ability to plan ahead. Computational approaches for mental simulation involve model-based reinforcement learning\cite{Sutton1990_Dyna}, action planning\cite{Nau2003_SHOP2}, or a combination of both \cite{Eppe2019_planning_rl,Hafez2020_dual-system}. 
However, even though there is cognitive evidence that mental simulation happens on multiple representational layers\cite{Butz2017_MindBeing,Frankland2020_SearchLoT}, there is a lack of approaches that use hierarchical mental simulation. 
Only a few hierarchical approaches that integrate planning with reinforcement learning build on mental simulation\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS,Yamamoto2018_RL_Planning,Yang2018_PEORL}, though the mental simulation mechanisms of these models are only implemented on the high-level planning layer. 
An exception is the work by \citet{Wu2019_ModelPrimitives}, who use mental simulation on the low-level layer to determine the sub-policies to be executed. 
Another exception is presented by \citet{Li2017_efficient_learning}, who perform mental simulation for planning on multiple task layers. 
However, we are not aware of any approach that performs hierarchical background planning, i.e., that trains a hierarchical policy by mentally simulating the action execution on multiple levels.
One possible reason for this lack is that high-level background planning requires stable low-level representations, and it is difficult to model a respective stability criterion.

% There exist several non-hierarchical model-based reinforcement learning methods\cite{Ha2018_WorldModels,Hafner2020_Dreamer,Sutton1990_Dyna} that perform background planning, i.e., the policy is trained by mentally simulating action execution instead of executing the actions in the real world.

% (e.g.\cite{Sutton1990_Dyna}).

\subsection{Prerequisites for sensorimotor abstraction, intrinsic motivation, and mental simulation}
Reinforcement learning builds on policies or inverse models that predict the actions to be executed in the current state to maximise reward or to achieve a goal state.
% Some approaches learn the policy directly, and others learn a value function that determines the policy. 
In contrast, a forward model predicts a future world state based on the current state and a course of actions. 
% Both kinds of models are critical prerequisites for compositional abstraction, intrinsic motivation, and mental simulation.
Our review shows that the vast majority of hierarchical reinforcement learning methods use inverse models for both the high-level and low-level layers. 
Some approaches exist that use an inverse model only for the low-level layer\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS,Yamamoto2018_RL_Planning,Yang2018_PEORL} and use decision-time planning to perform high-level decision-making.
Our review also implies that a forward model is required for several additional mechanisms that are necessary or at least highly beneficial for transfer learning, planning, and few-shot problem-solving. 
Some non-hierarchical approaches use a forward model to perform sensorimotor abstraction\cite{Hafner2020_Dreamer,Pathak2017_forward_model_intrinsic}. They achieve this with a self-supervised process, where forward predictions are learned in a latent abstract space. 
However, we are not aware of any hierarchical method that exploits this mechanism. 

A forward model is also useful to model curiosity as an intrinsic motivation mechanism, for example, by rewarding an agent for being surprised, where surprise is a function of the prediction error \cite{Friston2011}. 
% To perform these predictions, a forward model is required.
Curiosity has been demonstrated to alleviate the sparse rewards problem in reinforcement learning\cite{Pathak2017_forward_model_intrinsic,Roeder2020_CHAC}, but with few exceptions\cite{Colas2019_CURIOUS,Roeder2020_CHAC}, there is a lack of approaches that use a hierarchical forward model for generating hierarchical curiosity. 
% The third and most obvious application of a forward model is mental simulation. To simulate the effects of actions, be it for planning or motor imagery, agents must learn a forward model. 

% However, a well-known problem for mental simulation is the model bias\cite{Lesort2020_ContLearnRobo}. 
% A forward model that emulates the dynamics of a real environment is always biased and each predicted state-transition inheres an error.
% Predicting the outcome of a  sequence of actions involves the recursive computation of several state transitions. The error propagates further with each recursion, leading to imprecise mental simulation.
% To address this problem, recent non-hierarchical model-based reinforcement learning methods use Gaussian models that predict also the uncertainty of their predictions\cite{Kupcsik2017}. 
% However, the approach has not yet been applied in a hierarchical reinforcement learning architecture. 





==> intro.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=.19\columnwidth]{pics/Figure1a.pdf}
    \hspace{-0.7cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{(a.)}\end{minipage} 
    \hspace{0.3cm}
    \includegraphics[width=.19\columnwidth]{pics/Figure1b.pdf}
    \hspace{-0.7cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{(b.)}\end{minipage} 
    \hspace{0.3cm}
    \includegraphics[width=.19\columnwidth]{pics/Figure1c.pdf}
    \hspace{-0.7cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{(c.)}\end{minipage} 
    \hspace{0.3cm}
    \includegraphics[width=.19\columnwidth]{pics/Figure1d.pdf}
    \hspace{-0.7cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{(d.)}\end{minipage} 
    \hspace{0.3cm}
    \includegraphics[width=.19\columnwidth]{pics/Figure1e.pdf}
    \hspace{-0.7cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{(e.)}\end{minipage} 
    \hspace{0.3cm}
    \vspace{-10pt}

    \caption{
    % \rev{\textbf{A New Caledonian crow solves a food-access problem.}}{E- \ref{rev:ed:figure_captions}}
    \textbf{A New Caledonian crow solves a food-access problem.}
    % \rev{d}{E-\ref{rev:ed:figure_captions}}
    \textbf{a}, First, the crow picks up a stick. \textbf{b-c}, Then it uses the stick to pull a stone out of a tube. \textbf{d-e,} Finally, it uses the stone to activate a mechanism that releases food. 
    Although the crow has never solved this problem setup before, it is able to solve it instantly after a brief inspection phase.
    % , suggesting that the crow develops memorized abstract mental representations to plan ahead. 
    % \rev{
    Such zero-shot problem-solving is a prime example for \emph{hierarchical, goal-directed planning} that involves mental simulations and relies on a task-suitable, \emph{compositional abstractions}.
    % These mechanisms involve mental simulation, transfer learning, and representational abstraction.
    The authors reason that the crow \emph{plans ahead} because it can only see one side of the cubic setup at a time.\cite{Gruber2019_CrowMentalRep} 
    Hence, the crow must \emph{mentally simulate} the future steps. 
    There is also \emph{transfer learning} involved: previously learned solutions to similar sub-problems are transferred and combined to solve the new problem. 
    Successful planning and transfer learning can only be expected to occur once \emph{abstract compositional mental representations} have developed, which, for example, may encode tool manipulation options. %the abstract manipulation options afforded by the available tools. 
    % The crow is motivated to solve the problem because food is involved. However, it 
    % The crow has learned the affordances of the tools previously, when it learned to solve the individual sub-stages.
    %To learn tool affordances and compositional representations,
    To learn different tool manipulations, however, the crow relies on its \emph{intrinsic motivation} to acquire knowledge by playing and experimenting with the tools. 
    % A related study\cite{Kenward2011_tools_crows} concludes that ``heritable action patterns do not provide a complete explanation'' for the problem-solving abilities or crows, suggesting that ``crows are more inclined to object-combination play''.
    The images are used with permission by R. Gruber and co-authors\cite{Gruber2019_CrowMentalRep}.
    }.
    % }{R1-\ref{rev:r1:example}}
    \label{fig:crow_probsolving}
\end{figure*}

Humans and several other intelligent animal species have the ability to break down complex problems into simpler, previously learned sub-problems. This hierarchical approach allows them to solve previously unseen problems in a zero-shot manner, i.e., without any trial and error. 
For example, \autoref{fig:crow_probsolving} depicts how a crow solves a non-trivial food-access puzzle that consists of three causal steps: It first picks a stick, then uses the stick to access a stone, and then uses the stone to activate a mechanism that releases food \cite{Gruber2019_CrowMentalRep}. 
There exist numerous analogous experiments that attest similar capabilities to primates, octopuses, and, of course,  humans \cite{Butz2017_MindBeing,Perkins1992}.
Human and animal cognition research suggests that hierarchical learning and problem-solving is critical to develop such skills \cite{Botvinick2009_HierarchicalCognitionRL,Butz2017_MindBeing,Tomov2020}. 
This raises the question of how we can equip intelligent artificial agents and robots with similar hierarchical learning and zero-shot problem-solving abilities.

We address this question from the perspective of reinforcement learning (RL) \cite{Arulkumaran2017_DeepRL,Li2018_DeepRL_Overview,Sutton:2018}. 
Several studies suggest that RL is biologically and cognitively plausible \cite{Neftci2019_RL_BioArtificial_NatureMI,Sutton:2018}. Many existing RL-based methods are aiming at zero-shot problem-solving and transfer learning, but this is currently only possible for minor variations of the same or a similar task \cite{Eppe2019_planning_rl} or in simple synthetic domains, such as 2D grid worlds \cite{Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}.
A continuous-space problem-solving behaviour that is comparable with the crow's behaviour of \autoref{fig:crow_probsolving} has not yet been accomplished with any artificial system.
We suggest that the focus on hierarchical learning and problem-solving is largely missing, seeing 
that research in hierarchical reinforcement learning (HRL) is underrepresented, as suggested by our meta review in \autoref{box:appendix:meta_RL-survey} of the supplementary material.

In this article, we address this gap in three steps: First, we evaluate the neurocognitive foundations of hierarchical decision-making and identify important mechanisms that enable advanced problem-solving skills. 
Second, we reveal an integration problem of contemporary hierarchical RL methods: We show that the biological mechanisms have mostly been implemented already---but only in isolation and not in an integrative manner. 
Third, we suggest steps towards combining key methods and mechanisms to overcome the integration challenge for the development of a unifying cognitive architecture.





==> misc_old/notes_snippets_manfred.tex <==

% This implies that different intelligent species would conceptualize the world in different ways, ultimately leading to different languages and different self-representations. 
% The theory states that there exist so-called basic concepts that are directly linked to the body. 
% As an example for a basic concept, consider the concept \concept{front}, which is determined by the direction in which we usually move and where most sensory organs are directed to. 
% Other more abstract concepts are hierarchically grounded in basic concepts. 
% For example, consider abstract mathematical concepts, where the front determines the geometric angle of $0^{\circ}$.

\citet{Shapiro2019_EmbodiedCognition} takes a weaker perspective, stating that also agents with different bodies can have shared mental concepts. The grounding of the concepts, however, may be different. He states that even an imaginative spherical being that is capable of omnidirectional movement and sensing in a gravitation-free environment can have a concept for \concept{front} if other objects or agents in its environment have a distinctive side that has certain front-typical features, such as eyes. However, for the spherical being, the \concept{front} concept is not a basic one because it is not directly linked to its body schema. 

Hence, the body schema has a strong influence on higher cognitive functions because it directly influences how we think. 
This becomes evident in natural language, where metaphorical expression involve basic body-related concepts \cite{Eppe2016_GCAI_SemanticParsing,Trott2016}. 
As an example, consider the metaphor \concept{up} \emph{is} \concept{more}. An agent that lives in a gravitation-free environment would not be able to understand a sentence like ``The stock market goes up''.


As an additional example of how body schemas influence our high-level cognitive operations consider recent work on \emph{concept blending} \cite{Eppe2018_AIJ_Blending,Confalonieri2016b,Confalonieri2015}. One pillar of human creativity is the capability of inventing new concepts by means of a serendipitous combinations of known concepts \cite{Fauconnier2002}. This concept blending process strongly depends on body-driven conceptualizations of the world. We conclude that, therefore, creative thought is also a result of the active self. 

What remains open, though, is how we can model grounding of sensorimotor concepts computationally. Several approaches,  including the Theory of Event-Coding \cite{Hommel2015_TEC}, and Event Segmentation Theory \cite{Zacks2007EventPerspective,Gumbsch2019AutonomousPrimitives}, exist. However it is subject to future work to fully integrate these approaches within a unifying computational theory of high-level cognition. Research on the minimal active self fosters the development of such a unifying theory because it allows one to investigate how basic body-related concepts emerge from sensorimotor interaction. 


\subsection{Representational state abstraction}
Cognitive scientists often model abstract mental concepts, such as \emph{path} of \emph{container} in terms of role-filler-based embodied semantic representations, such as semantic frames \cite{Barsalou1992} or image schemas \cite{Lakoff1988,Feldman2009_neural_ECG}. 
For example, a \concept{path} schema has a role \concept{trajector} which is typically filled by an object or agent that moves along the path, and it has roles for \concept{start} and \concept{end}. In our previous work on human-robot dialog, we build on image schemas to perform semantic parsing \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, and show how embodied action-related representations facilitate semantic compositionality for human-robot interaction. 

Role-filler based representations are compatible with action-related semantic representations used in Artificial Intelligence. For example, in action planning, actions are commonly represented by sets of pre- and postconditions (cf. our previous work on action theory \cite{Eppe2015_JAL,Eppe2015_JAL_ASP}): a \concept{move-object} action has the precondition that the agent that moves the object must hold the object, and it has the postcondition that the object is at the target location. In our previous work \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, we have used semantic action templates that link this pre- and postcondition perspective with the role-filler semantics of a semantic language parsing process. 
For example, the \concept{move-object} action inherits structure from the compositional \concept{path} concept: the object to move fills the \concept{trajector} role of the concept, the current object location fills that \concept{start} role and the target location fills the \concept{end} role. 

% , the current object location fills that \concept{start} role, and the target location the \concept{end} role. 

The Neurocognitive and Psychological theories of event coding \cite{Hommel2015_TEC} and ideomotor theory \cite{Stock2004} are in-line with the AI-based pre- and postcondition perspective on actions, as they consider associations between actions and effects at their core. 
However, these and other related theories do not provide a clear consensus on whether conceptual mental action representations are symbolic \cite{Barsalou1999} or distributed \cite{Hommel2015_TEC}. A unifying proposal of modern theories (e.g.~\cite{Hommel2010}) suggests that conceptual compositional representations are distributed, and that language serves as a symbolification mechanism for the underlaying distributed representations. 
\emph{However, there exists no commonly agreed upon mathematical model of learning compositional action- and state representations that is mechanistically compatible to the neurocognitive perspective of distributed representations that are potentially symbolifiable.} 


Humans abstract their sensorimotor data streams and map them to conceptual embodied representations \citet{Barsalou2008_GroundedCognition}. 
High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
For example, on the lowest motor level, an \concept{open hand} action can be modelled as a sequence of continuous finger movements. The opening of the hand may be a semantic primitive within a high-level \concept{grasp} action that consists of \concept{[open hand, move hand to object, close hand]}. The grasp action itself may be a semantic primitive within another higher-level \concept{transport} behavior that consists of \concept{[grasp, move, release]}. 

This divide and conquer approach is also a prominent method to realize learning-based intelligent problem-solving behavior of robots and virtual agents. 

High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
This effectively reduces the branching factor of a problem-solving search process: for the high-level action selection, an agent only has to consider a small set of discrete high-level action primitives and not the large set of their possible low motor-level instantiations. 
This computational problem-solving perspective on sensorimotor abstraction is in-line with



% This article is targeted at researchers in Artificial Intelligence and related fields. Therefore, we can impossibly cover all findings from the life sciences and human sciences that are related to problem-solving, decision-making and mental representations. But how can we obtain an objective overview about the state of the art on learning-based decision-making and problem-solving in cognitive psychology and cognitive neuroscience? 

% In this section, we address this question by performing a meta review of recent survey articles in cognitive psychology and animal cognition. We select and analyze the most cited review articles on learning-based problem-solving from the last three years, which we identify as follows:

% \begin{enumerate}
%     \item 
% \end{enumerate}

% The analysis reveals that there exist several theories related to representational abstraction and predictive forward models for learning-based problem-solving that are largely agreed upon and described well enough to be formalized within a computational framework. 

==> results2.tex <==
\section{Critical discussion and outlook}
\label{sec:results}
Based on our considerations above and the supplementary \autoref{box:appendix:hrl_review} and \autoref{tab:hrl_properties},
we now proceed with summarising the shortcomings of current hierarchical reinforcement learning approaches. 
The shortcomings are consequences of specific challenges that arise from the integration of the different mechanisms (see \autoref{fig:challenges_shortcomings_solutions}). Here, we address these shortcomings with specific algorithmic suggestions. 
% We present an overview of the relation between the shortcomings, challenges and suggestions for potential partial solutions in 
% }{E-\ref{rev:editor:review_perspective}}
% We present a summary of these results in \autoref{sec:shortcomings_solutions}. 

\begin{figure*}
    \centering
    %\includegraphics[width=.8\textwidth,trim=2.5cm 4cm 2cm 4cm, clip]{pics/Shortcomings_Challenges_Solutions.pdf}
    \includegraphics[width=\textwidth]{pics/Figure6.pdf}
    \caption{
    \textbf{Shortcomings, challenges, and suggestions for HRL.}
    % \rev{\textbf{Shortcomings, challenges, and suggestions for HRL.}}{E \ref{rev:ed:figure_captions}} 
    Our section \nameref{sec:hrlFinal} identifies several shortcomings of contemporary HRL methods. We suppose that these result from at least four central challenges, and we provide three suggestions for key methods that may help to address the challenges.}
    \label{fig:challenges_shortcomings_solutions}
\end{figure*}

\subsection{Shortcomings and challenges of HRL architectures}
\label{sec:results:challenges}
% Our computational realizations section and the supplementary \autoref{tab:hrl_properties} provide a comprehensive overview over state-of-the-art computational hierarchical reinforcement learning approaches.
% % , in alignment with our structuring of cognitive prerequisites and mechanisms for the problem-solving abilities of intelligent biological agents (see \autoref{fig:cog_prereq}). 
We identify the following major challenges for current methods:

\begin{sloppypar}
\noindent \textbf{Hierarchical mental simulation requires stable hierarchical representations and precise predictions.}
Most current few-shot problem-solving methods build on transfer learning, but they neither leverage decision-time planning nor background planning to exploit hierarchical mental simulation.
While numerous non-hierarchical methods show how mental simulation can improve sample efficiency\cite{Deisenroth2011,Ha2018_WorldModels}, our summary in the supplementary \autoref{tab:hrl_properties} shows that reinforcement learning with hierarchical mental simulation on multiple layers is implemented in only one recent method\cite{Li2017_efficient_learning}.
% As a result, inter-dependencies between sub-tasks are hard to detect. 
A major reason for this shortcoming is that the low-level  policy should have already converged before the high-level forward model starts training. 
This problem has been addressed for model-free HRL \cite{Eysenbach2019_DiversityFunction}, but it has not yet been investigated with  predictive forward models. 
% \citet{Eysenbach2019_DiversityFunction} address this issue in a model-free architecture in two steps: first they pre-training low-level policies through an intrinsic reward function based on maximum entropy and once they have converged they use them to learn a high-level policy that composes the low-level policy. .  to pre-train domain-independent low-level policies first, and after convergence 
\end{sloppypar}

% This result is interesting because any approach with a forward model could straight-forwardly be extended to also consider planning\cite{Botvinick2014}.
% , and planning can be leveraged for few-shot problem-solving\cite{Sharma2020_DADS}. 
% Therefore, current model-based approaches do not exploit their full potential.

\begin{sloppypar}
\noindent \textbf{Intrinsic motivation requires forward models with elaborate uncertainty-handling.}
% In our survey, we distinguish between the three most frequently used kinds of intrinsic motivation: curiosity, diversity, and subgoal discovery. 
Our supplementary \autoref{tab:hrl_properties} show that curiosity and diversity are underrepresented intrinsic motivation methods: they are implemented in only 9 out of 50 surveyed papers, while our section \nameref{sec:cognitive_background} shows significant cognitive evidence that these mechanisms are critical for intelligent behaviour in biological agents\cite{Oudeyer2018_CompuCuriosityLearning}.

A potential reason for this shortcoming is that prediction-based intrinsic motivation suffers from an overly simplistic uncertainty handling of current computational forward models.
This is an issue for noisy observations or chaotic and unpredictable system dynamics. 
For example, \citet{Roeder2020_CHAC} achieve curiosity-driven intrinsic motivation by maximising the prediction error of a forward model. 
This causes the agent to suffer from the so-called \emph{noisy TV problem}, where an agent always strives to encounter unpredictable observations (such as a TV showing only white noise). 
This problem interferes with the problem of learning hierarchical representations because it does not address uncertainties of high-level representations if the learning of these representations has not yet converged.
\end{sloppypar}

\noindent \textbf{Compositionality requires elaborate role-filler representations.}
Only a few HRL methods consider compositionality. 
Exceptions include natural language-based representations of actions \cite{Jiang2019_HRL_Language_Abstraction} or symbolic logic-based compositional representations \cite{Oh2017_Zero-shotTaskGeneralizationDeepRL}.
Since compositional representations generally build on variable-value representations, these need to be researched first on a more foundational level to alleviate this shortcoming. 
Graph neural networks, a class of neural networks that encode entities and their interactions as nodes and edges within a graph \cite{Battaglia:2018}, are a promising approach for compositional representations.
When provided with the underlying graph structure, Graph neural networks seem to generalise better and support relational reasoning \cite{Battaglia:2018}.
However, discovering a suitably abstracted graph from data remains an open challenge.

\noindent \textbf{Inference-fitted state abstraction requires a strong learning signal.}
Recent HRL approaches \cite{Levy2019_Hierarchical,Roeder2020_CHAC} use the same state representation for each layer in the hierarchy. 
However, it seems cognitively more plausible to fit the level of abstraction to the level of inference needed on each hierarchical level.
For example, a high-level layer may only need to know whether an object is graspable, it does not need to consider its precise shape. This more detailed information, however, is relevant for the low-level layer that performs the grasping.
There exist RL-methods that learn state abstractions from visual data with a convolutional autoencoder\cite{Ha2018_WorldModels}. 
%There exist RL-methods, where abstract (aka. latent) representations are generated from visual data with a convolutional autoencoder\cite{Ha2018_WorldModels}. 
However, such representations are optimised for reconstructing the visual input---not for decision-making. 
Furthermore, in the existing recent vision-based architectures\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}, all hierarchical layers of the RL agent are provided with the same image embedding. %output of the ConvNet, i.e., with the same level of representational abstraction. 
Therefore, the abstractions are not inference-fitted. 
% There exist a few approaches that perform inference-fitted state abstraction\cite{Vezhnevets2017_Feudal}, and also some that involve compositional state representations\cite{Vezhnevets2020_OPRE}. 
% However, most of these build on hand-crafted abstraction functions that are not learned \cite{Eppe2019_planning_rl}.
A problem for learning inference-fitted abstraction functions is that the reward signal of reinforcement learning is a relatively weak driver for the learning process, compared to other methods like supervised learning. 
%Ideally, behavioral inferences should unfold selectively on the appropriate representational levels dependent on the current goals and motivations of the system.



% \subsection{Central challenges of integrated hierarchical architectures}
% \label{sec:results:challenges}
% We hypothesize that the above shortcomings are the result of several central challenges that occur when integrating the mechanisms depicted in \autoref{fig:cog_prereq} in a unifying hierarchical architecture.  


% % These involve advanced uncertainty models, computational implementations of bidirectional action-effect associations, and inference-fitted abstraction. 


% % \textbf{Uncertainty modelling}

% % \textbf{Bidirectional action-effect models}

% % \textbf{Inference-fitted abstraction}



% \noindent \textbf{Stabilize hierarchical representation learning.} 
% Hierarchical mental simulation demands stable high-level representations to learn a high-level forward model. 
% However, a general problem of hierarchical architectures is that a high-level layer can only learn meaningful behaviour after the lower-level layer has converged. 
% % A naive solution to address this issue is a threshold-based mechanism that detects the convergence of the lower-level to determine when the higher level layer may start training. 
% % This, however, does not consider continual and lifelong learning settings, where an agent's lower level behaviours and representations develop continuously. 
% % In hierarchical decision-making, this problem affects hierarchical mental simulation. 
% In the next subsection, we discuss how learning in hindsight\cite{Andrychowicz2017,Levy2019_Hierarchical} and bi-directional dynamics models\cite{Pathak2017_forward_model_intrinsic,Pathak2019_ICML_SelfSuperExploreDisa} may partially alleviate this problem.

% \noindent \textbf{Alleviate the model bias.}
% A forward model is never perfect, and multiple successive predictions lead to huge accumulated errors that render the predictions unusable. This problem is known as the model bias problem, and it demands for better uncertainty models to make the agent aware of the confidence of its predictions. 
% % Successful non-hierarchical approaches like PILCO \cite{Deisenroth2011} demonstrate the sample-efficiency of uncertainty-aware forward models based on Gaussian Process Models, but these models are only suitable for low-dimensional state and action representations. 
% Another dimension of this problem occurs with noisy observations or chaotic and unpredictable system dynamics, which is an issue for intrinsic motivation methods based on prediction. 
% For example, \citet{Roeder2020_CHAC} achieve curiosity-driven intrinsic motivation by maximizing the prediction error of a forward model. 
% This causes the agent to suffer from the so-called \emph{noisy TV problem}, where an agent always strives to encounter unpredictable observations (such as a TV showing only white noise), instead of searching for predictable situations that it just cannot predict yet. 

% In a hierarchical setting, this problem interferes with the problem of learning hierarchical representations, because high-level representations that are still being learned are hardly predictable at all. 


% \noindent \textbf{Improve variable-value assignment.}
% Abstract compositional representations build on rules to determine the semantics of the composed data structure. 
% These rules require, in one way or another, variable-value pairs, where the variable describes a general semantic property. 
% For example, the disentangled vector representations that occur in variational autoencoders (VAEs) are compositional data structures, where each slot of the vector is a variable that represents a certain object property (e.g. the angle of a visual object).
% In language, the variables are roles of syntactic constructions, and the values are the words that fill these roles. 
% A problem with VAEs is that they do not support dynamic semantic representations with varying variables because the structure of the latent representations fixed, and therefore, also  the set of variables is fixed. They also do not support variables that are assigned to other variables. 
% Variable-value assignment is a particular issue in hierarchical decision-making, where low-level sensorimotor data is abstracted to high-level compositional representations that are used for high-level decision-making. 

% % \citet{Kriete2013_SymbolProc} provide a neurologically plausible model of variable-value assignment where variables are areas in the prefrontal cortex that act like a pointer in computer science, pointing to other areas which represent values. 
% % This is somewhat akin to Transformer neural networks, where Query, Key and Value vectors are used for a self-attention-mechanisms. 



% \noindent \textbf{Strengthen the feedback signal.}
% Learning-based inference-fitted abstraction demands a strong feedback signal to learn the respective abstraction functions. 
% However, in reinforcement learning the reward signal is often relatively weak compared to a supervised loss signal, especially in sparse reward settings where handshaped continuous reward functions are not present.
% In hierarchical reinforcement learning, this problem is even more severe if the goal is to learn also abstraction functions for inference-fitted high-level state representations. 
% Hence, hierarchical reinforcement learning with inference-fitted abstraction demands a stronger feedback signal to stabilize the learning. 
% % In the subsection below, we propose a potential solution to address this problem, based on bi-directional dynamics models. 

\subsection{Outlook and suggestions for addressing the challenges}
\label{sec:results:solutions}
In the following, we sketch how computational key methods may potentially help to address the above challenges. 
% The methods will not solve all problems related to hierarchical reinforcement learning, but we believe that they are important key mechanisms for future developments. 

\noindent \textbf{Retrospective analysis of experiences.}
% \noindent \textbf{Learning in hindsight.}
% Hierarchical reinforcement learning demands stable high-level representations. 
A central problem of HRL is that stable high-level representations can only emerge once the learning of the lower-level has converged \cite{Eysenbach2019_DiversityFunction}. 
We suggest that a retrospective analysis of experiences can alleviate this issue.
This has been demonstrated for training a policy by learning in hindsight\cite{Andrychowicz2017,Levy2019_Hierarchical}, where the achieved world state of a policy is retrospectively pretended to be the desired goal state. 
% Learning in hindsight\cite{Andrychowicz2017} has been proposed  to alleviate the sparse reward problem in goal-conditioned reinforcement learning. 
% The technique builds on learning from failures, in the sense that an agent gets rewarded even if it fails to achieve a reinforcement learning goal. 
% This is realized by pretending in hindsight that the achieved goal was the actual goal. 
% \citet{Levy2019_Hierarchical} extend the method to hierarchical architectures by also proposing hindsight actions. 
% In their hierarchical framework, high-level actions are subgoals to be achieved by the lower-level layer. 
% Hindsight high-level actions are retrospectively defined as the subgoals that were actually achieved by the low-level layer, regardless of what the original subgoal was. 
% In other words, by pretending in hindsight that the executed action (aka. subgoal) was the intended action, there is no need any more to wait until the low-level behaviour has converged. 
We suggest that hindsight learning is a special case of a more general retrospective analysis of memorised experiences. 
For example, it is potentially possible to also learn hierarchical forward models in hindsight, without the high-level layer having to wait for a low-level layer to converge. %that a high-level layer has to wait for a low-level layer to converge.
We hypothesise that re-considering the outcome of past erroneous actions of a not yet fully trained low-level layer as a desired outcome can stabilise the high-level representations. 
Such a technique may also help to alleviate the model bias.
% , but, of course, there are still many other open ends to address. 





\noindent \textbf{Meta- uncertainty models.}
Prediction errors play an important role in mental simulation and intrinsic motivation. 
In our section \nameref{sec:cognitive_background} we have discussed the free energy principle, which involves two seemingly contradicting mechanisms that build on predictive processing models. 
On the one hand, there is active inference \cite{Schwartenbeck2019_CompUncertainExplo}, which seeks to minimise long-term surprise. This can be implemented by minimising a forward model's uncertainty or prediction error. On the other hand, there is active learning, which seeks to maximise information gain. This can be implemented by maximising uncertainty\cite{Haarnoja2018_SAC} or prediction errors \cite{Roeder2020_CHAC} through respective intrinsic reward functions.
\citet{Schwartenbeck2019_CompUncertainExplo} address this contradiction by building on \emph{expected uncertainty}\cite{Yu2005UncertaintyAttention} to unify both mechanisms. 
% Unexpected uncertainty can be understood as meta-uncertainty, i.e., the uncertainty about the uncertainty.
Expected as well as unexpected uncertainty then can be understood as a meta-uncertainty-analysis. 
We suppose that an intrinsic reward for high \emph{meta-}uncertainty may lead to exploratory behaviour, causing the exploration of high short-term but anticipated lower long-term meta-uncertainty. Furthermore, the gained certainty about the uncertainty of forward models can lead to improved predictive processes, which are aware of their own limits\cite{Baldwin:2021}. 

\noindent \textbf{Bidirectional dynamics models.}
Bidirectional models involve both forward and backward inference, and we suppose that this combination is beneficial for representational abstraction in
hierarchical architectures.
Our supposition is based on the work by \citet{Pathak2017_forward_model_intrinsic} and by \citet{Hafner2020_Dreamer}, who use a combined forward and inverse model to generate latent representations in a self-supervised manner. 
The bidirectional model operates on a latent space, generated by an abstraction function. 
% Their methods learn simultaneously the abstraction function, the forward model and the inverse model. 
By simultaneously performing inverse and backward prediction in the latent space, the abstraction function gains two important features: First, the latent space is de-noised because only the predictable parts of the latent observation determine the forward and backward prediction. Second, the method is self-supervised and, therefore, provides a more stable feedback signal than the comparatively weak reward signal.
This alleviates the prediction error and strengthens the overall learning signal. 

% The stronger learning signal is also better suited to learn advanced abstraction functions that generate compositional representations, e.g. disentangled state vectors or symbolic compositional representations\cite{Lyu2019_SDRL,Eppe2019_planning_rl}. 
% \noindent \subsection{Challenges remaining}
% The above proposals for addressing the central challenges of hierarchical reinforcement learning are  not sufficient for developing artificial agents that are as smart as the crow of \autoref{fig:crow_probsolving}. 
% The biggest challenge remaining is the integration of the methods, towards a unifying computational framework.
% A problem is the cross-dependencies between the individual methods, as each added component increases the complexity of training and evaluation.
% For example, hindsight learning requires bi-directional abstraction functions to map abstract high-level representation back to the context-specific low-level representations. 
% This is necessary because otherwise the system cannot reward successful high-level hindsight actions with the information from the low-level state representation. Another open question is how to model meta-uncertainty in bidirectional models. 
% % These cross-dependencies are not only conceptually difficult, they also imply software-technological challenges. Each one of the proposed mechanisms comes with its ows variants and hyperparameters TBC...
% It is impossible to foresee all remaining challenges, but we hope that we did present here some useful guidelines for next steps, grounded in cognitive and computational evidence. We encourage attempts to elaborate these further to understand the remaining challenges better.




==> revision.tex <==
\onecolumn

\thispagestyle{empty}%
\vskip-36pt%
{\raggedright\sffamily\bfseries\fontsize{20}{25}\selectfont Response to referees \\[10pt] \Large \newtitle  \par}%
\vskip10pt
{\raggedright\sffamily\fontsize{12}{16}\selectfont  \newauthor \par}
\vskip25pt%

% \section{Statement of revision}

\noindent \textbf{Dear Trenton Jerde, dear anonymous reviewers}\\[0pt]

\noindent Your response to the revision of our article was positive, and you accept the article for publication if we address your last minor comments and form issues. We also received final helpful comments by Reviewers 2 and 3. We highly appreciate that each individual referee took the time to review our revision. In the following, we provide the requested point-by-point description to detail how we addressed your last requests and suggestions. 

Where possible, we marked the changes in the document. However, many final suggestions resulted in shortening and subtle minor re-formulations that we left unmarked. 

% As with our last revision, we tried to maximise the convenience for the reviewers by marking the relevant rewritten passages in the text in \revv{dark blue colour and we also placed a side note on the article's margin to indicate which of the suggestions is addressed by the revised passage.}{Side notes contain references to the addressed suggestions.}
% In the side note, we refer to the suggestion with E (for editor) and R1, R2, R3 for the three reviewers, followed by the item number of the enumeration in the statement of revision below. For example, R3-\ref{rev:r3:controversial_theories:embodiment} refers to item \ref{rev:r3:controversial_theories:embodiment} raised by Reviewer 3.


\subsection{Editor's response}
\label{rev:editor}
The editor conditionally accepts our article and points us to eight form issues that we address as follows: 


\begin{enumerate}
    \item 
    \label{rev:editor:abstract}
    \textit{Abstract:} The editor asks us to shorten the abstract to 150-200 words. 
    
    \textit{Our response:} We improved the abstract by rephrasing and shortening several sentences. It now contains around 171 words. 
    
    \item 
    \textit{Length:} The editor asks us not to increase the length further and, if possible, shorten the text further instead.  
     
        
    \textit{Our response: } 
    We did not increase the length further. Instead, we managed to slightly further shorten the paper, so that it now consists of 4676 words, compared to our previously submitted version with 4739 words. 
    
    
    \item 
    \textit{Main text:} The editor reminds us to use British English, appropriate section headings, and he recommends improving the summary of our article at the end of the introduction. Furthermore, the editor recommends avoiding terms like ``new'' or ``novel''. 
        
    \textit{Our response: }
    In another iteration, we checked for using BE, appropriate section titles, and we improved the end of the introduction further. Furthermore, we removed occurrences of ``new'' and ``novel'' and ``first'' where appropriate. We kept occurrences of ``novel'' in the context of problem-solving, when we refer to a problem that an agent has never seen before. 
    
    \item
    \textit{Figures:} We were asked to check the figure guidelines.
        
    \textit{Our response: } We made sure to only use PDFs for our figures and to use suitable fonts within the figures. 
    
    \item 
    \label{rev:ed:figure_captions}
    \textit{Figure captions:} We were asked to update the figure captions to fit the figure caption guidelines.
        
    \textit{Our response: } We added short titles (printed in \textbf{bold}) that describe the figure as a whole to all captions.  We made sure all captions  are less than 200 words long.
    
    \item 
    \textit{Statistics reporting:} 
    We do not report any statistics in our article. 
        
    \item 
    \textit{References:} The editor asks us to consider again the guidelines for references.

    \textit{Our response: } 
     We fixed all references. There are very few papers we reference that have been published on ArXiv without peer review. However, these few exceptional articles have been cited very often and are publicly available. 
     Furthermore, we found that the numbering of the literature references in the previous version of the supplementary material was not appropriate: The numbering was not fully consecutive in the sense that there were ``jumps'' in the numbering of the references of the supplementary material. We fixed the problem in this final revised version.

    \textit{Related manuscripts:} 
    There are no related manuscripts submitted to other venues. We only published the first draft of this article as a preprint on arxiv (https://arxiv.org/abs/2012.10147). 
    
    
\end{enumerate}




\subsection{Reviewer 1}
\label{rev:r1}
The reviewer finds all of his concerns addressed and accepts our revision as it is.



\subsection{Reviewer 2}
The reviewer appreciates that we have substantially revised the article and supports the publication. He points out one last minor issue: 

\begin{enumerate}
    \item 
    \label{rev:r2:clarify_pred_errors}
    The reviewer suggests clarifying what we mean by prediction error minimisation.
    
    \textit{Our response:} We agree that confusions could arise on what is meant by prediction error minimisation. We changed the respective sentence on p.3 (right) to describe in more detail what we mean here (i.e., learning progress).
\end{enumerate}

\subsection{Reviewer 3}
\label{rev:r3}
The reviewer acknowledges that the revision has substantially improved over the previous version. The reviewer provides final constructive feedback regarding the following remaining minor issues:

\begin{enumerate}

    \item
    \label{rev:r3:clarify_contrib}
    The reviewer suggests clarifying further our contribution in the earlier parts of the paper. 
    
    \textit{Our response: }
    We clarified the contribution in the abstract, and we believe that the description of the contribution in the introduction is also appropriate (``We suggest steps towards combining key methods and mechanisms to overcome the integration challenge for the development of a unifying cognitive architecture.'')
    
    \item
    \label{rev:rev3:title}
    Based on the new pitch of the article, which is now less related to ``embodiment'' and ``principles'', the reviewer suggests re-considering the title. 
    
    \textit{Our response: }
    We agree that the title had potential for improvement. It is true that the distinction between ``principle'' and ``mechanism'' is blurry. Furthermore, in our new revision, the embodiment aspect is less explicit. 
    Another issue that we found with our title 
    % include that it described \textbf{what} we propose (principles and mechanisms to improve HRL), but not \textbf{why} (because we want intelligent problem-solving agents). Finally, the previous title
    is that it did not convey clearly enough our main contribution and the integration aspect of our work. Our main contribution is the presentation of intelligent problem-solving behaviour as integrated hierarchical reinforcement learning, and we now communicate this clearly in the new title ``\newtitle''. This new improved title resolves the issues with the terms ``mechanism'', ``principle'' and ``embodiment''.
    
    % Therefore, we now use the term ``mechanisms'' in the title. However, embodiment still plays a critical role because all MDP-driven agents must have (at least a virtual) body to perform actions. Furthermore, for example, representational abstraction is inherently governed by the agent's body. Hence, we prefer to keep the word in the title. Nevertheless, we agree that the integration aspect is also important. Therefore, we changed the title to ``\newtitle''.
    
    \item 
    \label{rev:r3:final_edit}
    The reviewer suggests further copy editing to fix last wording issues concerning capitalization and usage of vocabulary. 
    
    \textit{Our response: } We thank the reviewer for pointing out these last points. We did another full iteration of copy-editing to fix these and other wording issues.  
    
    \item
    \label{rev:r3:links_to_supp}
    The reviewer appreciates the supplementary material, but suggests considering better best practices for dividing between supplementary material and main text.
    
    \textit{Our response: } 
    We agree that there is plenty of supplementary material. However, we took care that the article is self-contained without consulting it. Specifically, we assured that all concepts are explained clearly also in the main text. For example, decision-time planning and background planning are sufficiently explained, and also the other terms used in the glossary. The glossary serves more as an additional quick look-up tool, and remains optional for those readers who require a more detailed description of a particular concept or term. 

    
\end{enumerate}




==> v0/cognitive_evidence.tex <==
\section{Cognitive Problem-solving and Learning Mechanisms}
\label{sec:cognitive_background}

Humans and some intelligent non-human animals including certain primates, dolphins, octopuses and corvids are excellent problem-solvers. 
% For example, New Caledonian crows can plan ahead several steps in a goal-directed manner, and they can transfer solutions to previously solved (sub-)problems to new ones \cite{Gruber2019_CrowMentalRep}. 
There exists extensive research in human and animal cognition and Psychology that identifies and describes mechanisms that are responsible for these capabilities \cite{Gruber2019_CrowMentalRep,Rumbaugh2003_Intelligence_Apes}. 
In this section, we will provide a brief high-level non-comprehensive overview about these mechanisms. To maintain the scope of this review feasible we consider those mechanisms that are relevant for hierarchical problem-solving.
Each of the following subsections refers to a family of cognitive mechanisms related to embodied problem-solving. 
% From each mechanism we derive a brief summary of desiderata that are relevant for hierarchical reinforcement learning. 

% \subsection{Multi-timescale learning}
% Plasiticity in the amygdala is fast, it is activity-dependent. In the triatum it is slow, it is dopamine-dependent. (see p. 136 left in \cite{Neftci2019_RL_artificial_bio}). Both operate in parallel on the same hierarchical level. For decision-making both are queried in parallel to integrate quickly learned but prone-to-noise behavior with slow but steadily learned behavior. 
% \mybox[black!20]{
% \begin{itemize}
%     \item \textbf{Multi-timescale learning.} \quad 
%     \item 
% \end{itemize}
% }

\subsection{Inverse models and ideomotor theory (Christian, Martin, Phuong)} 
The inverse model directly maps desires to actions. It implements reactive behavior. It is the basis of a fast decision-making system (Kahnemann's System 1?) 
Ideomotor theory suggests that there exists an inverse model that is responsible for action selection. The inverse model (bi-)associates actions with desired effects.

The Ideomotor principle was made popular by \citet{James1890_Psychology}, but its origins can be traced back even further to the early 19th century \cite{Stock2004_Ideomotor}.
According to the Ideomotor Principle, motor actions are bidirectionally linked to the perceptual effects they produce \cite{Koch2004_Ideomotor}.
This action-effect learning starts during early development when simple reflex-like motions, such as arm movements during motor babbling, are linked to the perceived sensory effects, such as a change in perceived hand position  \cite{Stock2004_Ideomotor}.
This action-effect association can be used at a later stage for goal-directed control.
When a particular perceptual effect is desired, such as grasping an object, the associated motor action are activated, resulting in a motion of the hand towards the object.


Related bidirectional action-effect learning were later implemented in control system.
\citet{Wolpert1998_ForwardInverse} proposed using modular coupled forward-inverse models for action control and later implemented this mechanism in their classical MOSAIC architecture \cite{Haruno2001_MOSAIC}.
The bidirectionality of the action-effect association is here made explicit by using two types of models:
A forward model is used to predict the sensory effect of a motor actions, while an inverse model receives the current and next sensory state as an input and outputs the action resulting in this state transition.
Coupled forward-and-inverse models find applications to this day outside of the reinforcement learning community (e.g., \cite{someRecentExamples}).


\mybox[black!20]{
\begin{itemize}
    \item \textbf{Inverse model.} \quad Ideomotor theory suggests that there exists an inverse model that is responsible for action selection. The inverse model associates actions with desired effects.
\end{itemize}
% The \textbf{computational requirements} for implementing the desiderata are:
% \begin{itemize}
%     \item Learning a forward model
%     \item ...
% \end{itemize}
}

% CG: I would suggest following the Ideomotor part with Theory of Event Coding, since they really fit together


\subsection{Active inference: curiosity, surprise and intrinsic motivation (Christian / Martin)}


\mybox[black!20]{
The active inference principle suggests the following desiderata for HRL architectures
\begin{itemize}
    \item \textbf{Minimize Free energy.} \quad Define an intrinsic reward function that is proportional to the forward prediction error. This will lead to an agent that strives to maximize the prediction error in the short run, so that the error is minimized in the long run. \quad 
\end{itemize}
% The \textbf{computational requirements} for implementing the desiderata are:
% \begin{itemize}
%     \item Learning a forward model
%     \item ...
% \end{itemize}
}

% Curiosity and overcoming sparse external rewards with intrinsic rewards. 

\subsection{Event segmentation (Christian / Martin)}

Event Segmentation Theory (EST) \cite{Zacks2007_EST} is concerned with why humans seem to perceive the continuous sensory activity in terms of discrete, conceptual events.
EST was originally formulated based on a variety of video segmentation tasks and the observation that humans tend to consistently segment the videos at similar points in time \cite{Zacks2001_EventStructure}.
EST suggests that these segmentations mirror the internal representation of the unfolding experience in terms of events.
Internal representations of events, or \emph{event models}, are a form of state abstraction, that encode entities with certain properties and their functional relations in a spatiotemporal framework \cite{Radvansky2011_EventPerception}.
According to EST, these event models guide the perception by providing additional information that can be used for forward predictions \cite{Zacks2007_EST}.
Over the duration of one event a subset of these event models is active.
A particular subset is active until an unexpected, transient error in prediction occurs \cite{Zacks2007_EST}.
This unexpected prediction error may result in a exchange of the currently active event models to a new subset that may be better suited for predicting the currently ongoing dynamics \cite{Radvansky2011_EventPerception}.
Thus, event models are highly compositional, in the sense that a particular subset of active event models constitutes to the perception of one particular event.
Furthermore, EST suggests, that such prediction error-based segmentations occur on multiple levels of perceptual processing resulting in a hierarchical organization of event models \cite{Zacks2007_EST, Zacks2001_EventStructure}.
%EST is supported by neurological evidence, that found that transient increases of brain activity occur when perceiving an event boundary, regardless whether the perception comes from passively viewing or reading. %Maybe add this to neurological evidence, TODO: References missing
In sum, EST proposes the existence of event models, a form of compositional, hierarchically organized state abstraction used for perceptual prediction and suggests that unexpectedly strong prediction error signals could be used for learning these abstractions.

%\label{sec:cognitive_evidence:event_segmentation}
%The theory of event segmentation suggests that there exist behavior primitives, that are determined by the prediction error of a forward model.

\mybox[black!20]{

\begin{itemize}
    \item \textbf{Event models}. \quad A form of state abstraction. Used for forward prediction. Transient prediction errors lead to an exchange of event models. \quad 
\end{itemize}
 The \textbf{computational requirements} for implementing the desiderata are:
 \begin{itemize}
     \item Learning a forward model
     \item Prediction error monitoring
     \item (maybe some preprocessed sensory information to identify involved entitites)
 \end{itemize}
}


\subsection{Semantic cognition, category learning and mental concept representation}
\label{sec:cognitive_evidence:semantic_cognition}
Humans think in categories \cite{Waldmann2017_Kategorisierung_Wissen}. 
There are several theories how this is achieved. There exist theories based on similarities, which include categorization by prototypes, exemplars and decision boundaries (cf. \cite{Waldmann2017_Kategorisierung_Wissen} for an overview). \citet{Rips2012_Concepts_Categories_theoryTheory} propose a category-learning principle based on theories that a cognitive agent has. In this theory-theory view, objects, situations, states and actions are represented by causal features and functional relations. 
This implies that mental categories are learned such that causal predictions are optimized. 
The authors also suggest that there exist categories of relations between objects. This implies, for example, that birds are categorized by a property \emph{can fly}. 

The theory-theory is compatible with research by \citet{Rogers2008_SemanticCognition}, who present the parallel distributed processing (PDP) theory. Herein, they extend previous work by \citet{Rumelhart1993_LearnConnRep}, who model compositional mental concept representations with a feed-forward supervised learning approach: Given neural representations for a semantic item (e.g.~canary bird) and a semantic relation (e.g.~can), the neural network learns to activate suitable attribute representations (e.g.~grow, move, fly, sing). 
\citet{Rogers2008_SemanticCognition} argue that the combination of knowledge about an object and a context (i.e., current stimulus) allow for anticipation and prediction. (E.g. a bird (object) sitting on a tree while a cat is approaching (context) will fly away). 

The authors show with a simple computational feed-forward neural network model how their PDP theory explains how humans induce properties from their experience. Since the vector representation of bird concepts is similar for all bird species, their forward-propagation of weights is similar. Hence, after having learned that certain birds can sing, and then having learned that a canary is a bird, humans can infer that canaries can sing. Note that this can also lead to false deductive conclusions.


\mybox[black!20]{
\begin{itemize}
    \item \textbf{Compositional concept and category representations}. \quad Concepts are represented by composing items with relations and arguments. \cite{Rogers2008_SemanticCognition,Rumelhart1993_LearnConnRep,Rips2012_Concepts_Categories_theoryTheory}.
\end{itemize}
}

% \subsection{Category learning (Manfred, Christian, Martin)}
% \label{sec:cognitive_evidence:category_learning}
% Humans think in categories \cite{Waldmann2017_Kategorisierung_Wissen}. There are several theories how this is achieved. There exist theories based on similarities, which include categorization by prototypes, exemplars and decision boundaries (cf. \cite{Waldmann2017_Kategorisierung_Wissen} for an overview). There exist also theories based on theories that a cognitive agent has. In this theory-theory view, objects, situations, states and actions are represented by causal features and functional relations. Similar to the semantic cognition perspective of \citet{Rogers2008_SemanticCognition}, this implies that, for example, birds are categorized by a property \emph{can fly}. 

% \citet{Waldmann2017_Kategorisierung_Wissen} state that mental categories are learned such that causal predictions are optimized. The paper also suggests that there exist categories of relations between objects. 


\subsection{Neural mechanisms of hierarchical planning and event representation}
\label{sec:cognitive_evidence:hierarchical_planning}
Neuroimaging makes it possible to observe how humans plan complex tasks. \citet{Balaguer2016_HierarchicalPlanning} present a fMRI-based study that depict how humans represent plans hierarchically. The authors' results suggest that the in the dorsomedial prefrontal cortex (dmPFC) maintains discrete abstract state representations, referred to as \emph{contexts}. The authors argue, that the neural cost of representation for discrete abstract state representations are lower than for more specific low-level representations. 

\citet{Schapiro2013_} and later \citet{Tomov2019_} showed that ``people can detect transitions between states belonging to different clusters in a graph with a particular topological structure, such that nodes in certain parts of the graph are more densely connected with each other than with other nodes'' \cite{Tomov2019_}. This is insofar compatible with the Event Segmentation Theory (EST) \cite{Zacks2007_EST}, as both assume certain bottleneck states that mark the start or end of a certain high-level representation. In EST, however, these states are identified by measuring the prediction error of a forward model, while \citet{Schapiro2013_} model bottleneck states as links between graph-theoretical communities.

\mybox[black!20]{
\begin{itemize}
    \item \textbf{Abstract discrete state representations}. \quad Humans represent plans as a hierarchical arrangement of discrete high-level states (contexts).  \cite{Balaguer2016_HierarchicalPlanning}.
\end{itemize}
}

\subsection{Event Coding (Christian / Martin)}
\label{sec:cognitive_evidence:event_coding}
%The theory of event coding (TEC) %\cite{Hommel2015_TEC,Hommel2001_TEC,Hommel2019_TEC} suggests, that mental representations (codes) of events and actions are composed from several other representations. 
Theory of Event Coding (TEC) \cite{Hommel2015_TEC,Hommel2001_TEC,Hommel2019_TEC} is a theoretical framework that builds upon the Ideomotor Principle.
In contrast to previous theories that deal with action and perception in isolation, TEC proposes that both actions as well as sensory information is encoded in a common format, i.e., an event code \cite{Hommel2001_TEC}.
An event, irrelevant whether it is the perception of a stimulus or an action, is internally encoded as a network of compositional feature codes \cite{Hommel2019_TEC}.
Such feature codes can represent information from all types of sensorimotor modalities, such as muscle activity, haptic stimulation, or visual information, and can encode properties of different complexity, ranging from something simple as color or shape to complex affordances such as `graspable-ness' \cite{Hommel2001_TEC}.
The activation of one feature code primes all event codes that share this particular feature code.

TEC explains both reactive as well as goal-directed behavior through the proposed event codes and feature codes they are made of.
If an action is followed by a particular effect, both the event codes for the action and the effect share a significant proportion of their feature codes.
Thus, by thinking about a particular desired effect, attentional mechanism activate the goal event code and the activation of shared feature codes triggers the activation of the action code leading to this effect \cite{Hommel2009_Action}.
TEC provides a similar explanation for reactive behavior: if a certain stimulus is often followed by a particular behavior, they share a large number of feature codes.
Thus, after enough exposure of this stimulus-behavior-combination, the mere perception of a certain stimulus automatically activates the behavior over the common feature codes \cite{Hommel2009_Action}.
 

Thus, TEC blurs the line between state and action abstraction, and instead proposes a general mechanism for sensorimotor abstractions, linking both motor and sensory representations in a common format.
Furthermore, TEC emphasizes that the compositionality of the underlying feature codes enables both goal-directed planning as well as reactive action-effect learning via simple associative learning.


\mybox[black!20]{
\begin{itemize}
    \item \textbf{Compositionality of event and action primitives}. \quad  Events are a compositional bundle of features \cite{Hommel2015_TEC}. 
    \item event codes can encode action and perception, thus, are both a state as well as an action abstraction
    \item feature codes that make up one event code are linked
    \item activation of one feature code primes related event codes
    \item explains how both goal-directed as well as reactive behavior can be achieved
    \item Are event codes forward or inverse models? Not clear to me... Seems like they can be both
\end{itemize}
}

\subsection{Training by mental imagery (Manfred / Christian / Martin)}

Athletes train by mentally simulating their body movement. 
Mental motor imagery: \citet{Jeannerod1995_MentalImageryMotor}.
\mybox[black!20]{
\begin{itemize}
    \item \textbf{Mental Imagery.} \quad Humans can train a skill by imagination, using a learned forward model, instead of physically executing action. \quad 
\end{itemize}
}

\subsection{Planning and Plan Verification (Manfred / Martin / Christian}
Intelligent biological agents can plan ahead. The planning is realized through mental simulation. For example, \autoref{fig:crow_probsolving} illustrates how New Caledonian crows can plan at least three steps ahead \cite{Gruber2019_CrowMentalRep} to solve a puzzle that provides reward in the form of food. The planning capability is possible with a high-level forward model that operates in the space of high-level mental representations and action primitives \cite{Taylor2014_CorvidCog}. Humans also commonly plan ahead, e.g., in chess. However, also the human planning-horizon is limited, most likely because the working memory of biological agents has a limited capacity \cite{SomebodyMustHaveInvestigatedThis}.


% Considering a limited time horizon imposed by the limited working memory, 
It is, however, unlikely that a large search space that grows exponentially with the planning horizon can completely be covered with an exhaustive cognitive search process \cite{}. A hypothesis by \cite{SomebodyMustHaveInvestigatedThis} is that the search space is pruned by an inverse model that generates candidate plans which are then subject to verification by mental simulation with the forward model. 
% Based on the verification result, the inverse model proposes a new plan if the previous plan could not be verified. 
This perspective is in-line with recent findings that suggest that a forward model is rather an auxiliary than an integral element for problem-solving \cite{Pickering2014_ForwardModels_AFM_IFM}. 

A similar mechanism is deemed to exist in mental concept blending \cite{Fauconnier2002,Eppe2018_AIJ_Blending}. Concept blending is a critical pillar of human creativity, which involves the combination of two existing concepts to obtain a new concept. During the so-called \emph{completion} phase of the blending, the blend is verified and, if necessary, updated to adhere so certain optimality criteria, such as consistency. 

\mybox[black!20]{
\begin{itemize}
    \item \textbf{Plan generation.} \quad Perform a search over the action space using a mental forward-model to find a plan that leads to a goal.
    \item \textbf{Plan verification.} \quad Use a mental forward-model to simulate actions chosen by an inverse model before actually executing them, in order to verify the desired outcome.
\end{itemize}
% The \textbf{computational requirements} for implementing the desiderata are:
% \begin{itemize}
%     \item Learning a forward model
%     \item ...
% \end{itemize}
}

\subsection{Embodied Sensorimotor Grounding and Mental Representations (Manfred)}
\label{sec:cognitive_background:grounding}
Humans abstract their sensorimotor data streams and map them to conceptual embodied representations \citet{Barsalou2008_GroundedCognition}. 
The conceptualization hypothesis by \citet{Lakoff1999}, which claims that humans organize their thought in terms of hierarchical mental concepts that are grounded in sensorimotor experience. The theory entails that our body determines the the way we think, i.e., our body-specific sensorimotor apparatus determines how we conceptualize the world \cite{Shapiro2019_EmbodiedCognition}. 
The conceptualization theory has further implications in cognitive lingusitics \cite{Feldman2006}, where attempts to represent mental concepts as so-called \emph{semantic frames} \cite{Osswald2014_FrameNet,Fillmore1985} within grammatical semantic schemas have been made \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing,Trott2016,Feldman2009_ECG}. 

A critical consequence of the embodied conceptualization theory is that both state and action concepts are represented in a compositional semantics that is based on roles and fillers. For example, an intentional action has roles for \concept{protagonist} (the agent executing the action), \concept{patient} (e.g. an entity being manipulated by the action), and so on. Cognitively plausible theories like Embodied Construction Grammar \cite{Feldman2009_ECG} propose to use inheritance structures to realize a hierarchy of actions. For example, a motion action inherits the role \concept{protagonist} from an abstract \concept{process} schema and adds the \concept{source} and \concept{goal} roles that determine the start and end of the motion. The motion schema is then used for further inheritance, e.g., to describe a \concept{walk} action where the protagonist is constrained to be a humanoid agent. 

Animal cognition provides further evidence that actions are compositional. Specifically, \citet{Flash2005_AnimalMotorPrimitives} propose a compositional set of motor primitives in vertebrates and invertebrates that combine to complex motor behavior using well-defined syntactic rules. 



\mybox[black!20]{
% From the embodied conceptualization theory, we derive the following desiderata for hierarchical reinforcement learning agents:
\begin{itemize}
    \item \textbf{Action abstraction.} \quad Sensorimotor experience leads to compositional embodied abstract action representations. The representations are compositional (c.f. also \autoref{sec:cognitive_background:action_abstraction}, \autoref{sec:cognitive_background:compositional_action_abstraction}). 
    \item \textbf{State abstraction.} \quad Sensorimotor grounding allows for mapping sensorimotor stimuli to abstract semantic state representations. 
    \item \textbf{Compositionality of abstract representations.} \quad The abstract state- and action representations are composed by sub-representations, and there exist rules to interpret the combination of sub-representations (cf. \autoref{sec:hrl:mechanisms:compositionality}). 
    % not necessarily symbolic but necessarily compositional. For example, a partial relational state representation \concept{onTopOf(A,B)} is composed of two arguments \concept{A} and \concept{B} and the relation type \concept{onTopOf}. An action \concept{grasp(object)} is composed of the action type \concept{grasp} and the patient of the action \concept{object}.
\end{itemize}
% The \textbf{computational requirements} for implementing the desiderata in a HRL-based agent are:
% \begin{itemize}
%     \item A sensorimotor grounding function for compositional action representations with temporal abstraction
%     \item A sensorimotor grounding function for compositional state representations with functional abstraction
% \end{itemize}
}

\subsection{Learning transfer and analogical reasoning}
\label{sec:cognitive_background:transfer_analogies}
Intelligent animals are able to transfer solutions between similar problems. For example, 
Research from education theory suggests that human transfer learning improves when explicitly taught to identify analogies between different problems \cite{Klauer1989_AnalogyTransfer}. 
Analogies are determined by isomorphisms between analogous problems from different domains. 
For example, an object transport problem with a robotic hand that involves \concept{[grasp(object),moveArm(goal),release(object)]} is analogous to a file movement problem on a computer that involves \concept{[cutInFolder(file), navigate(targetFolder),pasteInFolder(file)]}, with the obvious isomorphisms between the action types and arguments.

\mybox[black!20]{
% Cognitive and Psychological evidence for transfer learning and analogical reasoning suggests the following desiderata for hierarchical reinforcement learning agents:
\begin{itemize}
    \item \textbf{Transfer learning.} \quad Biological agents are able to identify problem-morphisms and to apply solutions to previously solved problems to new unsolved problems.
    \item \textbf{Learning analogies.} \quad To obtain general high-level state- and action representations that transfer across application domains, it is useful to explicitly foster the learning of analogies and problem-morphisms.
\end{itemize}
}


\subsection{Other mechanisms}
\citet{Colin2016_HRL_as_CreativeProbSolving} draw parallels between creative cognitive models of problem-solving and HRL. In particular, the authors link Boden's creative systems framework (CSF) with option-based HRL. Herein, they associate objects with policies, and describe the learning of policies for problem-solving as exploratory and transformational creativity, which supports the notions of insight and the \emph{Aha!} effect. The authors state that ``When a switch between options occurs on-line, in the course of the search process, transformational creativity occurs - similar to moments of insight in humans or animals.''.



\subsection{Requirements and implications of the above mechanisms}
Throughout this paper, we build on a recent review by \citet{Merel2019_HierarchicalMotorNature}, and consider problem-solving to be based on a form of hierarchical optimal feedback control (OFC). That is, we assume that there exists an intrinsically or extrinsically defined cost or reward function, and the agent strives to optimize its behavior with respect to this function.
Therefore, our study takes for granted that problem-solving is a hierarchical reward-driven process. To this end, we consider mechanisms that specifically related to hierarchical reinforcement learning. 

The mechanisms that we identify in this section imply the following requirements:
\mybox[black!20]{
\begin{itemize}
    \item \textbf{Inverse model.} \quad To select an action, an agent requires a policy (the inverse model) that associates states and goals with actions that lead from the state towards the goal. 
    \item \textbf{Forward model.} \quad Most of the mechanisms discussed so far, namely free energy, plan verification, mental imagery and event segmentation require a forward model to predict how an event or action changes the currently perceived state.
    \item \textbf{Compositional state abstraction.} Learning transfer and analogical reasoning (\autoref{sec:cognitive_background:transfer_analogies}), as well as sensorimotor grounding (\autoref{sec:cognitive_background:grounding}), requires an abstraction function for states and perception.  The abstraction function is temporal, i.e., it maps past and current perception on a lower level to a higher level.
    \item \textbf{Compositional action abstraction.} Learning transfer and analogical reasoning (\autoref{sec:cognitive_background:transfer_analogies}), as well as sensorimotor grounding (\autoref{sec:cognitive_background:grounding}) require an abstraction function for actions and motor commands. The abstraction function is temporal, i.e., it maps past and current motor commands on a lower level to an atomic action on a higher level.
\end{itemize}
}




==> v0/conclusion_old.tex <==
\section{Conclusion}
\label{sec:conclusion}
This review provides an overview about cognitive mechanisms that are deemed to be relevant for problem-solving. 

\subsection{Discrepancies between the cognitive mechanisms of biologial and artificial agents}
The key insight of this review is that current HRL methods have promising potential to realize problem-solving, at least on the level of intelligent animals, such as corvids and primates. However, we also identify a lack of mechanism related to forward models and compositional abstraction. 


\subsection{A unifying proposal for a model-based HRL framework.}


% \subsection{Notes}
% \begin{enumerate}
%     \item \citet{Lesort2018_StateRepLearning} provide a comprehensive overview over state representation learning, which is closely linked to HRL. 
%     \item \citet{Polydoros2017_MB-RL_RoboticsSurvey} provide an overview over model-based RL for robotics.
% \end{enumerate}


Motivation: high sample-efficiency and learning transfer
\begin{enumerate}
    \item Exploit the benefits of forward models (see \ref{sec:cognitive_background}).
    \begin{enumerate}
        \item Mental imagery improves sample-efficiency 
        \item Forward models allow for verification
        \item Forward models improve representational abstraction
    \end{enumerate}
    \item Exploit the advantages of a replay buffer (e.g. for case-based reasoning)
    \item Abstract compositional representations foster learning transfer
    \item Analogical reasoning
    

\end{enumerate}

\subsection{The mechanisms}
The following proposal for a computational framework integrates the mechanisms summarized in \autoref{sec:cognitive_background} to complement existing HRL methods. 

\subsubsection{Basic HRL framework with action abstraction and learning from failures}
As a basic framework we use the hierarchical actor critic (HAC) method with hindsight developed by \citet{Levy2019_Hierarchical}. This framework models action abstraction by representing high-level actions as low-level subgoals. It also allows for learning from failures due to the hindsight resampling. 

The framework essentially consists of several layers $l$, where each layer has an actor $\pi^l: \mathcal{S}^l \times  \mathcal{G}^l \mapsto \mathcal{A}^l$, i.e., an inverse model that suggests goal-directed action, and a critic $Q^l: \mathcal{S}^l \times  \mathcal{G}^l \times \mathcal{A}^l \mapsto \mathbf{R}$ that assesses how good an action is with respect to achieving a predefined goal. 

The framework is optimized for environments with sparse binary extrinsic rewards $r^E_t \in \{-1,0\}$. 

The critic is trained using the temporal difference method, i.e., the optimization criterion is to minimize the error 
\begin{equation}
\label{eq:framework_basic_q_min}
||Q(a_t,s_t,g) - (\gamma r_t + Q(a_t+1,s_{t+1},g))||_2^2
\end{equation}

\subsubsection{Forward model}
We propose to extend each layer $l$ with a forward model $f^l(s_t,a)=\hat{s}_{t+1}$ that predicts the next state $\hat{s}_{t+1}$ given the current state $s_t$ and an action $a_t$.

\subsubsection{State abstraction}

The basic HRL framework defined so far considers action abstraction but it does not consider state abstraction. This is, however, useful to reduce the decision space. Formally, a state abstraction between two successive hierarchical layers $l,l+1$ is a mapping $\phi: \mathcal{S^l} \mapsto \mathcal{S}^{l+1}$, where $\mathcal{S}^l$ and $\mathcal{S}^{l+1}$ are the state spaces of the respective layers. We will train the space abstraction building on \citet{Pathak2017_forward_model_intrinsic}'s proposal to integrate the state abstraction learning with the model learning. 
The authors propose instead of training the forward model $f^l$ to make predictions in the same state space, to train the model to make predictions in the higher-level space. Specifically, this means to minimize the following forward model error:

\begin{equation}
\label{eq:framework_fwd_phi_min}
||f^l(\phi^l(s_t),a_t) - \phi^l(s_{t+1})||_2^2
\end{equation}
and also the inverse model error:
\begin{equation}
\label{eq:framework_inv_phi_min}
||g^l(\phi^l(s_t), \phi^l(s_{t+1})) - a_t||_2^2
\end{equation}

However, the problem here is that fine low-level actions have only a marginal effect, if any, on the high-level state representation.

Therefore, we propose to train the abstraction from the lower-level layer $l-1$ to the current layer $l$ within the $l-$the layer forward model as follows:

\begin{equation}
\label{eq:framework_fwd_phi_min}
||f^l(\phi^{l-1}(s_t^{l-1}),a^l_t) - \phi^{l-1}(s_{t+1}^{l-1})||_2^2
\end{equation}



\subsubsection{Active Inference and curiosity-driven intrinsic rewards}
Using the forward model, we define an intrinsic reward as the error between the predicted next state and the actually achieved next state as follows:
\begin{equation}
\label{eq:intrinsic_reward}
r^{I}_t = ||f^l(\phi^{l-1}(s_t^{l-1}),a^l_t) - \phi^{l-1}(s_{t+1}^{l-1})||_2^2 
\end{equation}

We model the total reward $r_t$ used for the Bellmann update in \autoref{eq:framework_basic_q_min} as a function of the the weighted sum of the extrinsic reward given by the environment $r^E_t$ and the intrinsic reward $r^I_t$. 





A function $\phi$ abstracts from the perceptive input to a high-level object-oriented representation.
In this representation there exist object classes, where each class is constituted by a set of roles. The roles also encode relations to other objects. 
$\phi^{-1}$ maps from the high-level representation back to the perceptive input. Actions $a$ are represented as conditions $cond(a)$ and effects $eff(a)$. 

\subsubsection{Action verification}

\subsubsection{Training by imagination}

\subsubsection{Compositional high-level action representations}

\subsubsection{Compositional high-level state representations}
We suggest to use concatenation of vector embeddings to realize compositional state representations. The asymmetry of the concatenation is a feature, as it allows for plausibly modeling that the order in which concepts are concatenated has an effect on meaning. For example, as \citet{} point out, a \concept{boat house} is different from a \concept{house boat}, and the semantic difference between the concepts is indicated just by the difference in the sequential arrangement of the constituent words. Hence, we suggest to model conceptual representations not in a declarative but a procedural manner (unlike, e.g., in classical AI-based action planning \cite{PDDL}). 

\subsection{Future work}
This article has focused on a temporally minimal account of decision-making, in the sense that we have not explicitly addressed memory. However, by considering hierarchical state abstraction, an implicit account on memory is given. Moreover, in \autoref{sec:conclusion:framework}, we suggest to use recurrent neural networks which implicitly realize a basic emergent form of memory. Elaborating on the role of memory, however, is subsject to future work.

==> v0/framework.tex <==
\section{A model-based hierarchical framework with compositional representations}
\label{sec:framework}

% \subsection{Notes}
% \begin{enumerate}
%     \item \citet{Lesort2018_StateRepLearning} provide a comprehensive overview over state representation learning, which is closely linked to HRL. 
%     \item \citet{Polydoros2017_MB-RL_RoboticsSurvey} provide an overview over model-based RL for robotics.
% \end{enumerate}



\subsection{Motivation}
Goal: high sample-efficiency and learning transfer
\begin{enumerate}
    \item Exploit the benefits of forward models (see \ref{sec:cognitive_background}).
    \begin{enumerate}
        \item Mental imagery improves sample-efficiency 
        \item Forward models allow for verification
        \item Forward models improve representational abstraction
    \end{enumerate}
    \item Exploit the advantages of a replay buffer (e.g. for case-based reasoning)
    \item Abstract compositional representations foster learning transfer
    \item Analogical reasoning
    

\end{enumerate}

\subsection{The mechanisms}
The following proposal for a computational framework integrates the mechanisms summarized in \autoref{sec:cognitive_background} to complement existing HRL methods. 

\subsubsection{Basic HRL framework with action abstraction and learning from failures}
As a basic framework we use the hierarchical actor critic (HAC) method with hindsight developed by \citet{Levy2019_Hierarchical}. This framework models action abstraction by representing high-level actions as low-level subgoals. It also allows for learning from failures due to the hindsight resampling. 

The framework essentially consists of several layers $l$, where each layer has an actor $\pi^l: \mathcal{S}^l \times  \mathcal{G}^l \mapsto \mathcal{A}^l$, i.e., an inverse model that suggests goal-directed action, and a critic $Q^l: \mathcal{S}^l \times  \mathcal{G}^l \times \mathcal{A}^l \mapsto \mathbf{R}$ that assesses how good an action is with respect to achieving a predefined goal. 

The framework is optimized for environments with sparse binary extrinsic rewards $r^E_t \in \{-1,0\}$. 

The critic is trained using the temporal difference method, i.e., the optimization criterion is to minimize the error 
\begin{equation}
\label{eq:framework_basic_q_min}
||Q(a_t,s_t,g) - (\gamma r_t + Q(a_t+1,s_{t+1},g))||_2^2
\end{equation}

\subsubsection{Forward model}
We propose to extend each layer $l$ with a forward model $f^l(s_t,a)=\hat{s}_{t+1}$ that predicts the next state $\hat{s}_{t+1}$ given the current state $s_t$ and an action $a_t$.

\subsubsection{State abstraction}
The basic HRL framework defined so far considers action abstraction but it does not consider state abstraction. This is, however, useful to reduce the decision space. Formally, a state abstraction between two successive hierarchical layers $l,l+1$ is a mapping $\phi: \mathcal{S^l} \mapsto \mathcal{S}^{l+1}$, where $\mathcal{S}^l$ and $\mathcal{S}^{l+1}$ are the state spaces of the respective layers. We will train the space abstraction building on \citet{Pathak2017_forward_model_intrinsic}'s proposal to integrate the state abstraction learning with the model learning. 
The authors propose instead of training the forward model $f^l$ to make predictions in the same state space, to train the model to make predictions in the higher-level space. Specifically, this means to minimize the following forward model error:

\begin{equation}
\label{eq:framework_fwd_phi_min}
||f^l(\phi^l(s_t),a_t) - \phi^l(s_{t+1})||_2^2
\end{equation}
and also the inverse model error:
\begin{equation}
\label{eq:framework_inv_phi_min}
||g^l(\phi^l(s_t), \phi^l(s_{t+1})) - a_t||_2^2
\end{equation}

However, the problem here is that fine low-level actions have only a marginal effect, if any, on the high-level state representation.

Therefore, we propose to train the abstraction from the lower-level layer $l-1$ to the current layer $l$ within the $l-$the layer forward model as follows:

\begin{equation}
\label{eq:framework_fwd_phi_min}
||f^l(\phi^{l-1}(s_t^{l-1}),a^l_t) - \phi^{l-1}(s_{t+1}^{l-1})||_2^2
\end{equation}



\subsubsection{Active Inference and curiosity-driven intrinsic rewards}
Using the forward model, we define an intrinsic reward as the error between the predicted next state and the actually achieved next state as follows:
\begin{equation}
\label{eq:intrinsic_reward}
r^{I}_t = ||f^l(\phi^{l-1}(s_t^{l-1}),a^l_t) - \phi^{l-1}(s_{t+1}^{l-1})||_2^2 
\end{equation}

We model the total reward $r_t$ used for the Bellmann update in \autoref{eq:framework_basic_q_min} as a function of the the weighted sum of the extrinsic reward given by the environment $r^E_t$ and the intrinsic reward $r^I_t$. 



\subsubsection{With compositional state and action abstraction}


A function $\phi$ abstracts from the perceptive input to a high-level object-oriented representation.
In this representation there exist object classes, where each class is constituted by a set of roles. The roles also encode relations to other objects. 
$\phi^{-1}$ maps from the high-level representation back to the perceptive input. Actions $a$ are represented as conditions $cond(a)$ and effects $eff(a)$. 

\subsubsection{With verification}

\subsubsection{With training by imagination}

% \subsection{Theoretical evaluation}

% \subsubsection{Representational abstraction and discretization simplifies the decision space}

% \subsubsection{Forward models enable compositional representations}

% \subsubsection{Forward models allow for verification}

% \subsubsection{Compositionality simplifies the representational space and improves transferability}
% Argue with vocabulary size. 

% \subsubsection{}

==> v0/hrl.tex <==
\section{Computational Mechanisms in Hierarchical Reinforcement Learning}
\label{sec:hrl}

First approaches: Sutton 1999, Dietterich 2000, Barto and Mahadevan, 2003

There is clear evidence that human and animal problem-solving behavior builds on hierarchical cognitive processes \cite{Merel2019_HierarchicalMotorNature}. Therefore, we our study focuses on hierarchical reinforcement learning. 


\subsection{Background}

\subsubsection{Hierarchical Reinforcement Learning}
Reinforcement learning is defined in terms of hierarchical Markov Decision Processes (MDP). A single (shallow) MDP is determined by a 4-tuple $(S,A,P_{a},R_{a})$. 
Herein, $S$ is a set of states, $A$ is a set of actions, $P_{a}(s,s')=Pr(s_{t+1}=s'| s_{t}=s,a_{t}=a)$ is the probability that action $a$ in state $s_t$ leads to state $s'$, and $R_{a}(s,s')$ is the immediate reward received after transitioning from $s$ to $s'$ by performing action $a$.

Hierarchical reinforcement learning is defined in terms of hierarchical MDPs. We illustrate a general HRL model in \autoref{fig:hrl}.
The objective is to learn hierarchy of policies that maximize a function over cumulative rewards during a finite number of discrete state transitions.
The policy of the $l$-th hierarchical layer, denoted $\pi^l$, maps a state representation $s$ to an action $a^l$. 
% A universal policy maps a state $s$ and a goal $g$ to an action $a$. 
The action $a^l$ is a sub goal or sub behavior to be achieved by the lower-level $\pi^{l-1}$ policy, except for the lowest level where $a^0$ is a motor command. 

\begin{figure}
    \centering
    %trim={<left> <lower> <right> <upper>}
    \includegraphics[width=\textwidth,trim={0pt 0pt 0pt 150pt},clip]{pics/HierarchicalArchitecture.pdf}
    \caption{A general hierarchical problem-solving architecture with multiple layers of abstraction.}
    \label{fig:hrl}
\end{figure}

Throughout this paper, we refer to states $s_t$ as the state of the agent's sensor readings a discrete time $t$ if not specified otherwise. Note that this view is agnostic to whether or not the agent's environment is fully observable by the agent.


\subsection{Hierarchical Reinforcement Learning Approaches (temporary section)}
\label{sec:hrl:approaches}
{\color{gray}
This section is supposed to summarize all papers that we go through individually. For our collaborative work, it is easiest to do this paper by paper, or in aggregates of similar papers.
However, a goal of this paper is to directly bring the reader to the point that we want to make, i.e., the effects and benefits of the individual mechanisms. 
Therefore, this section will be removed later, and, instead, its ingredients will be compiled into subsections for the different mechanisms in \autoref{sec:hrl:mechanisms}. In other words: we will now structure everything paper-by-paper because it is easier to coordinate our work this way, and later we will restructure by mechanisms.}

\subsubsection{Not categorized}

\citet{Rasmussen2017_NeuralHRL} set a focus on neural plausibility. Their novelty is a spiking-based (leaky integrate and fire (LIF)) neural network model for hierarchical TD-learning. The author's model is quite exotic in the sense that it builds on continuous time, and not on discrete time representations. The framework is very general, and the authors present its function with some simple benchmark environments. 

\citet{Tessler2017_LifelongHRLMinecraft} present a lifelong learning approach to Minecraft where the agent acquires skills that can be re-used. These skills are implemented in a deep skills network. 


\citet{Han2019_hierarchicalSelfOrga} present \emph{Recurrent Multi-timescale Actor-critic with STochastic Experience Replay} (ReMASTER), an approach that focuses on using recurrent neural networks for hierarchical reinforcement learning. The approach features compositional action hierarchies through Multi-Timescale RNNS. However, the action representations are only temporally compositional. 

\citet{Rafati2018LearningRepresenations} propose a model-free method based on DQN. Their main contribution is the extension of this method with a clustering algorithm that supports unsupervised subgoal discovery. 

\citet{Ma2020_MultiAgentHRL} focus on decentralized multi-agent hierarchical reinforcement learning. The authors address the curse of dimensionality by subdividing the environment into sub-environments and regions.
This implies state abstraction, but not strictly in a compositional sense. 


\citet{Isele2016_FeatureZeroShotTransfer} focus on lifelong learning and knowledge transfer using task features. 
High-level tasks are expressed as coefficient vectors that are transferable among different problems. 
A task $\mathcal{Z}^(t)$ has a descriptor $m^{(t)}$ that is given to the learning low-level agent. 
The descriptor is represented by a feature vector $\phi(m^{(m)})$ where $\phi$ performs feature extraction. Each task has associated training data $\mathcal{X}^{(t)}$. There exists one policy $\pi^t$ per task, determined by parameters $\theta^t$. $\theta^t = L ~ s^t$, where $L$ is a shared basis over the model space and $s^t$ are sparse coefficients over the basis.
Another shared basis over the descriptor space $D$ determines $\phi$, i.e., $\phi(m^t) = D~s^t$.
Since the factored representations are composed from their coefficients, the high-level task descriptions could be considered as inherently compositional. However, it is unclear in how far the coefficients are interpretable, e.g., in a similar manner as the latent representation of variational autoencoders \cite{Higgins2017_B-VAE}. 
The approach allows transferring learned dynamics between different tasks within the same domain, e.g., for simulating different quadcopter controllers. 

\citet{Dietterich1999_MAxQ} present the MAX-Q approach to HRL, which has a focus on state abstraction \cite{Dietterich2000_StateAbstraction_MAXQ}. Herein, the state abstraction is implemented as an attention mechanisms that hides information that is not relevant for a certain sub-task. State abstraction is realized by removing those variables from the observation space that meet one out of five conditions that the authors refer to as 1) Subtask irrelevance, 2) Leaf irrelevance, 3) Result distribution irrelevance, 4) Termination, 5) Shielding. For example, in a passenger delivery domain, 1) eliminates the variable <destination> when executing the pick-up action of a passenger, since the destination is irrelevant for the pickup. The main contribution of the author's work is to demonstrate that the MAX-Q approach for HRL converges, also when using the proposed state abstraction. 


\citet{Jiang2019_HRL_Language_Abstraction} focus strongly on abstraction and compositionality in HRL. Natural language is a medium that heavily relies on these principles, which motivates the authors to use it as an abstract representation for goals and states. Specifically, the authors use language as an interface between low- and high-level policies. 
Herein, high-level actions are specified in the space of language, which ensures that the high-level actions are compositional. 
In an ablation study, the authors show that the HRL approach significantly benefits from the compositional representations. The authors ``find that our instruction-following agent is able to generalize to instructions that are systematically different from those seen during training.''.
To improve the efficiency of their approach, the authors us a goal relabeling strategy, inspired by the hindsight experience replay (HER)  method \cite{Andrychowicz2017}. 

The authors assume that there exists a mapping $\omega(g|s)$ that generates a distribution of natural language descriptions $g$ from a state $s$. They do not learn it. Also, even though the representation of the high-level actions is compositional, their generation is not. That is, the high-level actions are specified in the compositional space of language, but the policy is based on a DQN that selects one action out of 40 (or 400 for the visual representation) without actually composing the action. 


\citet{Akrour2018_RL_StateAbstraction} present an approach that explicitly proposes state abstraction as a means to improve the decision-space of high-level policies. Their approach is based on clustering. The authors propose a partitioning policy $\pi_p(c|s)$ that selects a state cluster $c$ given a state $s$, and a cluster-specific policy $\pi_c(a|s)$. 
The cluster-specific policy considers not only the state cluster but also the state, allowing to adapt the cluster-specific policy to the specifics of a state within a cluster. However, the state representation itself is not compositional. The authors do not mention transfer learning, i.e., they do not fully exploit their state abstraction. 



\citet{Saxe2017_HRL_Multitask_LMDP} define concurrent multitask linear MDPs (MLMDPs)to break down complex problems into a set of concurrently executable optimally compositional sub-problems. 
A high-level scheduling policy determines the subtasks. 
Each of the subtasks can be understood as temporal action abstractions. In addition, the approach also performs state abstraction by defining boundary states that cause the system to transition into the higher-level layer. However, the representations remain in the same representational space for all layers and the transition matrix that controls the state abstraction is manually defined. 



\citet{Hejna2020_HRL_Imitation_MorphologicalTransfer} propose a method for morphological transfer that enables to transfer policies between different robots. The authors propose a two-layered HRL agent where the high-level layer is universal for all morphologies and the low-level layer unique for each robot. The two different layers take as input different state representations. The high-level layer uses a morphology-independent state representation (base on a simple point mass), and the low-level layer a morphology-specific representation (based on a four-legged ant agent).
This simple form of transfer already shows moderate success for morphological transfer. 
When incentivizing the low-level policy of a complex agent to imitate the behavior of the corresponding policy of a simple agent, their system shows good performance for zero-shot high-level policy transfer. 
This performance can be further improved by finetuning (retraining) the high-level policy. 
\citet{Hejna2020_HRL_Imitation_MorphologicalTransfer} also demonstrate how KL-regularized training can be used for finetuning to additionally avoid catastrophic forgetting, a common problem when retraining a policy after task/morphology transfer.


% TODO CG: Does it make sense to maybe add a subsection about these Mixture-Of-Experts type of approaches? Something like the following approach, or what we did with SUBMODES, where you have a state or task space decomposition based on different forward and/or inverse models?
\citet{Wu2019} consider the problem of task decomposition and how this may improve lifelong reinforcement learning and task transfer.
They presuppose the existence of a set of simple forward models, or \emph{model primitives}.
Closely related to the mixture-of-experts framework \cite{Masoudnia2014}, each model primitive is specialized for a certain area of the environment.
Given this decomposition of the environment in terms of forward models, they decompose the task at hand accordingly: For each forward model an associated subpolicy is trained.
A gating mechanism weighs how much a single subpolicy contributes to the executed action, based on the relative prediction error of the associated forward model.
\citet{Wu2019} show that this task decomposition is not only effective for solving high-dimensional control tasks, but the forward models defined for one task also helps their system to learn useful subpolicies in a related but somehow different task.

\citet{Shankar2020_MotorPrimitives} present an approach to decomposition demonstrated trajectories into sequences of motor primitives, or action abstractions. 
They use an encoder-decoder approach where one component encodes a trajectory into a sequence of hidden states  while another component reconstructs the trajectory from the encoded sequence of latent states. 
By additionally enforcing some soft constraints, such as incentivizing few numbers of primitives per sequence and simplicity of the encoded motion per primitive, they learn various realistic motor primitives from demonstration.
Furthermore, they show that such an approach can be used within a hierarchical RL framework, where a high-level policy outputs a sequence of motor primitives, and the decoder-part of their system produces low-level actions given the sequence of primitives.

\citet{Yamamoto2018_RL_Planning} propose a hierarchical reinforcement learning method based on symbolic abductive planning. The main advantage of the approach is, in contrast to integrating classical symbolic planners into reinforcement learning, the ability of the abductive planner to choose different high-level goals based on the observations in the environment. 
A discrete, simulated grid-world environment (inspired by Game Minecraft) is used to evaluate the approach. The environment is partially observable and features delayed, sparse rewards, and multiple goals. In the environment, the agent can move around, gather, and combine resources and avoid certain objects (lava fields). Due to the random initialization of the environments, not all possible goals (object combinations that yield different rewards) are reachable.
The abductive planner decides on the most profitable goals, based on the agent's observations, by integrating the extrinsic reward for different object combinations into the evaluation function that rates possible abductions. The sub-goals of the symbolic plans, based on these abductions, serve as goals for the low-level reinforcement learner, which is realized with Proximal Policy Optimization (PPO) with a reward signal from the abductive planner. The authors compare their approach to a non-hierarchical RL algorithm and a hierarchical RL algorithm with a symbolic planner without abductions (i.e., a planner can not plan for different high-level goals based on the observations in the environment). They show that their approach improves learning efficiency in terms of sample efficiency.

\citet{Ghazanfari2017_AssociationRules} use the principle of Association Rule Mining (ARM) to extract relevant subgoals from action sequences and arrange them in a hierarchical graph, thus achieving an automatical and unsupervised task decomposition. The approach can be applied to discrete single as well as multi-task scenarios. The algorithm works in two steps: after an initial exploration phase, where a normal q-learner explores (and exploits) the environment, the trajectory of visited states is represented as a transaction in terms of ARM, and all visited states of successful trajectories form the itemset. Association rules, in this case, rules that describe which states follow each other in successful trajectories, are rated according to support and confidence, measuring the relevance and reliability of the found rules. Rules above a given threshold are then composed into a hierarchy in a second step. In the case of a large number of (similar) states, these states can be clustered to further reduce the complexity. The approach is successfully evaluated in different grid-world scenarios without and with multiple tasks and achieves a speedup compared to a q-learning baseline. The approach works with any discrete RL algorithm; the authors chose a non-neural q-learner for their experiments.

\citet{Lample2018_PlayingFPSGames} propose a hierarchical, recursive deep-q learning approach for a first-person shooter (FPS) game in a three-dimensional environment. They extend the deep q-learning by introducing \emph{co-training}, instead of only using raw pixel input to train the neural networks, semantic, high-level information about the presence of objects in the visual input of the agent is used. The purpose of the LSTM-based architecture is to compensate for the partially observable environment. The training procedure is modified, by sampling a sequence observations from the replay memory and only updating on the last few observations, as the earlier ones do not have sufficient history. The architecture is hierarchically split into two independent components for the navigation phase(exploration of the map, collecting items, and finding enemies) and the action phase (fighting enemies). Hardcoded rules enable the switch between the sub-networks depending on the state of the game. Finally, reward shaping is used to create a dense-reward environment. During the evaluation, the approach outperformed human players.

\citet{Li2020_SubPolicy} present a hierarchical extension to Proximal Policy Optimization (PPO \cite{schulman2017proximal}), called Hierarchical Proximal Policy Optimization (HiPPO), that allows on-policy training of simultaneous training of all hierarchy levels. 
Herein, a master policy selects sub-policies.
The approach addresses a challenge in transfer learning with hierarchical  RL-architectures, where traditionally only the higher levels are retrained without adapting the pretrained sub-policies to a new task. The training is based on decoupling manager, the high-level and low-level) gradient by modeling the high-level decision as part of the low-level observation. Like in related approaches, high-level updates happen slower than low-level updates, only every n time steps. However, the number of steps between updates is randomized between a lower and an upper limit, randomizing the time commitment to specific sub-policies, which could be shown to help with zero-shot adaptation. The approach was evaluated in high dimensional continuous simulation environments using hopper, ant, cheetah, and snake models for locomotion and navigation tasks. HiPPO outperforms non-hierarchical (PPO) and state-of-the-art hierarchical RL algorithms (\cite{Nachum2018_HIRO, Bacon2017_OptionCritic, Frans2017}. Additionally, the adaptation of pretrained skills, generated with DIAYN (\cite{Eysenbach2019DiversityFunction}) outperforms PPO with fixed sub-policies.

\citet{Frans2017} introduce Metalearning Shared Hierarchies (MLSH) for learning hierarchically structured policies. The goal of the algorithm is to generate shared sub-policies (primitives) that allow a sample-efficient adaptation to unseen tasks. MLSH is based on the idea of a task-specific high-level (master) policy and a set of shares low-level policies. The low-level policies should both be fine-tuned to specific tasks but also robust to transfer and diverse.  Fast learning of these sub-policies is enabled by repeated resetting of the high-level policy. In detail, the training cycles are divided into two phases: in the warm-up phase, only the high-level policy is optimized to select a good sub-policy. This selection is modeled as a single action and the next N time steps in which the sub-policy is executed are modeled as a single transition in the environment. Next, in the joint update phase, both high and low-level policies are optimized:  A set of experiences is collected, and the high-level policy updated in the same way as during the warm-up phase. The same experiences are then reused to update the sub-policies by modeling the decision of the high-level policy as an extension of the environment, i.e., adding the output of the high-level policy to the agent's observation. Only the sub-policy that is selected by the master-policy is updated. After a predefined number of training steps, a new task is chosen,  the master policy is reset, and the training cycle is repeated. MLSH was evaluated on different simulated environments ranging from discrete two-dimensional environments with sparse rewards to continuous three-dimensional environments with dense and sparse rewards (walker, four-legged ant). PPO (\cite{schulman2017proximal}) was for the experiments, however other RL algorithms (both on-policy and off-policy) are assumed to work as well. MLSH was shown to outperform the PPO and Option Critic \cite{Bacon2017_OptionCritic} baselines. Moreover, MLSH could learn complex sparse-reward tasks by transferring low-level policies from previous tasks.

\citet{sharma2019dynamics} present a two-phase HRL approach that combines unsupervised model-free learning of primitives with model-based learning and planning. The proposed algorithms, Dynamics-Aware Discovery of Skills (DADS), focuses on the discovery of diverse but also predictable primitives in continuous skill spaces. The approach enables zero-shot planning in the learned latent space. DADS is based on mutual-information-based exploration. More precisely, during the initial unsupervised learning phase, the mutual information of the next state s0 and current skill z conditioned on the current state s is maximized. In turn, this maximizes the diversity of transitions produced in the environment while turning z into a good predictor of the next state. Entropy regularization clusters action-sequences with similar state-transitions into one skill. This part of the presented approach is similar to DIAYN \cite{Eysenbach2019_DiversityFunction}. At test time, the approach realizes model-based zero-shot planning in latent space (the skills Z) using model predictive control. At each time step, plans are generated, and the optimal plan with regard to a reward function is chosen, and its first step is executed before the replanning cycle begins anew. In contrast to traditional model-predictive-control, plans are created in the latent space, not in the action space. Therefore each planning step is a skill (not an action), which in turn creates longer plans wich fewer steps. The approach is evaluated in the high-dimensional continuous simulation environment MuJoCo (walker, four-legged ant, half cheetah - all of which develop stable gaits without supervision). The unsupervised learning phase of DADS generates primitives which are optimized for diversity (like DIAYN) but also for the predictability. In comparison to DIAYN, the resulting primitives show a smaller variance, i.e., after a given amount of time steps, the positions of an agent in the environment following one skill show less variance. This quality is essential for planning and temporal compositionality. As a result, DADS is able to outperform hierarchical DIAYN in a four-legged ant navigation task.

\citet{heess2016learning} present an end-to-end learning approach for locomotion task based on a two-level hierarchical approach. The low-level "spinal" network uses only proprioceptive sensors for learning sensorimotor primitives, while the high-level "cortical" network uses all sensors. The approach is evaluated in a continuous high dimensional simulation environment on different models (swimming snake, quadrupled walker, humanoid). The approach focuses on combining the advantages of a high-frequency closed-loop motor controller and a low-frequency, recurrent, high-level controller for complex tasks in reward-sparse environments, which is inspired by biological models. The algorithm is realized with on-policy training of a policy gradient framework with hierarchical noise, i.e., noise on both the output of the high-level and the low-level controller, with the high-level noise held constant during high-level iteration. The training is organized in two phases: Pre-training with a simple task is used to train controllable low-level controllers, using a provisional high-level controller that will be discarded. This phase develops basic locomotion skills by rewarding moving from a random position to another random position in the environment using reward shaping (dense rewards). In the transfer phase,  more complex tasks with sparse rewards are learned. The low-level controller is no longer updated, but a new high-level controller is trained. Compared to non-hierarchical baseline end-to-end learning, the complex tasks could be solved.

%Not hierarchical in the typical sense
\citet{ghosh2017divide} present Divide and Conquer Reinforcement Learning (DnC), an RL approach based on dividing the initial state space into "slices" and training independent policies that are iteratively integrated. Though not hierarchical in the traditional sense, the iterative integration of policies can be seen as creating an implicit hierarchy. The approach is designed towards environments with a high variance in start or goal states, which can induce high variance policy gradient estimates, complicating effective learning. DnC does not use high-level action representation; however, it can solve complex, continuous tasks (grasping, catching) in the low-level torque action space. The algorithm implemented using k-means clustering to partition the initial states using Trust Region Policy Optimization (TRPO, on-policy). Similar to hierarchical approaches like DIAYN, sub-policies that are enforced to be diverse, using the KL divergence. During the construction of a unified policy, intermediate supervised distillation steps help share information between the local policies. The approach has been positively evaluated on complex, continuous tasks (grasping, manipulation, and locomotion) simulated environments.

%Not hierarchical in the typical sense
\citet{barreto2017successor} present a transfer framework for scenarios with a changing reward function in a constant environment with regard to the environment's dynamics. The approach decouples the dynamics of the environment from the rewards by using successor features as a value function and by extending the algorithm for policy improvement from a single policy to a set of policies. The underlying idea is to use knowledge about the dynamics of the environment from a wide range of subtasks, where the sub-tasks vary only in terms of the reward function. Several, also biologically plausible, scenarios for this are given, e.g., the search for food, water and other resources depending on the agent's hunger and thirst. The approach implemented on the basis of Q-learning and DQN (off-policy) and positively evaluated in a simulated environment navigation task and a two-joint robot arm control task. The approach is not hierarchical in the strict sense that there is a low-level and a high-level controller; however, the idea to decouple learning the environment's dynamics from the task-specific reward can also be seen as a hierarchy.

%Not hierarchical as a contribution but evaluated on HIRO
\cited{quereshi2020composing} present an approach for transferring and composing task-agnostic skills using an encoder-decoder architecture. Based on a finite set of primitive policies (skills), a compositional MDP is defined by introducing a compositional state as the cross-product of the actual state and outputs of the different primitive policies. The architecture that generates a weighted mixture of the primitive policies consists of three components: The encoder produces a latent representation of the learned skills, from the outputs of the primitive policies. The encoder is realized as a bidirectional recurrent neural network using LSTM units. The input to the decoder input are the latent skill representations and current state of the environment. The decoder is realized as a feed-forward network and outputs a parameterization for the attention network. Finally, the attention network outputs a probability distribution over primitive policies as a mixture of wheigts. 
The approach is trainable with RL and HRL methods, for the later HIRO \cited{Nachum2018high} was used, where the low-level policies are replaced with the presented composite policy. The approach was evaluated in simulated 3d environments, using different continuous control tasks like the ant maze with complex push tasks, half-cheetah, and simulated robotic arm push task. The subset of more complex tasks (ant navigation in a complex maze, sometimes requiring push sub-tasks to reach the goal) was evaluated using the HIRO baseline in comparison to HIRO with composite low-level policy. It could be shown that the presented approach outperforms baseline. While not directly a hierarchical approach, the presented methodology is relevant as it can enhance the performance of other hierarchical approaches.



\subsubsection{Soft hierarchies}
\citet{Haarnoja2018_LatentSpacePoliciesHRL} develop a method that, unlike all other categories enlisted here, proposes a `soft breakdown' of high-level problems to lower hierarchical layers. The authors' idea is to allow even the lowest layer to be able to solve a problem on its own, and if it is unsuccessful, at least reduce the workload for the next higher level. This implies that the high-level problem description is provided directly to all hierarchical layers.  To realize this, the authors use latent variables that serve as communication channels between the individual layers. Herein, the latent variables of the lower-level represent the action space for the higher level. 
Each layer can either be trained through the external reward or a manually shaped reward for a subtask.

%Learning Modular Neural Network Policies for Multi-Task and Multi-Robot Transfer





\subsubsection{Hierarchical actor-critic (low-level actions as subgoals)} 
Actor-critic architectures consist of an actor $\pi(s,g)=a$ that maps states and goals to actions, and of a critic $q(s,a,g)$ that estimates the expected cumulative return when $a$ is executed in $s$, given a goal $g$. The hierarchical actor-critic methods investigated here are characterized by the fact that high-level actions correspond to subgoals to be achieved on the next lower layer.


\citet{Levy2019_Hierarchical} present an actor-critic approach on hierarchical reinforcement learning. With the off-policy approach, actions are represented as subgoals in the low-level perceptive space. The perceptive space is provided by a simulated robotic environment and consists of object locations, rotations and velocities. The approach builds on the deep deterministic policy gradient (DDPG) \cite{Lillicrap2016_DDPG} approach, extended with Hindsight Experience Replay (HER) \cite{Andrychowicz2017}, action replay and goal replay. The replay mechanisms allow the agent to learn in hindsight which subgoal has been achieved. This densifies the reward signal, because even if a subgoal is not achieved, the agent gets rewarded for what it has achieved. This is realized by pretending in hindsight that the actually achieved state is the goal that it was supposed to achieve. 
\citet{Beyret2019} also employ DDPG and HER for learning a hierarchical actor-critic structure, where a high-level policy produces subgoals for a low-level policy. 
Crucially, they additional employ a form of curriculum learning when using their replay buffer, where initial subgoals are sampled in proximity to current states to speed up the learning  progress.
\citet{Nachum2018_HIRO} present a similar approach to \citet{Levy2019_Hierarchical}, but without experience replay. Instead, the approach includes also a correction algorithm for the high-level policy. This is motivated by the fact that when the low-level policy improves, the high-level policy should be corrected.


\citet{Oh2017_Zero-shotTaskGeneralizationDeepRL} present an actor-critic approach that is based on learning multiple sub-tasks. The sub-tasks are transferable among different problem domains because the agent also learns analogies between the sub-tasks. This is realized with simple compositional task embeddings. For example, let [Visit X] : [Visit Y] :: [Pick up X]: [Pick up Y] denote the analogy between sequences of visit and pick actions, then the embeddings allow the agents to anticipate novel combinations like [Pick up Y] : [Visit X]. Note that this implies a discrete and compositional high-level action space. 

The approach by \citet{Oh2017_Zero-shotTaskGeneralizationDeepRL} has been extended in a later paper \cite{Sohn2018_Zero-ShotHRL}. Here, the high-level layer is implemented as a Neural Subtask Graph Solver, i.e., a softmax policy, that reasons over the preconditions, costs and rewards of subtasks to infer the optimal path over subtasks. As in the previous work, the high-level action representation is compositional, which enables one-shot learning and learning transfer. 

\citet{Yang2018HierarchicalControl} extend the deep deterministic policy gradient algorithm--DDPG~\citep{Lillicrap2016_DDPG} to a hierarchical algorithm--h-DDPG, aiming to enable agent to learn basic and compound skills simultaneously in a two layer architecture (of hierarchy). The first layer consists of one actor and multiple critics corresponding with multiple basic skills, while the second layer hosts a meta critic which learns compound skills for compound tasks by choosing the basic skill with highest value from a given set of basic skills. This design implies the close similarity between different compound tasks. Furthermore, dedicated reward function needs designing for every single basic and meta critics. It is worth noting that both layers share the same pre-processing convolution network for visual input. 

For the multitask setting, \citet{wulfmeier2020compositional} develop a novel hierarchical and compositional actor-critic algorithm, Regularized Hierarchical Policy Optimization--RHPO, where the hierarchical policy supporting shared sub-policy across tasks. In other words, only the high-level part of the hierarchical policy is conditional on the task information, whereas the low-level part aims to learn general and task-independent behaviors. Furthermore, authors define high level policy as a categorical distribution over low level Gaussian policies. The target hierarchical policy is optimized by applying policy improvement step through a temporal non-parametric and structure-independent policy, which is constraint wrt the target parametric policy (under the KL divergence).

\citet{Eysenbach2019DiversityFunction} use the maximization of an information-theoretic objective (maximum entropy policy) for learning skills for an intrinsically motivated agent without a reward function. Among other applications in imitation learning or adaptation to novel tasks, these skills can serve as primitives for hierarchical reinforcement learning in reward-sparse environments.
The learned skills should be distinct and explore large parts of the state space. This is achieved by using discriminability between skills as an objective during learning. Formally, the set of skills can be represented as a mixture of policies whose entropy can be maximized. The approach is implemented with a soft actor-critic and successfully evaluated on various tasks ranging from simple 2d navigation, inverse pendulum, and mountain car to continuous control tasks like half-cheetah, hopper, and quadrupled walker in simulated 2d and 3d environments.


\subsubsection{HRL approaches with a focus on zero-shot problem-solving and transfer-learning}
Only a few recent HRL approaches are specifically tailored towards one-shot and zero-shot problem-solving, similar to the initial crow-example of this paper (\autoref{fig:crow_probsolving}). For example, 
\citet{Oh2017_Zero-shotTaskGeneralizationDeepRL} present a method where an agent learns to execute instructions in a first-person discrete-space virtual environment, similar to Mine Craft. Instructions are solvable by a low-level layer. In this paper, it is remarkable that the instructions given as compositional representations. There are multiple action types, including Visit, Pick up, and Transform. Each of the actions is realized as a parameterized skill \cite{daSilva2017_parameterizedSkills}. In this case, it has an argument and an integer value. The arguments are objects in the environment, which leads to instructions like  ``Pick up three sheep''. Due to the compositionality of the parameterized skills, the low-level agent is able to execute high-level instructions that it has never seen before. 

\citet{Sohn2018_Zero-ShotHRL}

\subsubsection{Object-oriented RL}
Object-oriented RL (OORL) is specifically tailored to realize compositional state-space abstraction. The approach has been most influenced by \citet{Diuk2008_OORL}, who propose a deictic approach where objects are assigned to a class, and each class is determined by a specific finite set of attributes. Each object instance then has values assigned to the attributes. A state representation is the union over all object instantiations. This state-space representation is very similar to compositional linguistic schema representations \cite{Feldman2009_ECG} and mental concept representations \cite{Eppe2018_AIJ_Blending}. 

Recent approaches to implement OORL include the model-based approach by   \citet{Keramati2018_FastExploreOORL}, who assume an object detector that processes a visual domain representation of an Atari game to provide a list of object with their attributes. The authors train a forward model that operates on the state-space representation resulting from the object detector. They implement a surprisal-based policy that uses an optimistic Monte Carlo Tree Search method to optimize exploration. 

\citet{Watters2019_CobraOORL} present an OORL approach called COBRA, where a visual abstraction based on a variational autoencoder encodes the state space as a set of objects where each object belongs to a certain object class with class-specific attributes. In this work, objects are geometric shapes, and the approach is designed for actions that can affect only one object at a time. Like \citet{Keramati2018_FastExploreOORL}, the authors use a forward model to implement curiosity. However, instead of using the forward-prediction loss here they use a prediction of the prediction loss to generate rewards for an exploration policy. 

\citet{DaSilva2017_MOO-MDP} present an approach for multi agent OORL. They use a state representations based on objects hat are instances of attributed classes, similar to most other OORL approaches. However, in their approach, an agent is itself an abstract class, which leads to a reduced state space size. The application is a discrete-space grid world environment.  

\citet{Costa2018_OORL_Curriculum} present an approach for object-oriented curriculum generation. The curriculum is generated under the assumption that smaller tasks with less objects are easier to learn. 

The object-oriented approach by \citet{Zhu2018_OODynamicsPredict} is strictly speaking not reinforcement learning, but focuses on object-oriented dynamics prediction. The framework first runs a visual object detector on the input data stream and then learns the dynamics of the relations between the objects. In their approach, object boundaries are represented as masks over the perceived input, so essentially by an attention mechanism. 

Even though the abstract state representation that OORL features makes it very suitable for transfer learning, only \citet{Marom2018_Zero_shotTransOORL} empirically investigates transfer learning empirically in an OORL context. Herein, the transfer is between two environments within the same domain but of a different size, hence no far transfer is happening. 
\citet{Costa2018_OORL_Curriculum} touch the topic of transfer learning as well, but focus more on the transfer of curricula, i.e., they do not perform an empirical study to transfer skills. 



\subsubsection{Methods based on options}
Options framework has been introduced by \citet{Sutton_1999_options}. An option is a temporally limited behavior, such as picking up an object, going to lunch, etc. The framework is, therefore, a natural starting point for developing hierarchical methods where complex behaviors must be broken down into simpler ones. 
\citet{Bacon2017_OptionCritic} extend the method with an option-critic approach that learns not only the options but also their termination conditions. This implements temporal action abstraction, but the authors do not mention state abstraction. 
% 

The h-DQN approach by \citet{Kulkarni2016_HDQN} is also based on the options framework. It involves goal abstraction, as it allows to model subgoals as spatial relations like \emph{on top of}. However, the authors leave open how exactly such relations are abstracted from the perceptive input, such as the visual state-representation obtained from the Atari Game environment in which the authors evaluate their approach. 
The high-level layer of the agent operates on a non-compositional discrete action space over options. The high-level state representation is object-oriented and, therefore, compositional. During an exploration phase, the agent 

\citet{Machado2017_PVF_Laplace_OptionDiscovery} present a method based on proto-value functions to learn options, i.e., to temporally abstract actions. This involves also a state abstraction function $\phi$ which learns features of the state-space. The abstraction function governs the policy selection indirectly because it is used for the computing rewards.
Furthermore, the abstraction is used to generate intrinsic rewards, determined by \emph{eigenpurposes} of options. That is, each option has a purpose (such as moving into a specific room). This is realized by using proto-value functions over the abstract state space. 

\subsubsection{Approaches based on auxiliary tasks}
Auxiliary tasks are similar to options. However, often the auxiliary tasks are defined implicitly by domain-independent reward function. 

\citet{Riedmiller2018_SAC-X} present an approach based on scheduled auxiliary control (SAC-X). The framework specifically addresses sparse rewards by modeling domain-independent intrinsic auxiliary rewards in addition to external rewards. Each reward is assigned to a low-level auxiliary behavior policy, called intention. A high-level scheduler learns to control the selection of the policies. The approach is off-policy and does not use a forward model. Strictly speaking, the scheduler is not a policy in the sense that it considers the current state as input but the previous high-level task (cf. Eq. (6) and paragraph below). It is unclear how exactly this works. 

\citet{Riedmiller2018_SAC-X}'s method is similar to the work by \citet{Cabi2017_intentionalunintentional}, who learn several control tasks simultaneously. Both approaches do not use explicit abstract state representations. However, \citet{Cabi2017_intentionalunintentional} perform an interesting implicit state abstraction in the sense that it defines rewards based on a formal language that allows for conjunctions of propositional facts. As an example, consider an auxiliary task that is driven by the subgoal that one object must be in a \emph{near} relation with another object. That is, the goal representations are abstract but the state representations are not. The work by \citet{Cabi2017_intentionalunintentional} is also interesting because the action abstraction is compositional: Instead of executing one high-level action at a time, the agent continuously executes a composition of multiple low-level tasks generated by multiple policies. A result of the authors is that the learning performance grows with the number of simultaneously composed tasks. It is, however, unclear how the method selects the high-level tasks to be executed, or whether all are only learned at the same time. 
The Work by \citet{Cabi2017_intentionalunintentional} is not a hierarchical method because it does not 

%(Arulkumaran2017_Classifying_Optionf_for_Deep_RL, not in .bib file)
Arulkumaran et al. combine the options framework with deep Q-networks. Their architecture is adapted from multi-task learning with DQNs: A shared convolutional part of the architecture extracts a state representation from raw pixel data; different option heads, consisting of dense layers learn the policies for sub-actions while a supervisory network, using the same convolutional input and dense layers, decides on the option head to use in a given situation. The work is evaluated on the computer game catch, where dropping balls of different colors have to be caught or avoided. The authors show that in a negative transfer task (one ball has to be caught, one has to be avoided), their architecture outperforms a standard DQN in terms of sample complexity. A limitation of the approach is that for training the option heads, an oracle is used so that only the right head is trained for a given option.


%Schaul2013_Better_Generalization_with_Forecasts (missing in .bib)
\citet{Schaul2013_Better_Generalization_with_Forecasts} evaluate the generalization ability of the state representation mechanism \emph{Forecasts, aka. (General Value Function or GVF)} in comparison to \emph{Predictive State Representations (PSRs)}.
Both mechanisms represent states as a set of \emph{features (called
tests)} that are predictions about future observations
resulting from a sequence of actions. The difference between the mechanism is that \emph{PSRs} use a fixed sequence of actions while 
\emph{Forecasts} use an \emph{option} that is then realized by a low-level controller. Schaul and Ring use two discrete grid world scenarios to evaluate the generalization. These environments are characterized by the fact that the agent's immediate sensory feedback is often insufficient to localize the agent. As the evaluation focuses on the representational mechanisms, batch updates with the full model of the environment are used. The authors show that \emph{Forecasts} are able to distinguish nearly identical states in the grid-world based on long action sequences and conclude that fixed-length features (PSR) do not generalize well to other tasks.




\subsubsection{Methods based on Feudal reinforcement learning}
Feudal Networks follow a hierarchical distribution of roles, where higher level agents command lower level agents to perform certain tasks. This implies immediate interaction between direct ranks, where a low-ranking agent accepts orders from its immediate supervisor, the supervisor follows the commands of their immediate superiors and so on. The idea of Feudal Reinforcement Learning (FRL) was first introduced by \citet{Dayan1993_Feudal}. The authors model the communication between hierarchical layers via goals, provided by higher levels and directed to lower levels, in a top down fashion. 

Feudal Networks for Hierarchical Reinforcement Learning (FuN) \cite{Vezhnevets2017_Feudal} introduce a fully differentiable deep reinforcement learning architecture inspired by FRL.
The two main components of FuN are the worker and the manager. 
These compose two levels of hierarchy, where the Manager is the top level defining goals for the lower level Worker. These goals are defined by the Manager itself, at a lower temporal resolution than the goals sought by the Worker. The Worker’s duty is to decide upon making simple directional actions within the environment whereas the Manager aims to approach the overall goal of completing the task. The lower temporal resolution is achieved by employing dilated LSTMs. 
The Worker generates actions based on external observation, the Manager’s goal and its own state. The Manager and the Worker take an observation from the environment and compute a shared intermediate representation in the form of an embedding vector. The Manager’s goals are trained using an approximate transition policy gradient. This is an efficient form of policy gradient training which relies on the assumption that Worker’s behavior will eventually align with the goal. The Worker is trained using an intrinsic reward to produce actions that allow the goal directions to be reached.

A key difference between FuN and the options framework is that in FuN the subgoals to be achieved by the worker are represented in a low-dimensional latent space, and not in the low-level perception space. The manager of the FuN also involves a latent state representation. 

\cite{Dilokthanakul2019_Feature} extends the Feudal Network~\cite{Vezhnevets2017_Feudal} with an auxiliary task in the lower level of hierarchy (i.e. feature-control or pixel-control) as a source of intrinsic reward. The intrinsic reward is computed based on the differences between two consecutive frames wrt a certain patch in the whole image--pixel based, or wrt the mean activation of a selective feature map--feature based. This additional reward is provided by the metacontroller to bias the subcontroller to complete the subgoals. At the same time, the metacontroller learns to selects the subgoal sequence for the subcontroller to maximize the accumulated extrinsic reward from the environment. By leaking the extrinsic reward to the subcontroller, the approach also allows the subcontroller to optionally solve the main task by its own. The combination of the two type of rewards help to align the task of representation learning with the main task of the RL agent. The approach does not show the ability to abstract the state representation for planning task with the metacontroller. 

\subsubsection{Non-hierarchical RL approaches}

\paragraph{Approaches Featuring Compositionality}
\citet{ToroIcarte2018_MultiTask_LTL_RL} use linear temporal laogic (LTL) to decompose a task into subtasks that can be learned by a reinforcement learning agent. 

\paragraph{Transfer Learning}

\citet{Devin2017_Transfer_RL} tackle the problem of transfer learning between different tasks and robot morphologies. 
Due to the lack of a direct supervision signal, applying traditional approaches for transfer learning to reinforcement learning is challenging. The authors instead propose a decomposition of the learned policy into task-specific and robot-specific modules to realize zero-shot transfer learning for novel robot-task combinations or at least accelerate their learning.
The algorithm is realized with Guided Policy Search but can be adapted to other methods like policy gradient or actor-critic. The approach is evaluated in a simulation environment with two different morphologies (3 DoF and 4 DoF arm) and two different tasks (reaching and drawer opening). 
While a decomposition, according to morphology, is not applicable in a biological context, the authors argue that their approach offers a generic framework for composable policy modules and could, in theory, be adapted for hierarchical reinforcement learning.

\paragraph{Model-based RL}
There are several non-hierarchical RL approaches that use a forward model for training a controller. The canonical implementation of this approach is referred to as Dyna-Q and has been proposed by \citet{Sutton1990_Dyna}.

The strategic attentive writer (STRAW) approach by \citet{Vezhnevets2016_STRAW} learns to abstract actions in an end-to-end manner based on observations from the environment. Essentially, macro-actions are clusters over sequences of micro-actions that occur commonly. Strictly speaking, the approach is not hierarchical in the sense that it involves multiple decision-making layers. However, the clustering into macro-actions effectively creates abstract action primitives. 

\citet{Pathak2017_forward_model_intrinsic} present a method for state abstraction in which they train a forward model $f$ and an inverse model $g$ in an abstract latent state-space.  The latent state space is generated from the perceptive input $s$ with a mapping function $\phi$. By minimizing the forward prediction error in the latent space $||f(\phi(s_t),a_t) - \phi_{s_{t+1}}||_2^2$ and the inverse model error in the latent space $||g(\phi(s_t),\phi(s_{t+1})) - a_t||_2^2 $, the abstraction $\phi$ learns to consider only those aspects of the perceptive input that are relevant for the action execution. This idea, that the authors later refer to as Inverse Dynamic Features (IDF) has later been extended by \citet{Pathak2019_ICML_SelfSuperExploreDisa} and \citet{Burda2019_ICLR}. 

\subsubsection{Non-RL Hierarchical Problem-solving}
\citet{Zhang2018_CompPlanAttr} introduce composable planning with attributes. This is very similar to our recent approach that integrates planning with RL \cite{Eppe2019_planning_rl}, just that there is no hardcoded mapping from states to high-level semantic representations (as in our case) but a learned mapping of states to attributes. The authors label their approach as ``composable planning'', but the representations of states and actions are not compositional (rather are action sequences composable due to the planning). That is, the representations of the attributes that the authors learn are not compositional. 

\subsection{Representational Properties and Mechanisms of existing HRL approaches}
\label{sec:hrl:mechanisms}

\subsubsection{Inverse models / policies}
\label{sec:hrl:mechanisms:inverse_models}
An inverse model maps a state and possibly a goal to an action. Reinforcement learning either learns the inverse model directly (policy iteration) or, for discrete action spaces, it learns a value function that determines a value for each action in a given state, and the inverse model is then simply the selector of the action with the highest value. 

% All RL methods use an inverse model by definition (see \autoref{sec:background}). However, many approaches learn the inverse model indirectly, by learning a value function that assigns values to state-action pairs or state-goal-action triples. However, this can be considered also an inverse model, because the action-selection  is still performed on the b

\subsubsection{Forward models}
\label{sec:hrl:mechanisms:forward_models}

\subsubsection{Perceptual representation and preprocessing}
\label{sec:hrl:mechanisms:perception_preprocessing}
We consider the perceptual state representation as the input to the lowest-level policy. Proof-of-concept approaches \cite{Saxe2017_HRL_Multitask_LMDP} often build on a fully observable gridworld domain with a discrete perceptual space. There is also a tremendous increase in approaches that use simulated robotic environments with a realistic physical environment, such as provided by the Mujoco simulator \cite{}. Most of these approaches \cite{Eppe2019_planning_rl,Levy2019_Hierarchical,TBC} use the object data provided by the simulator. In that case, the perceptual space consists of the continuous coordinates, angles and velocities of the agent and objects in the environment. Another class of implementations use visual input, either provided by the rendering engine of a simulator (\cite{Eppe2019_planning_rl,Levy2019_Hierarchical,TBC}) or by a real camera \cite{}.

\subsubsection{Action abstraction}
\label{sec:hrl:mechanisms:action_abstraction}
Action abstraction is, by definition, an inherent mechanism of any HRL method. The probably most influential method for action abstraction has been proposed by \citet{Sutton_1999_options} as the \emph{options} framework. 

Other approaches, specifically those base on universal value function approximators (UVFAs) \cite{Schaul2015} represent high-level actions as subgoals in the low-level state-space. For example, \citet{Levy2019_Hierarchical} and also \citet{Nachum2018_HIRO} 

\subsubsection{State abstraction}

\subsubsection{The compositionality principle}

The principle of compositionality implies that the semantics of a compositional expression is determined by the semantics of its constituent expressions and certain interpretation rules to combine the constituent expression. 
In terms of reinforcement learning, this means that the meaning of a compositional action representation is determined by multiple constituent expressions and a set of rules to combine them. There is a distinction between syntactic and semantic compositionality.

As an example for syntactic and semantic compositionality, consider an action representation \concept{grasp(ball)}. 
The expression consists of several sub-expression and symbols, i.e., an action type symbol (``\concept{grasp}'') a semantic patient symbol (``\concept{ball}'') and delimiter symbols (``('',``)''). There exist syntactic rules that determine that the semantic patient of the action is described by the expression within the delimiters and the action type is determined by the expression before the opening delimiter. Hence, the expression \concept{grasp(ball)} is \emph{syntactically compositional}. 
This syntactic compositionality has the advantage that less atomic symbols are necessary to represent all possible combinations of action types (e.g. $n_a=4$ action types \concept{``grasp'', ``push'', ``move'', ``release''}) and arguments (e.g. $n_o=4$ object types \concept{``ball'', ``block'', ``stick'', ``pencil''}) compared to the number of symbols (e.g. $n_{total} = n_o * n_a = 16$) that would be required if each composed action would be represented by one non-compositional atomic expression like \concept{``graspBlock''}). Syntactic compositionality is not limited to symbolic expressions, but also applicable to distributed numerical expressions, such as vector representations. For example, a vector $v_1$ is a compositional representation if it is composed of other vectors, e.g., $v_2$ and $v_3$, and if there is an vector operation symbol $\circ$ that represents interpretation rules, e.g., $v_1 = v_2 \circ v_3$. 

In the context of embodied intelligent agents, the expression is also semantically compositional if an agent knows how to act based on the compositional representation just by interpreting the constituents of the expression and the semantic interpretation rules. For example, if an intelligent agent has a certain action policy for each action type, and if it has rules that correctly modulate the action policy for each object type even if the specific combination of action and object type is unknown to the agent, then the action representation is semantically compositional. 
It is this semantic compositionality that is interesting in the context of HRL for intelligent embodied agents. 

\paragraph{Compositionality of abstract high-level action representations}
Semantic compositionality of action representations is algorithmically useful because it simplifies the decision space of a problem-solving agent. Considering the above example with $n_a$ action types and $n_o$ action arguments. A non-compositional action representation requires an agent to decide between $n_a \cdot n_o$ action possibilities, whereas a compositional action representation reduces the decision space to $n_a + n_o$ possibilities.

In hierarchical reinforcement learning, high-level action representations are not always compositional. For example, most approaches based on options \cite{Sutton_1999_options}, i.e., low-level task-specific policies, involve a high-level policy that is essentially a classifier that selects an appropriate option given the current environment state. The output representation of the high-level policy is, therefore, simply a single index to indicate which option to execute on the low-level layer. The policy could be seen as a rule that tells the system how to interpret the representation, but the index itself is not composed of other expressions. 

In our survey, we found several approaches that feature compositional action representations. \citet{Saxe2017_HRL_Multitask_LMDP} compose high-level actions from concurrent linearly solvable Markov decision processes (LMDPs). This guarantees optimal compositionality, and the authors demonstrate the agent can successfully execute compositional policies that it has never solved before. The authors evaluate their work in simple grid-world domains. 

\paragraph{Compositionality of abstract high-level state representations}
We consider compositionality of high-level state representations in the following sense: Consider a high-level policy that takes as input syntactically compositional state representations (e.g. \concept{onTopOf(object1,object2)}). If the policy can correctly interpret the state representation, this means that the policy learns rules for interpreting the state representation semantically. In that case, syntactically compositional state representations are also semantically compositional. State representations are not necessarily symbolic; in most approaches they are, in fact, distributed continuous vector representations. 
For example, \citet{Zhong2019} propose to use a Variational Autoencoder (VAE) \cite{Higgins2017_B-VAE} to learn compositional state representations from sensorimotor exploration, in a manner that is independent from HRL. 
The Feudal Reinforcement Learning approach by \citet{Vezhnevets2017_Feudal} uses a dense neural network layer as a state abstraction function, providing a vector representation as output. This may lead to representations that are implicitly compositional, (cf. vector embeddings \cite{Mikolov2013}), but the authors do not elaborate on this. 


\subsubsection{Intrinsic reward}

\subsubsection{Active inference, free energy, surprise and curiosity}

\subsubsection{Goal space and extrinsic rewards}

\subsubsection{Learning transfer and analogy learning}

\subsubsection{On-policy vs. off-policy training}
\begin{table*}[h!]
The table is here: \url{https://1drv.ms/x/s!AkFdeL8LlTTlip9lJdytKEfulJ6wdg?e=Fh2nYr}
  \begin{center}
    \caption{Properties of existing HRL approaches}
    \label{tab:hrl_properties}
%     \pgfplotstabletypeset[
%       multicolumn names, % allows to have multicolumn names
%       col sep=semicolon, % the seperator in our .csv file
%       display columns/0/.style={
% 		column name=Method, % name of first column
% 		string type,
% 		column type={p{.3\textwidth}}},  % use siunitx for formatting
%       display columns/1/.style={
% 		column name=Action abstraction,
% 		,string type,
% 		column type={p{.3\textwidth}}},  % use siunitx for formatting
% 	  display columns/2/.style={
% 		column name=State abstraction,
% 		,string type,
% 		column type={p{.3\textwidth}}},  % use siunitx for formatting
%       every head row/.style={
% 		before row={\toprule}, % have a rule at top
% 		after row={
% % 			\si{\ampere} & \si{\volt}\\ % the units seperated by &
% 			\midrule} % rule under units
% 			},
% 		every last row/.style={after row=\bottomrule}, % rule at bottom
%     ]{hrl_table.csv} % filename/path to file

  \end{center}
\end{table*}



==> v0/intro_old.tex <==

\begin{figure*}
    \centering
    %trim={<left> <lower> <right> <upper>}
    \includegraphics[width=.19\columnwidth,trim={196pt 81pt 167pt 38pt},clip]{pics/1-crow-pickstick.png}
    \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(1)\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/2-crow-usestick.png}
    \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(2)\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/3-crow-getstone.png}
    \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(3)\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/4-crow-usestone.png}
    \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(4)\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/5-crow-havefood.png}
    \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(5)\end{minipage} 
    % \includegraphics[width=.18\textwidth,trim={0pt 0pt 0pt 105pt},clip]{pics/crow4.jpg}
    \caption{A New Caledonian crow solves a food-access problem \cite{Gruber2019_CrowMentalRep}: First, the crow picks a stick (1); then it uses the stick to access a stone (2,3); finally, it uses the stone to activate a mechanism that releases food (4,5). The crow has never solved this problem setup  before. Nevertheless, after a brief inspection phase, it is able to solve the problem in one shot, i.e., without any further trial and error. 
    % From the inspection phase, it knows where the individual stations are, but the stations are not visible from each other, e.g., the crow cannot see the stone-station from the stick-station. 
This suggests that the crow develops and uses memorized abstract mental representations to plan ahead.}.
    \label{fig:crow_probsolving}
\end{figure*}

\section{Introduction (1.5p)}
\label{sec:intro}

Humans and certain intelligent animal species have the ability to break down complex unknown problems into hierarchies of simple previously learned sub-problems. This hierarchical approach also allows them to solve previously unseen problems in a one-shot manner, without any further trial and error. 
% What are the mechanisms that are responsible for the capability to unseen solve problems by insight and causal inference in a one-shot manner, without any trial and error?
% Humans and certain intelligent animal species are able to perform \emph{one-shot problem-solving}. They can solve a previously unseen causally non-trivial problem by breaking it down into a hierarchy of previously learned sub-problems. 
For example, \autoref{fig:crow_probsolving} depicts how a New Caledonian crow solves a non-trivial food-access puzzle that consists of three causal steps: It first picks a stick, then uses the stick to access a stone, and then uses the stone to activate a mechanism that releases food \cite{Gruber2019_CrowMentalRep,Taylor2009}. 
Other experiments with crows demonstrate their transfer-learning performance \cite{Taylor2014_CorvidCognition}, and there exist numerous related experiments that attest similar capabilities to primates \cite{Rumbaugh2003_Intelligence_Apes} and, of course,  humans \cite{Perkins1992}.
Yet, little is known about the cognitive mechanisms that are responsible for these capabilities. 



A common method to illuminate the cognitive processes of biological agents is to model them computationally and to evaluate them with virtual or robotic agents. 
The currently existing computational systems provide less sophisticated problem-solving mechanisms than intelligent biological agents, but there exist several promising cognitively inspired computational methods that have the potential to be developed further, to achieve a problem-solving performance that is in many aspects similar to the crow's behavior.
One of the currently most popular computational methods for learning-based problem-solving is reinforcement learning \cite{Arulkumaran2017_DeepRL,Li2018_DeepRL_Overview}. 

Several studies suggest that reinforcement learning is in many aspects biologically and cognitively plausible (cf. \cite{Neftci2019_RL_BioArtificial_NatureMI,Sutton2017} for an overview). 
Existing RL-based methods are to some extent able to perform one-shot (aka. zero-shot) problem-solving and learning transfer. However, this is currently only possible for minor variations of the same or a similar task \cite{Eppe2019_planning_rl} or in in simple synthetic domains, such as a 2d gridworld \cite{Sohn2018_Zero-ShotHRL,Oh2017_Zero-shotTaskGeneralizationDeepRL}. A continuous-space problem-solving behavior that is comparable with the crow's behavior of \autoref{fig:crow_probsolving} has not yet been realized on any embodied computational system. 


So what are the critical cognitive prerequisites for learning-based problem-solving and skill transfer? What are the most critical shortcomings of existing reinforcement learning architectures? And how can we overcome the limitations of existing reinforcement learning methods?
Research in human and animal cognition strongly suggests that problem-solving and learning happens on multiple hierarchically arranged representational layers \cite{TODO}. 
However, the fraction of recent reinforcement-learning based approaches that involve hierarchical structures is very small. 
We performed a comprehensive search over reinforcement learning review articles since 2015 using the Microsoft Academic search engine (see \autoref{sec:appendix:meta_RL-survey} for details). 
The most cited review article on RL since 2015 \cite{Arulkumaran2017_DeepRL} dedicates 1/6th of a page out of 16 pages to HRL. In the second most cited article \cite{Garcia2015_safeRLSurvey}, HLR is not considered at all, i.e, the word stem `hierarchic' does not appear anywhere in the text. The third most cited review article \cite{Li2018_DeepRL_Overview} dedicates 2/3rd of a page out of 85 total pages to HRL.
From 37 reinforcement learning reviews and surveys published since 2015, only two contain the word stem ``hierarchic'' in their abstract. 

% The , and the lack thereof in 
Based on this meta-survey and the reported importance of hierarchically structures mechanisms and representations for biological problem-solving agents, we hypothesize that a critical reason why computational systems fail to perform better is that the existing approaches do not investigate enough the hierarchical aspects of learning and problem-solving. 

To systematically and comprehensively address our hypothesis, and to further illuminate the finer-grained mechanistic discrepancies between the sophisticated problem-solving behavior of intelligent biological agents and the limited capabilities of existing computational reinforcement learning agents, we structure this review as follows:

 In \autoref{sec:cognitive_background}, we present a review on research in human and animal cognition related to learning, decision-making and goal-directed behavior. From this survey, we extract core mechanisms and principles that are suitable and sufficiently understood to be modeled within a computational framework. 
We show that many of these mechanisms are based on hierarchical mental abstraction and sensorimotor prediction using a forward model. 
%
Based on our survey over cognitive problem-solving and learning mechanisms, we review the state of the art in recent hierarchical reinforcement learning in \autoref{sec:hrl}. 
% This review is comprehensive with respect to HRL literature published between January 2017 and May 2020, and we also consider the most important previous work. 
%
In \autoref{sec:conclusion} we conclude that most approaches computational hierarchical approaches are model-free, whereas the results from \autoref{sec:cognitive_background} suggest that problem-solving is highly dependent on a predictive forward model. Another critical gap that we reveal is that most computational approaches implement temporal action abstraction but they do not address state abstraction and compositional sensorimotor grounding. 

% There exist several different subdisciplines within Artificial Intelligence that address hierarchical one-shot problem-solving. As examples consider Task and Motion Planning (e.g. \cite{Toussaint2018}) or hierarchical planning (e.g. \cite{Nau2003_SHOP2}). 
% However, a keyword search in relevant conferences such as IJCAI, AAAI, ICLR reveals that most progress in the past years has been made in the 
% 

% \begin{wrapfigure}{r}{0.5\textwidth} 

% \end{wrapfigure}




==> v0/notes.tex <==
\section{Notes}
\begin{enumerate}
    \item Nature formatting guides (Nature Journal itself, not sub-journals like NMI) \url{https://www.nature.com/nature/for-authors/formatting-guide}
    \item Summary guideline: \url{https://www.nature.com/documents/nature-summary-paragraph.pdf}
    \item For Reviewers: \url{https://www.nature.com/nature-research/editorial-policies/peer-review}
    \item Anonymity: https://www.nature.com/documents/nr-double-blind-peer-review.pdf
	\item Author instructions:     \url{https://mts-natmachintell.nature.com/cgi-bin/main.plex?form_type=display_auth_instructions}
	\item Submission system: \url{https://mts-natmachintell.nature.com/cgi-bin/main.plex}



\end{enumerate}


==> v0/strategic_outline.tex <==
\section{Strategic outline}
\subsection{Why is this paper well worth reading?}
\begin{itemize}
    \item Biological agents can perform problem-solving better than humans (in many but not all ways). 
    So what are the mechanisms that artificial agents lack and that biological agents have?
    \item Several other reviews in this area investigate related issues, e.g. they relate computational reinforcement learning with biological foundations (e.g. \citet{Neftci2019_RL_artificial_bio}, Nature Machine Intelligence). 
    However, there is a lack of review articles that investigate the integration of reasoning with control for problem-solving. 
\end{itemize}



\subsection{Who are we to be credible so that you can believe what we write?}

Several important papers in continual learning, reinforcement learning, cognitive modelling, etc.

\subsection{What are the goals of this paper?}
We want to understand how current learning-based problem-solving systems could be improved, further towards human-level performance. This involves three subgoals:
\begin{enumerate}
\item We want to understand and summarize widely accepted principled mechanisms 
\item We want to identify shortcomings of current computational architectures that integrate reasoning and motor control for problem-solving
\item We want to propose a computational framework that is capable of learning human-level problem-solving. (e.g. Duncker's candle problem, or the crow tool-use problem)
\end{enumerate}


\subsection{How do we achieve the goals?}
Three steps:
\begin{enumerate}
    \item Perform meta-survey in cognitive psychology and related areas to identify mechanism that are important. 
    \item Analyze existing HRL approaches with respect to these mechanisms and identify lack of some mechanisms.
    \item Suggest how shortcomings can be overcome by proposing a unifying computational framework that fixes the shortcomings.
\end{enumerate}


==> v1/results.tex <==
\section{Critical discussion and outlook}
\label{sec:results}
For our discussion and outlook, we first summarise the state-of-the-art implementations in hierarchical reinforcement learning and summarise their shortcomings based on our overview in the supplementary \autoref{tab:hrl_properties}. 
Second, then identify possible reasons for these shortcomings and link them to challenges that arise from the integration of the different mechanisms. 
Third, we provide proposals for techniques and methods to overcome these shortcomings. 
We present an overview of the relation between the shortcomings, challenges and proposed solutions in \autoref{fig:challenges_shortcomings_solutions}.
% We present a summary of these results in \autoref{sec:shortcomings_solutions}. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,trim=2.5cm 4cm 2cm 4cm, clip]{pics/Shortcomings_Challenges_Solutions.pdf}
    \caption{Our section \nameref{sec:hrlFinal} identifies several shortcomings of contemporary HRL methods. We suppose that these result from at least four specific central challenges that are hard to overcome. We also provide three suggestions for key methods that may help to address the challenges.}
    \label{fig:challenges_shortcomings_solutions}
\end{figure*}

\subsection{Shortcomings of existing HRL architectures}
Our computational realizations section and the supplementary \autoref{tab:hrl_properties} provide a comprehensive overview over state-of-the-art computational hierarchical reinforcement learning approaches.
% , in alignment with our structuring of cognitive prerequisites and mechanisms for the problem-solving abilities of intelligent biological agents (see \autoref{fig:cog_prereq}). 
Based on this overview, we identify the following major struggles of the current methods:


\noindent \textbf{Hierarchical mental simulation.}
While numerous non-hierarchical methods show how mental simulation can improve sample efficiency\cite{Deisenroth2011,Ha2018_WorldModels}, our summary shows that reinforcement learning with hierarchical mental simulation is underrepresented.
% As a result, inter-dependencies between sub-tasks are hard to detect. 
Most current few-shot problem-solving methods build on transfer learning, but they neither leverage decision-time planning nor background planning to exploit hierarchical mental simulation.
A problem is that high-level mental predictions require stable hierarchical representations and precise forward models. 
% This result is interesting because any approach with a forward model could straight-forwardly be extended to also consider planning\cite{Botvinick2014}.
% , and planning can be leveraged for few-shot problem-solving\cite{Sharma2020_DADS}. 
% Therefore, current model-based approaches do not exploit their full potential.

\noindent \textbf{Intrinsic motivation.}
In our survey, we distinguish between the three most frequently used kinds of intrinsic motivation: curiosity, diversity, and subgoal discovery. 
Our section \nameref{sec:hrlFinal} and the supplementary \autoref{tab:hrl_properties} show that curiosity and diversity are underrepresented intrinsic motivation methods: they are implemented in only 8 of 47 surveyed papers, while our section \nameref{sec:cognitive_background} shows significant cognitive evidence that these mechanisms are critical for intelligent behaviour in humans\cite{Oudeyer2018_CompuCuriosityLearning}. 
We suggest below that one reason for this shortcoming may be that prediction-based intrinsic motivation suffers from an overly simplistic uncertainty handling of current computational forward models.


\noindent \textbf{Compositional representations.}
All hierarchical reinforcement learning methods inherently perform representational abstraction, e.g., through options or subgoals, but only a few methods consider compositionality. Exceptions include natural language-based representations of actions \cite{Jiang2019_HRL_Language_Abstraction} or symbolic logic-based compositional representations \cite{Oh2017_Zero-shotTaskGeneralizationDeepRL}.
None of these approaches ground these abstractions tightly in sensorimotor experiences. 
However, as we describe in section \autoref{sec:cognitive_background}, compositionality has many benefits for transfer learning and decision-time planning. 
Since compositional representations generally build on variable-value representations, these need to be researched first on a more general level to alleviate this shortcoming. 

\noindent \textbf{Inference-fitted state abstraction.}
Recent hierarchical actor-critic approaches \cite{Levy2019_Hierarchical,Roeder2020_CHAC} use the same state representation for each layer in the hierarchy. However, it seems cognitively more plausible to fit the level of abstraction to the level of inference to be performed on each hierarchical layer.
There exist RL-methods, where abstract (aka. latent) representations are generated from visual data with a convolutional autoencoder\cite{Ha2018_WorldModels}. 
However, representations generated by autoencoders are optimized for reconstructing the input data, and not for using the latent representations to perform decision-making. 


% There exist a few approaches that perform inference-fitted state abstraction\cite{Vezhnevets2017_Feudal}, and also some that involve compositional state representations\cite{Vezhnevets2020_OPRE}. 
% However, most of these build on hand-crafted abstraction functions that are not learned \cite{Eppe2019_planning_rl}.
A problem for learning inference-fitted abstraction functions is that the reward signal of reinforcement learning is a relatively weak driver for the learning process, compared to other methods like supervised learning. 




\subsection{Central challenges of integrated hierarchical architectures}
\label{sec:results:challenges}
We hypothesize that the above shortcomings are the result of several central challenges that occur when integrating the mechanisms depicted in \autoref{fig:cog_prereq} in a unifying hierarchical architecture.  


% These involve advanced uncertainty models, computational implementations of bidirectional action-effect associations, and inference-fitted abstraction. 


% \textbf{Uncertainty modelling}

% \textbf{Bidirectional action-effect models}

% \textbf{Inference-fitted abstraction}



\noindent \textbf{Stabilize hierarchical representation learning.} 
Hierarchical mental simulation demands stable high-level representations to learn a high-level forward model. 
However, a general problem of hierarchical architectures is that a high-level layer can only learn meaningful behaviour after the lower-level layer has converged. 
% A naive solution to address this issue is a threshold-based mechanism that detects the convergence of the lower-level to determine when the higher level layer may start training. 
% This, however, does not consider continual and lifelong learning settings, where an agent's lower level behaviours and representations develop continuously. 
% In hierarchical decision-making, this problem affects hierarchical mental simulation. 
In the next subsection, we discuss how learning in hindsight\cite{Andrychowicz2017,Levy2019_Hierarchical} and bi-directional dynamics models\cite{Pathak2017_forward_model_intrinsic,Pathak2019_ICML_SelfSuperExploreDisa} may partially alleviate this problem.

\noindent \textbf{Alleviate the model bias.}
A forward model is never perfect, and multiple successive predictions lead to huge accumulated errors that render the predictions unusable. This problem is known as the model bias problem, and it demands for better uncertainty models to make the agent aware of the confidence of its predictions. 
% Successful non-hierarchical approaches like PILCO \cite{Deisenroth2011} demonstrate the sample-efficiency of uncertainty-aware forward models based on Gaussian Process Models, but these models are only suitable for low-dimensional state and action representations. 
Another dimension of this problem occurs with noisy observations or chaotic and unpredictable system dynamics, which is an issue for intrinsic motivation methods based on prediction. 
For example, \citet{Roeder2020_CHAC} achieve curiosity-driven intrinsic motivation by maximizing the prediction error of a forward model. 
This causes the agent to suffer from the so-called \emph{noisy TV problem}, where an agent always strives to encounter unpredictable observations (such as a TV showing only white noise), instead of searching for predictable situations that it just cannot predict yet. 

In a hierarchical setting, this problem interferes with the problem of learning hierarchical representations, because high-level representations that are still being learned are hardly predictable at all. 


\noindent \textbf{Improve variable-value assignment.}
Abstract compositional representations build on rules to determine the semantics of the composed data structure. 
These rules require, in one way or another, variable-value pairs, where the variable describes a general semantic property. 
For example, the disentangled vector representations that occur in variational autoencoders (VAEs) are compositional data structures, where each slot of the vector is a variable that represents a certain object property (e.g. the angle of a visual object).
In language, the variables are roles of syntactic constructions, and the values are the words that fill these roles. 
A problem with VAEs is that they do not support dynamic semantic representations with varying variables because the structure of the latent representations fixed, and therefore, also  the set of variables is fixed. They also do not support variables that are assigned to other variables. 
Variable-value assignment is a particular issue in hierarchical decision-making, where low-level sensorimotor data is abstracted to high-level compositional representations that are used for high-level decision-making. 

% \citet{Kriete2013_SymbolProc} provide a neurologically plausible model of variable-value assignment where variables are areas in the prefrontal cortex that act like a pointer in computer science, pointing to other areas which represent values. 
% This is somewhat akin to Transformer neural networks, where Query, Key and Value vectors are used for a self-attention-mechanisms. 



\noindent \textbf{Strengthen the feedback signal.}
Learning-based inference-fitted abstraction demands a strong feedback signal to learn the respective abstraction functions. 
However, in reinforcement learning the reward signal is often relatively weak compared to a supervised loss signal, especially in sparse reward settings where handshaped continuous reward functions are not present.
In hierarchical reinforcement learning, this problem is even more severe if the goal is to learn also abstraction functions for inference-fitted high-level state representations. 
Hence, hierarchical reinforcement learning with inference-fitted abstraction demands a stronger feedback signal to stabilize the learning. 
% In the subsection below, we propose a potential solution to address this problem, based on bi-directional dynamics models. 

\subsection{Suggestions for addressing the challenges}
\label{sec:results:solutions}
In the following, we sketch how a collection of previously proposed methods may help to address the above challenges. The methods will not solve all problems related to hierarchical reinforcement learning, but we believe that they are important key mechanisms for future developments. 


\noindent \textbf{Learning in hindsight.}
Hierarchical reinforcement learning demands stable high-level representations. 
This is a problem because stable high-level representations can only emerge once the learning of the lower-level has converged. 
We suggest that one potential key method to alleviate this issue is learning in hindsight. 
Learning in hindsight has been proposed by \citet{Andrychowicz2017} to alleviate the sparse reward problem in goal-conditioned reinforcement learning. The technique builds on learning from failures, in the sense that an agent gets rewarded even if it fails to achieve a reinforcement learning goal. This is realized by pretending in hindsight that the achieved goal was the actual goal. 
\citet{Levy2019_Hierarchical} extend the method to hierarchical architectures by also proposing hindsight actions. 
In their hierarchical framework, high-level actions are subgoals to be achieved by the lower-level layer. 
Hindsight high-level actions are retrospectively defined as the subgoals that were actually achieved by the low-level layer, regardless of what the original subgoal was. 
In other words, by pretending in hindsight that the executed action (aka. subgoal) was the intended action, there is no need any more to wait until the low-level behaviour has converged. 
We suppose that this is a valuable component of a unifying framework with stable hierarchical representations. Stabilizing the high-level representations by learning in hindsight may also help to alleviate the model bias, but, of course, there are still many other open ends to address. 

\noindent \textbf{Bi-directional dynamics models.}
Bi-directional models involve both forward and backward inference, and we suppose that this combination is beneficial for addressing several challenges. Our supposition is based on the work by \citet{Pathak2017_forward_model_intrinsic} and by \citet{Hafner2020_Dreamer}, who use a combined forward and inverse model to generate latent representations in a self-supervised manner. 
The bi-directional model operates on a latent space representation that is generated by an abstraction function. 
Their method learns simultaneously the abstraction function, the forward model and the inverse model. 
By simultaneously performing inverse and backward prediction in the latent space, the abstraction function gains two important features: i) the latent space that it generates is noise-free because only the predictable parts of the observation determine the forward and backward prediction. ii) the method is self-supervised and, therefore, provides a more stable feedback signal than the comparatively weak reward signal. 
This leads to more stable high-level representations, it alleviates the prediction error, and it strengthens the overall learning signal. The stronger learning signal is also better suited to learn advanced structured abstraction functions that generate compositional representations, e.g. disentangled state vectors or symbolic compositional representations\cite{Lyu2019_SDRL,Eppe2019_planning_rl}. 



\noindent \textbf{Meta- uncertainty models.}
Prediction errors play an important role in mental simulation and intrinsic motivation. 
In our section \nameref{sec:cognitive_background} we discuss active inference and active learning\cite{Schwartenbeck2019_CompUncertainExplo} as two seemingly contradicting mechanisms that build on predictive processes models. 
Active inference seeks to minimize long-term surprise, of which a special case is to minimize a forward model's uncertainty or prediction error. Active learning, however, seeks to maximize the information gain. This seemingly contradicts active inference because recent research shows that active learning can be achieved by maximizing the uncertainty\cite{Haarnoja2018_SAC} or prediction error \cite{Roeder2020_CHAC}. 
\citet{Schwartenbeck2019_CompUncertainExplo} builds on \citet{Yu2005UncertaintyAttention}'s concept of \emph{expected uncertainty} to explain how both mechanisms can be unified. 
Unexpected uncertainty can be understood as meta-uncertainty, i.e., the uncertainty about the uncertainty.
We suppose that an intrinsic reward for high meta-uncertainties would lead to explorative behaviour, causing low long-term meta-uncertainties. The gained certainty about the uncertainty of forward models can lead to new predictive processes that are aware of their own model bias. 




\noindent \subsection{Challenges remaining}
The above proposals for addressing the central challenges of hierarchical reinforcement learning are most probably not sufficient for developing artificial agents that are as smart as intelligent animals, such as the crow of \autoref{fig:crow_probsolving}. 
The biggest remaining challenge lies in the integration of the methods, towards a unifying computational framework.
A problem is the cross-dependencies between the individual methods.
For example, hindsight learning requires bi-directional abstraction functions to map abstract high-level representation back to the context-specific low-level representations. 
This is necessary because otherwise the system cannot derive the high-level hindsight actions from the low-level state representation. Another open question is how to model unexpected uncertainty in bidirectional models. 
% These cross-dependencies are not only conceptually difficult, they also imply software-technological challenges. Each one of the proposed mechanisms comes with its ows variants and hyperparameters TBC...
This article does not provide solutions to these remaining challenges, and it is impossible to foresee them all. However, we present here some guidelines for next steps, and attempts to develop computational models of our proposed integrated framework will help to understand the remaining challenges better. 




==> v2/abstract.tex <==
\begin{abstract}
According to cognitive Psychology and related disciplines, the development of complex problem-solving skills depends on several critical mechanisms, including hierarchical mental representations.
Hierarchical reinforcement learning may be considered the most promising computational approach that may eventually yield comparable problem-solving skills in artificial agents and robots. 
However, to date the problem-solving abilities of intelligent animals---including human and non-human primates, crows, and octopuses---still are clearly superior to those of artificial systems.
\revv{In this article, we propose an integrative computational architecture to enable advanced problem-solving skills in artificial agents.}{E-\ref{rev:editor:review_perspective}}
Our proposal builds on three elements: First, we present a survey of the literature in cognitive Psychology, suggesting that most critical cognitive mechanisms for solving complex problems involve compositional abstraction and predictive processing.
Second, we relate the gained insights with contemporary hierarchical reinforcement learning methods for accomplishing similar problem-solving skills in artificial agents.
\revv{Interestingly, our results suggest that all identified cognitive mechanisms have been implemented individually in isolated computational architectures, raising the question of why there exists no single unifying architecture that integrates them.
We address this gap in the third part of this article, and provide an integrative perspective on the computational challenges to develop such a unifying architecture. Herein, we propose cognitively inspired methods to address the involved integration challenge.}{E-\ref{rev:editor:review_perspective}; E-\ref{rev:editor:difficulties:integration}; R3-\ref{rev:r3:clarify_contrib}}
We expect our results to guide the development of more sophisticated cognitively inspired hierarchical machine learning architectures.
% , so that future artificial agents achieve a problem-solving performance on the level of intelligent non-human animals like crows. 
\end{abstract}

==> v2/all_table.tex <==

% \cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}

\begin{table*}[!ht]
{\sffamily 
% The full Excel table is here: \url{https://1drv.ms/x/s!AkFdeL8LlTTlip9lJdytKEfulJ6wdg?e=Fh2nYr}
  \centering
  \captionsetup{singlelinecheck = false, justification = raggedright}
\caption{Abilities, mechanisms and prerequisites of recent hierarchical reinforcement learning  approaches.}
\vspace{-10pt}
  \scriptsize
\rowcolors{2}{TableRowColor}{TableRowColor}
  \begin{tabular}{R{.14\textwidth}  C{.05\textwidth}  C{.06\textwidth}  C{.08\textwidth}  C{.055\textwidth}  C{.055\textwidth}  C{.08\textwidth}  C{.08\textwidth}  C{.08\textwidth}  C{.08\textwidth} }

\arrayrulecolor{black}            
  \rowcolor{TableRowColor}
            & \multicolumn{3}{ c  }{\scshape \large Abilities} & \multicolumn{4}{ c  }{\scshape \large Mechanisms} & \multicolumn{2}{ c }{\scshape \large Prerequisites} \\

\rowcolor{TableRowColor}
  {\scshape \large Approach} & Few-shot problem-solving & Transfer learning --------------- \begin{minipage}{.06\textwidth} N: near \\ F: far \end{minipage} \newline & Decision-time planning ------------------ \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline &  \multicolumn{2}{ c }
   {
  \begin{minipage}{.13\textwidth} {\centering \vspace{5pt} Sensorimotor abstraction \\ --------------------------- \\} B: basic \\ I: inference-fitted \\ C: compositional \\ \hspace{2pt}  ( actions )~~~~~~~~~ ( states )\end{minipage} 
   } & 
   Intrinsic motivation ------------------- \begin{minipage}{.1\textwidth}C: curiosity \\D: diversity \\SG: subgoals\\[0pt]  \end{minipage} &
   Mental simulation ------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline & 
    \newline Forward model -------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline & 
   Inverse model / policy ------------------- \begin{minipage}{.08\textwidth} H: high-level \\ L: low-level \end{minipage} \newline \\\hline

\arrayrulecolor{white}

\citetsupp{Akrour2018_RL_StateAbstraction} & - & - & - & I,C & I & - & - & - & H,L\\\hline
\citetsupp{Arulkumaran2016_Classifying_Options_for_Deep_RL} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Bacon2017_OptionCritic} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{barreto2020fast} & (X) & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Beyret2019_DotToDot} & - & - & - & C & - & - & - & - & H,L\\\hline
\citetsupp{Blaes2019_CWYC} & - & - & H & I & - & C, SG & H & H,L & L\\\hline
\citetsupp{Chuck2020_HyPe} & - & - & - & I & - & C & - & - & H,L\\\hline
\citetsupp{Dietterich2000_StateAbstraction_MAXQ} & - & - & - & I & I,C & SG & - & - & H,L\\\hline
\citetsupp{Eppe2019_planning_rl} & - & - & H & I,C & I,C & SG & H & H & L\\\hline
\citetsupp{Eysenbach2019_DiversityFunction} & - & N & - & I & - & D & - & - & H,L\\\hline
\citetsupp{Frans2018_MetaLearningHierarchies} & (X) & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Ghazanfari2020_AssociationRules} & - & - & - & I & I & - & - & - & H,L\\\hline
\citetsupp{Ghosh2019_ActionableRep} & - & - & - & I & I & SG & - & - & H,L\\\hline
\citetsupp{Haarnoja2018_LatentSpacePoliciesHRL} & - & - & - & I & - & SG & - & - & H,L\\\hline
% \citetsupp{Hafez2020_dual-system} &  &  &  &  &  &  &  &  & \\\hline
\citetsupp{Han2020_hierarchicalSelfOrga} & X & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Heess2016_transferModulControl} & X & F & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Hejna2020_MorphologicalTransfer} & X & F & - & C & - & - & - & - & H,L\\\hline
\citetsupp{jaderberg2019human} & - & N & - & I & I & SG,(D) & - & - & H,L\\\hline
\citetsupp{Jiang2019_HRL_Language_Abstraction}  & X & N & - & I,C & B & - & - & - & H,L\\\hline
\citetsupp{Kulkarni2016_HDQN} & - & - & - & I & I,C & SG & - & - & H,L\\\hline
\citetsupp{Levy2019_Hierarchical} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Li2017_efficient_learning} & - & - & H & I,C & - & - & H,L & H,L & H,L\\\hline
\citetsupp{Li2020_SubPolicy} & X & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Lyu2019_SDRL} & - & - & H & I & I,C & SG & H & H & L\\\hline
\citetsupp{Ma2020_MultiAgentHRL} & - & - & H & I & I & - & H & H & L\\\hline
\citetsupp{Machado2017_PVF_Laplace_OptionDiscovery} & - & - & - & I & I & D & - & - & H,L\\\hline
\citetsupp{Nachum2018_HIRO} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Oh2017_Zero-shotTaskGeneralizationDeepRL} & X & N & - & I,C & I & SG & - & - & H,L\\\hline
\citetsupp{Qiao_2020_HRL-Driving} & - & - & - & I & - & SG & - & - & H,L\\\hline
\citetsupp{Qureshi2020_CompAgnosticPol}	& -	& F& 	-& 	I,C	&-& 	SG,D& 	-& 	-& 	H,L \\\hline
\citetsupp{Rafati2019_model-free_rep_learning} & - & - & - & C & - & SG & - & - & H,L\\\hline
\citetsupp{Rasmussen2017_NeuralHRL} & - & N & - & I,(C) & I & SG & - & - & H,L\\\hline
\citetsupp{Riedmiller2018_SAC-X} & - & - & - & I & - & SG & - & - & H,L\\\hline
\citetsupp{Roeder2020_CHAC} & - & - & - & C & - & C,SG & - & - & H,L\\\hline
\citetsupp{Saxe2017_HRL_Multitask_LMDP} & - & - & - & I,C & - & SG & - & - & H,L\\\hline
\citetsupp{Schaul2013_Better_Generalization_with_Forecasts} & - & - & - & I & I,C & - & - & - & H,L\\\hline
\citetsupp{Shankar2020_MotorPrimitives} & - & - & - & I & - & D & - & - & H,L\\\hline
\citetsupp{Sharma2020_DADS} & X & N & H & I & - & D & H & H & L\\\hline
\citetsupp{silver2016mastering} & - & - & H & I & I & - & H & H & L\\\hline
\citetsupp{Sohn2018_Zero-ShotHRL} & X & N & - & I,C & I & SG & - & - & H,L\\\hline
\citetsupp{sutton2011horde} & - & (N) & - & - & I & - & L & L & L\\\hline
\citetsupp{Tessler2017_LifelongHRLMinecraft} & (X) & N & - & I,C & - & - & - & - & H,L\\\hline
\citetsupp{Vezhnevets2017_Feudal} & - & - & - & I & I & - & - & - & H,L\\\hline
\citetsupp{Vezhnevets2020_OPRE} & - & - & - & I,C & I,C & -  & - & - & H,L\\\hline
\citetsupp{Wu2019_ModelPrimitives}	& -	& N	& -	& I	& -	& -	& L	& L	& H,L \\\hline
\citetsupp{Wulfmeier2020_HierachicalCompositionalPolicies} & - & N & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Yamamoto2018_RL_Planning} & - & - & H & I,C & - & SG & H & H & L\\\hline
\citetsupp{Yang2018_PEORL} & - & - & H & I & - & SG & H & H & L\\\hline
\citetsupp{Yang2018_HierarchicalControl} & - & - & - & I & - & - & - & - & H,L\\\hline
\citetsupp{Zhang2020_AdjancentSubgoals} & - & - & - & C & - & SG & - & - & H,L\\\hline
  \end{tabular}
 \normalsize
    \label{tab:hrl_properties}
}
\end{table*}



==> v2/cogShortNew.tex <==
\begin{figure*}[ht!]
    \centering
    % \includegraphics[width=0.9\textwidth]{pics/illustration_basic.pdf}
    %trim={<left> <lower> <right> <upper>}
        %\includegraphics[width=.6\textwidth,trim={110pt 0pt 0pt 0pt},clip]{pics/cog_abilities.pdf}
        %\includegraphics[width=\textwidth,clip]{pics/CognitiveMechanismsIllustrationGrey.pdf}
        \includegraphics[width=\textwidth]{pics/cog_illustration_8.pdf}
    \caption{Prerequisites, mechanisms, and features of biological problem-solving agents. 
    \emph{Forward-} and \emph{inverse models} are prerequisites for higher-order mechanisms and abilities.
    \emph{Compositional abstractions} of forward models allow the agent to decompose a problem into reusable substructures, e.g., by learning which part of an object is easily graspable, such as the stem of a glass.
    \emph{Intrinsic motivation} applied with the help of forward models can drive an agent to interact with its environment in an information-seeking, epistemic way, e.g., by eliciting interactions with the glass to learn more about its properties.
    \emph{Mental simulations} enable the exploration of hypothetical state-action sequences, e.g., by imagining how the hand position will evolve while reaching for the glass.
    %These mechanisms form the foundation for more complex problem solving abilities:
    Given these mechanisms, an agent can flexibly achieve desired goal states via hierarchical, compositional \emph{goal-directed planning}, e.g., planning to drink from the glass by first suitably grasping and then appropriately transporting it.
    Compositional abstractions enable the agent to perform \emph{transfer learning}, e.g., by executing suitable grasps onto other objects with stem-like parts, such as the shown teapot. %i.e., the agent can use its knowledge from one task for a related problem
    In summary, these abilities enable \emph{few-shot problem-solving}.}
    \label{fig:cog_prereq}
\end{figure*}

\section{Neurocognitive foundations}
\label{sec:cognitive_background}
In the following, we propose that the complex problem-solving skills in biological agents can be distinctively characterised by particular cognitive abilities. 
In our perspective, these abilities depend on key cognitive mechanisms, including  abstraction, intrinsic motivation, and mental simulation.
% These mechanisms depend on certain neuro-functional prerequisites.
% \autoref{fig:cog_prereq} shows how complex structures as well as planning and reasoning abilities build upon forward and inverse models. 
% Together, cognitive abilities that we deem crucial for higher level intelligence become enabled, including few-shot problem solving and transfer learning. 
% Here we start with a characterization of these crucial cognitive abilities and then exhibit some of the key mechanisms and prerequisites needed to enable them. 
\autoref{fig:cog_prereq} outlines how these mechanisms may develop from forward and inverse models, as the fundamental neuro-functional prerequisites.
% Together, cognitive abilities that we deem crucial for higher level intelligence become enabled, including few-shot problem solving and transfer learning. 
% We start with a characterization of the crucial cognitive abilities and then exhibit the key mechanisms and prerequisites needed to enable them. 



\subsection{Cognitive abilities}
As distinct cognitive abilities, we focus on the following phenomenologically observable traits and properties.

\smallskip
\noindent
\textbf{Few-shot problem-solving} is the ability to solve unknown problems with few ($\lessapprox 10$) trials. 
\revv{
Zero-shot problem-solving is a special case of few-shot problem-solving, where no additional training at all is required to solve a new problem.}{R2-\ref{rev:r2:sugg:ref_few_shot}}
% 
% We refer to the ability of solving unknown problems with few trials as few-shot problem-solving. 
% In many cases, agents are able to solve new problems without any trial and error at all (one-shot or zero-shot problem-solving).
% If a problem can be solved ``on sight'', i.e., without any trial and error, we speak about zero-shot or one-shot problem-solving\footnote{We use the terms zero-shot and one-shot problem-solving interchangeably}.
% For simple problems, few-shot problem-solving is trivial. For example, catching a ball is usually a purely reactive behaviour that builds on a direct neural mechanism to map the observation of the flying ball to appropriate motor commands. Such problems are solvable with current computational RL methods\cite{Li2018_DeepRL_Overview}. 
% It involves solving difficult problems that require, e.g., using tools in new contexts. 
For example, a crow can use a stick as a tool for a novel food-access problem without further training (see \autoref{fig:crow_probsolving}), given it has previously solved related problems \cite{Gruber2019_CrowMentalRep}.
%For example, consider the aforementioned problem-solving example of the  crow\cite{Gruber2019_CrowMentalRep} (see \autoref{fig:crow_probsolving}). The crow knows how to use a stick as a tool without any further training, because it has previously solved related problems.
% Here we are interested in the cognitive abilities that enable few-shot problem-solving for such advanced problems. 
We identify two abilities that are most central for such problem-solving, namely transfer learning and decision-time planning (see \autoref{fig:cog_prereq}). 

\smallskip
\noindent
\textbf{Transfer learning}
 allows biological agents to perform few-shot pro\-blem-solving by transferring the solution of a previously solved task to novel, but analogous, unseen tasks \cite{Perkins1992}. This significantly reduces and sometimes eliminates the number of trials to solve a problem. 
 %Near transfer refers to the transfer of skills between domains or situations that are rather similar, e.g. learning to catch a ball and then catching other objects. In contrast, far transfer requires the transfer of more abstract solutions between different situations typically via abstract analogies.  
%Such analogies are determined by mappings between problems from different domains. 
% For example, consider an object transport problem with a robotic hand that involves the following sequence of three actions: [\concept{grasp(object)}, \concept{moveArm(goal)}, \concept{release(object)}]. Herein, \concept{grasp}, \concept{moveArm} and \concept{release} denote actions types and \concept{object} and \concept{goal} denote arguments passed to the action types. 
% The sequence of actions is analogous to a file movement problem on a computer that involves \concept{[cutInFolder(file)}, \concept{ navigate(targetFolder)}, \concept{pasteInFolder(file)}], with the obvious mappings between the action types and arguments. 

\revv{Some cognitive theories consider such \textbf{analogical reasoning} as a critical cornerstone of human cognition.}{R2-\ref{rev:r2:sugg:analogical_reasoning}, R3-\ref{rev:r3:bold_claims}} 
For example,%
% metaphors can be understood as mappings between analogous concepts in different domains\cite{Feldman2009_neural_ECG}.
it has been argued that analogies are used in mechanical inference, to understand a mechanical system by using knowledge from other domains\cite{Hegarty2004_MechReasMentalSim}.
Education theory suggests that human transfer learning improves when explicitly trained to identify analogies between different problems\cite{Klauer1989_AnalogyTransfer}.
%For example, conceptual metaphor theory\cite{Feldman2009_neural_ECG} understands metaphors as mappings between analogous concepts in different domains.
%In addition to evidence from linguistics, there is also significant evidence from education theory and research on mechanical reasoning that analogical reasoning improves problem-solving: 
%The Psychology of mechanical inference suggests that analogical knowledge about the dynamic properties of mechanical objects is often transferred between domains\cite{Hegarty2004_MechReasMentalSim}. 
%\revv{
%For example, knowledge about the effect created by a person jumping into a pool can be transferred to other mechanical problems that involve over-flooding water containers\cite{Hegarty2004_MechReasMentalSim}.}{R2-\ref{rev:r2:sugg:trans_learn_para}}
\revv{However, while humans seem skilful in applying analogies for problem-solving, it seems to be more difficult to discover new ones. 
For example, the phenomenon of functional fixedness describes the human problem-solving tendency to use objects only in the way they are traditionally used \cite{Duncker1945}.}{R3-\ref{rev:r3:controversial_theories}, R2-\ref{rev:r2:sugg:trans_learn_para}}
% \todo{Find more recent papers that underpin this further, i.e., search for papers > 2017 that cite the above papers from the 80/90ies and that have a related message.}

\smallskip
\noindent
\textbf{Goal-directed planning.}
Behaviour is traditionally divided into two categories: Stimulus-driven, \revv{habitual}{R2-\ref{rev:r2:sugg:habitual}} behaviour and goal-directed, planned behaviour\cite{Dayan2009, Dolan2013, ODoherty:2017}.
%\rev{Habitual behaviour refers to forms of reflexive control that are strongly automated, computationally efficient, and mainly learned from past reinforcements \cite{Dolan2013}.
%In contrast, planned behaviour refers to forms of reflective control, where future outcomes and actions are considered \cite{Dolan2013}.}{R2-\ref{rev:r2:habits}} 
Stimulus-response theories suggest that  most behaviour is learned from past reinforcements \cite{Dolan2013}. %learned by forming associations that were previously reinforced \cite{Thorndike}.
One of the main critics of this approach was Tolman, who showed
%However, this contradicts Tolman's research, 
% \cite{Dolan2013} and showing 
that rats can find rewards in a maze faster when they have visited the maze before, even if their previous visit had not been rewarded \cite{Tolman1930,Butz:2002c}.
% This implies that the rats had learned a cognitive map of the maze, using it to plan their behaviour once a reward was detected \cite{Butz:2002c}. %% wäre schön, wenn wir dieses Zitat wieder mit reinnehmen - es zeigt exakt mit einem lern-Modell, was der vorherige Satz aussagt.


\revv{Advances in AI and cognitive science have influenced one another to understand goal-directed planning.
An influential model for action control was the TOTE model \cite{Miller:1960}, where actions are selected based on an iterative, hierarchical feedback loop. Herein, a desired anticipated state is compared to the current sensory state to select the next action.
% Lashley \cite{Lashley1951} proposed that goal-directed planning requires access to a broader temporal context or \emph{schema} \cite{Botvinick:2004}.
%Building upon this model and related pioneering work on behavioural hierarchies \cite{Lashley1951}, 
Similar to TOTE, many recent theories view planning as a hierarchical process with different levels of abstraction \cite{Botvinick2014, Tomov2020, Wiener2003}.
%Thereby, humans seem to first plan high-level actions before considering actions at a finer granularity\cite{Wiener2003}.}
}{R2-\ref{rev:r2:sugg:planningclaims}, R2-\ref{rev:r2:sugg:agreement}, R3-\ref{rev:r3:bold_claims}, R3-\ref{rev:r3:circular_inspiration}, R3-\ref{rev:r3:controversial_theories:planning}}

\revv{But what kind of information is considered while planning?
%While such a sequential process of action selection remains popular to this day, it is not clear what kind of information is used for action evaluation and inference. 
Ideomotor theories of action generation \cite{Stock2004_Ideomotor} suggest that anticipated action effects determine action selection.
Accordingly, the Theory of Event Coding \cite{Hommel2001} claims that representations of actions and their effects are stored in a common code, whereby action effect anticipations can directly activate corresponding actions \cite{Hommel2001}.
%The Theory of Event Coding \cite{Hommel2001}, a prominent theory building upon ideomotor theories, claims that representations of actions and their effects are stored in a common code and that the anticipation of an action's effect directly induces a activation of the corresponding action \cite{Hommel2001, Hommel2009_Action}.
Various experimental evidence supports this link between action generation and effect prediction \cite{Hommel2001, Hoffmann:2003, Kunde:2007}.
%When action-effect-codes are learned on different levels of abstraction, planning can be realised by hierarchically predicting action effects on different time-scales and levels of abstraction \cite{Butz2016}.
%In order to form hierarchical encodings out of action-effect complexes, event-predictive process have been suggested to play a crucial role \cite{Zacks2007_EST,Butz:2021,Butz2017_MindBeing}.
%These processes essentially induce an inductive learning bias to integrate predictable interaction dynamics into compressed event-predictive structures, enabling the anticipation of final behavioural results without the need to simulate all intermediate details. 
% As a consequence, hierarchical, model-based, goal-directed planning becomes possible without the need to think through all the details of the individual event-respective steps \cite{Butz2017_MindBeing, Hommel2009_Action, Hommel2001, Kunde:2007}.
}{R2-\ref{rev:r2:sugg:planningclaims}, R2-\ref{rev:r2:sugg:agreement}, R3-\ref{rev:r3:bold_claims}, R3-\ref{rev:r3:circular_inspiration}, R3-\ref{rev:r3:controversial_theories:planning}}
\revv{Our supplementary \autoref{box:appendix:automatization} describes how the continuous learning of action-effect associations questions the traditional dichotomy between planned and habitual behaviour\cite{Dolan2013}.}{R2-\ref{rev:r2:habits}, R2-\ref{rev:r2:sugg:automatization}} 





%Habituation of behaviour, which is comparable to model-free policy optimization in reinforcement learning\cite{Botvinick2014,Dayan2009}, enables an agent to learn one particular skill in a controlled environment.
%However, complex problem-solving in a new or changing environment requires some form of prospective planning\cite{Butz2017_MindBeing, Dolan2013, Hoffmann:2003}.
%
%
%Over the last decades, more research has focused on understanding the mechanisms and representations involved in goal-directed planning.
%It is now generally agreed upon that, during planning, humans predict the effect of their actions, compare them to the desired effects, and, if required, refine their course of actions\cite{Hoffmann:2003,Kunde:2007}. 
%This is deemed to be a hierarchical process where the effects of actions on different levels of abstraction are considered\cite{Botvinick2014, Tomov2020}. 
%Thereby, humans tend to first plan high-level actions before considering actions at a finer granularity\cite{Wiener2003}.
%Hierarchical planning can dramatically decrease the computational cost involved in planning \cite{Botvinick2014, Dolan2013}.
%Additionally, hierarchical abstractions enable automatizing originally planned behaviour, thus further alleviating computational cost \cite{Dayan2009}.


%Biological agents often don't rely only on a reactive policy, but combine it with planning or plan verification. They achieve this by mentally comparing the anticipated outcome of their actions with their goal. In case the predictive anticipation reveals that reactive policy has undesired side-effects or does not lead to the goal, agents can refine the course of actions until their anticipation considers the goal achieved. \todo{Add literature and elaborate. Maybe TEC, but how does TEC relate to (mental) planning?}


\subsection{Cognitive mechanisms for transfer learning and planning}
Our survey suggests three critical mechanisms to enable planning and transfer learning, namely sensorimotor abstraction, intrinsic motivation, and mental simulation.


\textbf{Sensorimotor abstraction.}
% Humans think in terms of abstract mental concepts\cite{Barsalou2008_GroundedCognition}. 
\revv{According to theories of embodied cognition}{R3-\ref{rev:r3:controversial_theories:embodiment}}, abstract mental concepts are inferred from our bodily-grounded sensorimotor environmental interaction experiences \cite{Barsalou2008_GroundedCognition,Butz2017_MindBeing,Butz2016,Pulvermuller:2010}. 
%Thus, a crucial mechanism required for both transfer learning and efficient goal-directed planning, is the formation of abstract representations from sensorimotor information.
% Martin: ich sehe nicht, wie das folgen soll - würde ich hier rausnehmen: 
% Therefore, \emph{sensorimotor abstraction} is a crucial mechanism required for both transfer learning and goal-directed planning.
Herein, we differentiate between \emph{action abstraction} and \emph{state abstraction}.
%
Action abstractions refer to a temporally extended sequence of primitive actions, sometimes also referred to as options\cite{Sutton1999_options} or movement primitives\cite{Flash2005_AnimalMotorPrimitives, Schaal_2006}.
For example, \emph{transporting an object} is as an action abstraction since it is composed of a sequence of more primitive actions, such as \textit{reaching} and \textit{lifting} (see \autoref{fig:cog_comp}). %, and \textit{transporting} (see \autoref{fig:cog_comp}).
%For example grasping an object can be seen as an action abstraction since it is composed of a sequence of multiple more primitive actions, such as reaching out for an object, then grasping it, etc.
% The elementary actions that compose an action abstraction are typically rather loosely defined through their effects.
% For example, we can tell that a robot arm we have never seen before is grasping an object, even though the anatomy, the unfolding control algorithms, and the involved motor commands may largely vary from our human ones.
%
State abstractions refer to encoding certain parts of the environment while abstracting away irrelevant details.
Accordingly, state abstractions may decompose a scene into task-critical aspects, such as graspability, containment, or hollowness.
%For example, a simple state abstraction may simply encode the presence of a particular object, such as a \textit{wine glass}. % or some form of \textit{container}.
%Moreover, state abstraction may decompose the scene and relevant entities into task-critical aspects, such as graspability, solidity, or containment.
For example, both \textit{wine glasses} and \textit{tea pots} have the property of being a \textit{container} and being \textit{graspable} (see \autoref{fig:cog_comp}).
Meanwhile, a \textit{container} implies \textit{hollowness}, etc.---illustrating the hierarchical and \textbf{compositional} nature of such abstractions. 
%A simple example of a state abstraction is a code that specifies whether a certain type of object is present in a scene. 
%State abstractions can be hierarchically structured:
%A single object can be subdivided into a partonomy, i.e., a hierarchical organization of its parts and their spatial relationship (see \autoref{fig:cog_comp}) \cite{Minsky1974, Zacks2001_EventStructure}.
%Objects can also be organized taxonomically, reflecting a hierarchical relationship that focuses on particular conceptual aspects \cite{Minsky1974, Zacks2001_EventStructure}.
%For example, an affordance-oriented \cite{Gibson:1979} taxonomy of beverage containers could classify \textit{wine glasses} and \textit{beer mugs} both as \textit{drinking vessels}, while a \textit{teapot} would be classified as a \textit{pot} instead.
%Meanwhile, \textit{beer mugs}, \textit{wine glasses}, and \textit{teapots} are all \textit{graspable containers}.

% State and action abstractions are not mutually exclusive and may cross-reference each other. For instance, a  state abstraction that describes whether an object is graspable relies on the existence of the action abstraction \emph{grasp}. %, and encodes whether an object is a suitable target for grasping.

% Thus, a key property of conceptual abstractions is their \textbf{compositionality}.
%Conceptual abstractions and cross-references to other conceptual abstractions within imply a representational key property: \textbf{compositionality}.
%The formal compositionality principle is closely related to linguistics.
%It states that an expression or representation is compositional if it consists of subexpressions, and if there exist rules that determine how to combine the subexpressions \cite{Szabo:2020}. 
%The Language of Thought theory\cite{Fodor:2001} transfers the compositionality principle from language to abstract mental representations, claiming that thought must also be compositional. 
%\revv{For example, \citet{Frankland2020_SearchLoT} state that humans are easily able to imagine previously unseen situations and objects by composing their known constituents. The authors refer to the \emph{golden pavements} and \emph{ruby walls} imagined by Scottish philosopher David Hume in \emph{A Treatise of Human Nature}.}{R2-\ref{rev:r2:sugg:hume}}
%\revv{It is still being debated whether abstract combinatorial mental concepts, upon which the Language of Thought builds, are represented as local symbols or by means of distributed encodings  \cite{Hummel2011_Symbols_Neural}. However, the important point to make is that there is evidence for the existence of combinatorial generalization in both symbolic and connectionist literature.
% For example, recent neuroimaging techniques indeed revealed that the compositionality of mental representations can actually be observed in neural codes.
%For example, \citet{Haynes2015_CompositionalNeuroRep} show that the neural codes in the ventrolateral prefrontal cortex, which encode compound behavioural rules, can be decomposed into neural codes that encode their constituents. 
%}{R3-\ref{rev:r3:controversial_theories:LoT}} 
% Similar results have been obtained for neural codes that represent food compositions\cite{Barron2013_CombinedChoicesConcepts}.

Cognitive linguistics and related fields suggest that abstractions benefit from compositionality \cite{Feldman2009_neural_ECG}. 
Formally, expressions are compositional if they are composed of subexpressions and rules to determine the semantics of the composition. 
The Language of Thought theory\cite{Fodor:2001} transfers the compositionality principle from language to abstract mental representations, claiming that thought must also be compositional. 
For example, humans can easily imagine previously unseen images by composing their known constituents from linguistic descriptions \cite{Frankland2020_SearchLoT}.
\revv{It is still being debated whether the abstract mental representations are encoded as local symbols or by means of distributed encodings \cite{Hummel2011_Symbols_Neural}, but in both cases there is evidence for the existence of combinatorial generalisation.
For example, \citet{Haynes2015_CompositionalNeuroRep} show that the neural codes in the ventrolateral prefrontal cortex, which encode compound behavioural rules, can be decomposed into neural codes that encode their constituents.}{R3-\ref{rev:r3:controversial_theories:LoT}}


For sensorimotor abstractions, the rules of composition need to be flexibly inferred by our minds to form plausible environmental scenarios in accordance with our world knowledge \cite{Butz2016,Gaerdenfors:2014,Lakoff1999}.
%Compositional rules for sensorimotor abstractions are flexibly inferred by our minds in an attempt to form plausible environmental scenarios in accordance with our world knowledge \cite{Butz2016,Gaerdenfors:2014,Lakoff1999}.
Such \textbf{common sense compositionality} makes abstractions applicable in meaningful manners. 
The filling in of an abstract component (e.g., the  target of a grasp) is constrained towards applicable objects (e.g., a graspable object such as a teapot), as depicted in \autoref{fig:cog_comp}.
From an algorithmic perspective, common sense compositionality brings enormous computational benefits:
Abstractions, e.g., a grasping-encoding, are much more economically if they can be applied in various situations, e.g. for different grasping targets.
Common sense compositionality essentially simplifies the identification of analogies by enabling morphisms between representations, an advantage well-known in cognitive theories of creativity and concept blending\cite{Eppe2018_AIJ_Blending,Turner2014} (cf. supplementary \autoref{box:appendix:compositionality-example}).


%In the remainder, we will refer to this type of representation-independent compositionality as \textbf{common sense compositionality}. That is, compositional rules that are grounded in and flexibly inferred by our intuitive knowledge about the world. %, without asking (yet) for how these rules are encoded.
%This common sense compositionality essentially enforces that our minds attempt to form plausible environmental scenarios and events that unfold within given conceptual information about a particular situation\cite{Butz2016,Gaerdenfors:2014,Lakoff1999}. % Butz:2008h details that in a related manner focusing on the "anticipatory drive"
% Consider the processes that unfold when understanding a sentence like ``He sneezed the napkin off the table''.
% % For example, compositionality allows one to correctly understand previously unheard sentences like ``He sneezed the napkin off the table''. 
% Most people have probably never heard or used this sentence before, but everyone with sufficient world and English grammar knowledge can correctly interpret the sentence, imagining a scene wherein the described event unfolds\cite{Butz2016}. 
%
%
%Common sense compositionality makes abstractions applicable in meaningful manners, by constraining the filling in of an abstract component (e.g., the  target of a grasp) towards applicable objects (e.g., a graspable object such as a teapot), as depicted in \autoref{fig:cog_comp}.
%Note the awkwardness -- and indeed the attempt of the brain to resolve it -- when disobeying common sense compositionality, such as when stating that `The dax fits into the air' or `grasping a cloud' \cite{Butz2016}.
% \autoref{fig:cog_comp}) illustrates compositional action and state abstractions in the context to reaching, grasping, lifting, and transporting objects. 

% Common sense compositionality indeed may be considered a hallmark and cornerstone of human creativity, as has been (indirectly) suggested by numerous influential cognitivists \cite{Barsalou2008_GroundedCognition,Fillmore1985,Lake2017,Lakoff1999,Sugita:2011,Turner2014,Werning:2012}.
%Compositionality enables the application of an abstractions in previously unseen situations.
% As a result, an abstraction can be applied to novel situations.
%For example, once one has mastered the ability to grasp, one can grasp objects of various shapes as long as they have certain properties that make them graspable (see 
%
%The key aspect of both state and action abstractions is their \textbf{compositionality}.
%
%Besides that properties of an object, or its parts can be described. The \concept{container}-property, for example, is such a state abstraction\cite{Butz2016} describing particul.
%Here several constraints have to be met: There have to be two objects, one smaller than the other with the smaller one being placed inside the larger one, etc.
%However, only a few aspects of the state space are constrained.
%For example the size of the container can be arbitrarily large, as long as the contained object can still fit inside.
%
%We define action abstractions as a sequence of motor commands that follow certain constraints on the type of motor commands involved and the order of elementary commands.
%In related disciplines, such as kinematics and robotics, analogous concepts are found to describe extended sequences of actions, such as movement primitives, behavioural primitives or options\cite{Flash2005_AnimalMotorPrimitives, Sutton_1999_options}.
%For example, consider grasping an object as an abstract action.
%The grasping is composed of multiple motor commands, such as the extension of ones arm and the closing of ones fingers.
%Thereby the order of these motor commands is fixed: Closing the grip needs to follow the reaching motion.
%The elementary motor commands that compose an action abstraction are loosely defined through their effects.
%For example, one requirement for the grasping abstraction is that the end-effector needs to move towards the target.
%However, the exact motor commands and their duration are not relevant for the abstract action representation.
%For example, we can clearly tell that a robot arm that we have never seen before is grasping an object, even though the anatomy and the involved motor commands may largely vary to our human ones.
%
%We refer to state abstractions as a set of sensory states defined over some constraints.
%\concept{An object is inside a container}, for example, is such a state abstraction.
%For this state abstraction we can list several constraints\cite{Butz2016}:
%For example, it is required that there are two objects present, with one object being smaller than the other one.
%Besides that, the bigger container object needs to be, at least partially, hollow and the smaller object needs to be positioned within the hollow space of the container object.
%However, the constraints limit only a few aspects of the state space, while still allowing certain degrees of freedom.
%For example the size of the container can be arbitrarily large, as long as the contained object can still fit inside. % within its hollow space.
%
%
%

% For a review on further neuroscientific evidence for compositional representations, we refer to \citet{Frankland2020_SearchLoT}. 

\begin{figure}
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/ActionAbstraction_Box_a.pdf}
\end{minipage}
\hfill
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/StateAbstraction_Box_b.pdf}
\end{minipage}
\hfill
\begin{minipage}{.32\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/SensorimotorAbstraction_Box_c.pdf}
\end{minipage}
\caption{Compositional action and state abstractions. \emph{Action abstractions} describe a sequence of more primitive actions (a.). \emph{State abstractions} encode certain properties of the state space (b). Their \emph{compositionality} enables their general application, by instantiating abstract definitions (the graspable target of reaching), with a specific object (teapot) (c.). \label{fig:cog_comp}}
\end{figure}

% \todo{Can we find evidence from neuroscience and cognitive sciences that underpin the below algorithmic considerations?}

%From an algorithmic perspective, common sense compositionality yields benefits for analogical reasoning and planning. 
%It simplifies the identification of analogies because it enables compositional morphisms between representations. 
% This reduces the space of possible problem-morphisms and, therefore, the space of possible analogies.
%This advantage is well-known in cognitive theories of creativity, e.g., concept blending\cite{Eppe2018_AIJ_Blending,Turner2014}, where the search for analogies is a computational bottleneck.
%%For example, consider two problem descriptions that both involve $n_a$ action types (e.g. grasping, pushing, lifting) with one argument and $n_o$ possible arguments (e.g. ball, block, stick). 
%%If the action representations are not compositional, there exist $n_a \cdot n_o$ atomic action representations, which results in $(n_a  \cdot n_o)^2/2$ possible morphisms. 
%%In contrast, if the action representations are compositional, only morphisms between the action types and morphisms between the objects are required, reducing the search space over action morphisms to $(n_a^2 + n_o^2)/2$. 
%%
%% (possible arguments) and $n_r$ binary relations between objects. 
%% The number or possible (grounded) actions is $n_a^{grnd} = n_a \cdot n_o$, and the number of possible (grounded) binary relations is $n_r^{grnd} = n_r \times n_o^2$. 
%% If the action and relation representations are not compositional, i.e., if we consider the grounded representations, this results in $n_r^{grnd}^2 + n_a^{grnd}^2 = n_a^2 \cdot n_o^2 + n_r^2 \times n_o^4 = $ possible morphisms. Whereas if we consider compositional morphisms (between the non-grounded representations) there are only $n_a^2 + n_r_^2 + n_o^2$ possible morphisms. 
%%
%% For example, consider two problem descriptions, each consisting of $n_a$ action types with one argument, $n_o$ object types (possible arguments) and $n_r$ binary relations between objects. 
%% The number or possible (grounded) actions is $n_a^{grnd} = n_a \cdot n_o$, and the number of possible (grounded) binary relations is $n_r^{grnd} = n_r \times n_o^2$. 
%% If the action and relation representations are not compositional, i.e., if we consider the grounded representations, this results in $n_r^{grnd}^2 + n_a^{grnd}^2 = n_a^2 \cdot n_o^2 + n_r^2 \times n_o^4 = $ possible morphisms. Whereas if we consider compositional morphisms (between the non-grounded representations) there are only $n_a^2 + n_r_^2 + n_o^2$ possible morphisms. 
%%
%Similarly, compositional state- and action representations for goal-directed planning lead to a lower computational complexity, because action and object types can be flexibly combined as long as critical properties match.
%For example, consider the combinatorial explosion that is involved in the physical interaction with objects. An object interaction can be represented as a composition of action type (e.g. grasping, pushing, lifting) and object type (e.g. ball, block, stick). To represent all possible actions, it is more economical to use three action type representations and three graspable object type representations plus a composition operation, instead of using nine separate representations that represent each possible combination of object and action separately.
%Along these lines, action grammars have been proposed, which systematically form an effect-oriented taxonomy of tool-object interactions \cite{Worgotter:2013}. 
%As a result, common sense compositionality enables the utilisation of objects as tools in innovative manners---when, for example, utilising a stone as a hammer \cite{Butz2017_MindBeing,Lakoff1999}. 
%Moreover, it enables drawing analogies across domains---when , for example, talking about ``holding onto a thought'' for later utilisation.
%
%Common sense compositionality thus seems to be key for truly intelligent artificial systems.
%We propose that apart from the addition of suitable inductive learning biases, such as event-segmentation tendencies \cite{Butz2016,Butz2017_MindBeing,Butz:2020,Shin:2020tsi,Zacks2007_EST}, suitably targeted intrinsic motivation and the ability to play out mental simulations are of critical importance.

\smallskip
\noindent
\textbf{Intrinsic motivation} affects goal-directed reasoning by setting intrinsically motivated goals. % affects goal-directed reasoning and planning because it sets intrinsically motivated goals that an agent may aim to achieve. 
% The most basic behaviour of biological agents purely strives for satisfying homeostatic needs, such as hunger or thirst. However, advanced behaviour, such as exploration and play, seems to be partially decoupled from the primary biological needs.
From a cognitive development perspective, the term \emph{intrinsic motivation} was coined to describe the ``inherent tendency to seek out novelty, [...] to explore and to learn''\cite{RyanDeci2000}. % TODO - should add page numbers here
Here, \emph{intrinsic} is used in opposition to extrinsic values, which are rather associated with the satisfaction of needs or the avoidance of undesired outcomes \cite{Friston2015}.
% This term is now widely used in developmental robotics and reinforcement learning to describe functions that reward learning progress and exploration as opposed to rewards given by the environment (e.g.,\cite{Oudeyer2007,Schmidhuber2010}).
Intrinsic motivations induce a general exploratory behaviour, curiosity, and playfulness.
%Simple exploratory behaviour can even be found in worms, insects, and crustaceans \cite{Pisula2008} and may be elicited by rather simple tendencies to wander around or evade overcrowded areas. %while being satiated or an inborn tendency to evade overcrowded areas.   
\revv{Curiosity refers to information gain-oriented exploratory behaviour\cite{Berlyne1966, Loewenstein1994, Oudeyer2007}.
%Combined with developing common sense compositionality, this drive can elicit hypothesis testing behaviour even by means of analogy making. 
Curiosity is closely related to playfulness, where novel interactions are tried-out in a skill-improvement-oriented manner. Playfulness can be observed in certain intelligent animal species such as dogs and corvids\cite{Pisula2008}.}{R2-\ref{rev:r2:sugg:intrinsic_motivation}} 
%Exploratory behaviour is phylogenetically one of the oldest forms of behaviour that is found in worms, insects, and crustaceans as well as in higher animals such as birds and mammals .
%Through exploration, biological agents acquire new knowledge and skills, which helps them to improve their overall problem-solving abilities by (1.) building representations of an unknown environment and (2.) discovering better solutions for familiar problems.
% Along similar lines, playfulness in animals can be considered an intrinsic motivation.
% In contrast to exploration, 
%Play is thought to encourage practicing skills in a safe or simplified environment during earlier stages of development.
%Hence, by playing, biological agents can refine their non-optimized skills and, thus, improve their performance for a specific set of problems.

%Current neurocognitive theories suggest that neural forward models are the central functional prerequisite for curiosity-driven intrinsic motivation.



%Curiosity causes intrinsic motivation and is, therefore, deemed to heavily determine the overall behaviour of biological agents\cite{Oudeyer2007}. By being curious, biological agents acquire new knowledge and skills, which helps them to improve their overall problem-solving capabilities.  

\smallskip

\noindent
\textbf{Mental simulation} describes the ability of an agent to anticipate the dynamics of its environment on various representational levels. %meanwhile,
%enables biological agents to reflect on and to anticipate the dynamics of its environment on various representational levels in the past, present, and future, and even fully hypothetically.
For example, \emph{motor-imagery} is deemed to enable athletes to improve the execution of challenging body movements (e.g. a backflip) by mentally simulating the movement\cite{Jeannerod1995_MentalImageryMotor}, and engineers can rely on mental simulation when developing mechanical systems \cite{Hegarty2004_MechReasMentalSim}. 
%On the reasoning side, consider human engineers who rely on  mental simulation when developing mechanical systems, such as pulleys or gears.
%The simulation involves visual imaginations but also includes non-visual properties like friction and force \cite{Hegarty2004_MechReasMentalSim}. 
Several researchers suggest that mental simulation also takes place on higher reasoning levels. For example, \citet{Kahnemann1982_MentalSim}, \citet{Wells1989_MentalSimCausality}, and later \citet{Taylor1998_MentalSim} report how mental simulation improves planning of future behaviour on a causal conceptual level. 
% \todo{Find some more recent papers (e.g. 2018 or younger) to underpin all this. Write more on planning.}

\smallskip

\subsection{Forward-inverse models as functional prerequisites}

Sensorimotor abstraction, intrinsic motivation, and mental simulation are complex mechanisms that demand a suitable neuro-functional basis. 
% Too little is known to provide here a full summary of the neural foundations of these prerequisites. 
%However, from a functional cognitive point of view, it is possible to describe these mechanisms with two simple functional prerequisites, namely 
\rev{We propose that this essential basis is constituted by forward and inverse models \cite{Stock2004_Ideomotor}. % \cite{Wolpert1998_ForwardInverse}. % Butz:2008h (anticipatory drive - sollte hier mit rein)
Forward models predict how an action affects the world, while inverse models determine the actions that need to be executed to achieve a goal or to obtain a reward.}{R2-\ref{rev:r2:wolpert:kawato}}
%Note that inverse models may be implicitly inferred from the available forward models, but more compact inverse models, which are closely related to habits and motion primitives, certainly foster the proficiency of particular behavioural skills further \cite{Barsalou2008_GroundedCognition,Butz2017_MindBeing,Dezfouli:2014,Schaal_2006}. % Butz:2007g -- diese Psch.Rev. paper gibt eben auch ein Review zu dem drüber ausformulierten Punkt.

\smallskip
\noindent
\textbf{Forward-inverse models for mental simulation.}
To perform mental simulation, an agent needs a forward model to simulate how the dynamics of the environment behave, possibly conditioned on the agent's actions.
%However, even when equipped with a well-predicting forward model, the consideration of all possible actions and action sequences quickly becomes computationally intractable. 
However, the consideration of all possible actions and their consequences quickly becomes computationally intractable. 
% it is impossible to consider all possible actions at the agent's disposal as candidate actions.
%It is impossible to consider all actions at an agent's disposal as candidate actions so solve a certain problem. 
Hence, action-selection requires more direct mappings from state and desired inner mental state to potential actions. 
This can be accomplished by an inverse model or behaviour policies, which generate candidate actions for accomplishing a current goal.
%This is accomplished by inverse models. 
%In RL, inverse models are represented as behaviour policies.
%Selecting actions can happen in a reflex-like manner on the motor level but it can also serve as a heuristic to generate candidate actions for accomplishing a current goal. 
% In that case, a biological agent uses its inverse model to generate candidate actions, and to simulate them for planning its goal-directed behaviour. 
%For example, when designing a new mechanical system, engineers have an intuition about how to put certain mechanical parts together, depending on the goal function they want to achieve with the system. Based on their intuition, they mentally simulate and verify the functioning of the mechanical system\cite{Hegarty2004_MechReasMentalSim}. 

\smallskip

\noindent
\textbf{Forward-inverse models for intrinsic motivation.}
Forward and inverse models are also needed for intrinsic motivation. 
For example, prediction error minimisation has been demonstrated to be a useful intrinsic reward signal to model curiosity\cite{Kaplan:2004, Schmidhuber2010, Oudeyer2007}.
%\citet{Kaplan:2004} build on this idea and propose to use learning progress, i.e., the improvement of an internal predictive model, as intrinsic reward to incentivize visiting currently unpredictable situations.
% Once the agent learned enough from these situations, resulting in a stagnation of the learning progress, other situations become more interesting\cite{Oudeyer2018_CompuCuriosityLearning}. 
% This approach also accounts for situations that are unpredictable per se, such as sensory noise: These are ignored when using learning progress as intrinsic reward\cite{Schmidhuber:2010}.
%This was demonstrated in a playground experiment\cite{Kaplan:2007}, where a robot was placed on baby play mat and could manipulate various toys.
%The robot first spent time with situations that are easier to learn before progressively focusing on more difficult situations - showing the emergence of developmental stages under this learning regime\cite{Kaplan:2007, Oudeyer:2018}.
%The formalizations of intrinsic motivation sparked a large interest in the fields of developmental robotics and reinforcement learning and led to various novel versions of intrinsic motivation, such as predictive information maximization\cite{Martius:2013}, or intrinsically motivated goal exploration processes\cite{Forestier:2017}. %, that all derive intrinsic reward functions from forward model-based measures. 
%All of these approaches require some form of forward model, such that learning progress, prediction errors or related measures can be quantified.
Similarly, Friston et al.~propose that intrinsically motivated behaviour emerges when applying \emph{active inference}\cite{Friston2011, Friston2015}, i.e., the process of inferring actions to minimise expected free energy, which includes approximations of anticipated uncertainty \cite{Friston2010, Friston2015}. 
%Active inference describes the process of inferring actions to minimize expected free energy, which includes approximations of anticipated uncertainty \cite{Friston2010, Friston2015}. 
The authors argue that active inference can lead to epistemic exploration, when an agent acts out different behaviour to reduce anticipated uncertainty about their forward predictions \cite{Friston2015, Oudeyer2018_CompuCuriosityLearning}.
%Active inference describes the process of inferring actions to minimize expected free energy, which includes approximations of anticipated surprise\cite{Friston2010, Friston2016}. 
%Free energy is decomposed into various sources of uncertainty.
%One part is uncertainty about future states or outcomes given a certain sequence of actions \cite{Friston2015}. %certain policy\cite{Friston2015}.
%The agent strives to reduce this uncertainty, and with it overall expected free energy, by activating the actions that cause the uncertainty.
%Hence, active inference can lead to epistemic exploration, where an agent acts out different behaviour to learn about its consequences\cite{Friston2015, Oudeyer2018_CompuCuriosityLearning}.
%Here, the forward model is required to predict future states given an action, and also to estimate the uncertainty of the prediction.
\rev{However, active inference and the free energy principle has been criticised as overly general, and its falsifiability has been questioned\cite{Colombo:2018}.}{R3-\ref{rev:r3:bold_claims}, R3-\ref{rev:r3:controversial_theories}}
%\rev{However, it needs to be noted that Friston's Free Energy Principle has been critized for being too general and its epistemic status has been questioned \cite{Colombo:2018}.}{R3-\ref{rev:r3:bold_claims}, R3-\ref{rev:r3:controversial_theories}}

\smallskip
\noindent
\textbf{Forward-inverse models for abstraction and grounding.}
Over the last decade, various theories including predictive coding\cite{Huang2011}, the free energy principle\cite{Friston2010}, and the Bayesian brain hypothesis\cite{Knill2004}, have viewed the brain as a generative machine, which constantly attempts to match incoming sensory signals with its probabilistic predictions\cite{Clark2013}.
Within these frameworks, prediction takes place on multiple processing hierarchies that interact bidirectionally:
Top-down information provides additional information to predict sensory signals, while bottom-up error information is used to correct high-level predictions \cite{Clark2016_SurfUncertainty}.
% Thereby, representations of states and features of the world develop as generative models. 
%Meanwhile, future states are predicted in a probabilistic manner\cite{Clark2013}.
\citet{Butz2016} proposes that this hierarchical processing leads to the emergence of abstract, compositional encodings on higher processing levels, e.g., a container-concept, which enable predictions of lower-level features, e.g., the occlusion and transport of a contained object.
 % or its position changing when moving the container.
%On lower processing levels, actual incoming sensorimotor signals are predicted, while on higher levels more abstract, conceptual and compositional predictive encodings emerge\cite{Butz2016}.
%In this way, rather complex state abstractions, such as the aforementioned \concept{container}-concept, can form. 
%As a result, high-level predictions, e.g., of an object being within a container, enable predictions on lower levels.
%For example, consider the  prediction of sensory information about how an object's position will change over time while it is occluded.
Event Segmentation Theory (EST)\cite{Zacks2007_EST}  makes the role of forward predictions for learning sensorimotor abstractions even more explicit:
According to EST, transient prediction errors are used to segment the continuous stream of experience into conceptual event-encodings, as detailed in the supplementary \autoref{box:appendix:EST}.








==> v2/conclusionShort.tex <==
\section{Conclusion}
\label{sec:conclusion}
Our review provides an overview of the cognitive foundations of hierarchical problem-solving and how these are implemented in current hierarchical reinforcement learning architectures.
% As a benchmark example, we refer to recent results from animal cognition \cite{Gruber2019_CrowMentalRep}, demonstrating how a crow develops mental representations of tools to solve a previously unseen food-access problem at the first trial (see \autoref{fig:crow_probsolving}). 
Herein, we consider few-shot problem-solving as the ultimate ability of intelligent beings that learn to solve causally non-trivial problems with as few trials as possible. 
As our main research question, we ask for the computational prerequisites and mechanisms to enable problem-solving for artificial computational agents on the level of intelligent animals. 
We further pose the challenge to integrate the different mechanisms. 

We appreciate that the cognitive theories we summarise are often contentious and controversial, as indicated in the \nameref{sec:cognitive_background} section. 
However, in our discussion, we show that the particular combination of the described theories have the potential to yield algorithmic synergies. 
% For instance, a forward model is highly synergistic because it enables intrinsic motivation, self-supervised abstraction, decision-time planning and background planning. 
\rev{
% The abstract concept of a forward model that we describe in this article does not presuppose any hardware constraints. Therefore, the synergies it creates are agnostic to the underlying computational hardware and apply to \emph{in vivo} (biological) as well as to \emph{in silico} (computational) implementations. 
In other words, we reason that if a particular mechanism is useful for computational architectures, then it is very likely to be beneficial for biological cognitive systems as well, and vice versa. 
In this way, cognitive sciences and artificial intelligence inspire each other, and they will hopefully converge to novel insights that are relevant for both fields and useful for the future of AI and humanity.}{R3-\ref{rev:r3:circular_inspiration}}
% Our article does not provide a solution to all problems of hierarchical reinforcement learning, but it provides guidelines and proposals for future research to address major remaining challenges. 

% Our research provides four main contributions. First, we performed a literature survey and a top-down structuring of cognitive abilities, mechanisms, and prerequisites for few-shot problem-solving (see \autoref{fig:cog_prereq}). Second, we reviewed recent hierarchical reinforcement learning architectures to identify whether and how the existing approaches implement the prerequisites, mechanisms, and abilities towards few-shot problem-solving (see \autoref{tab:hrl_properties}).
% Third, we identified four major shortcomings in state-of-the-art computational approaches, based on our review. 
% Fourth, we identified the underlying computational challenges that arise when integrating the cognitive mechanisms, and, as an outlook, we sketched-out proposals to address them.


% Three of these shortcomings are based on the lack of hierarchical forward models, but we also identify a lack of hierarchical reinforcement learning approaches that perform state abstraction, and we reveal a lack of approaches that exploit compositional representations. 
% The development of hierarchical forward models is particularly important because this potentially enables compositional abstraction to address the other gaps in the state of the art.
% In addition, hierarchical forward models are a critical prerequisite also for curiosity-driven intrinsic motivation and mental simulation.

% Nonetheless, we were able to identify several methods that address these gaps in the state of the art in isolation. 
% Not seeing any major reason why these approaches could not be integrated, we suggest that most of the tools to realise higher levels of intelligent behaviour in artificial agents have already been investigated. 
% The key is to combine them effectively. 
% This demonstrates significant potential to develop intelligent agents that can learn to solve problems on the level of intelligent biological agents.



==> v2/glossary_box.tex <==
\begin{infobox}[Glossary]
\label{box:appendix:glossary}


% \begin{tabular}{p{2.5cm} l}
% \textbf{Decision-time planning}     &  blablabla\\
% \textbf{Background planning}     &  blablabla\\
% \textbf{Abductive search}     &  blablabla\\
% \textbf{Intrinsic motivation}     &  blablabla\\
% \textbf{State abstraction} & as;fldkj \\
% \textbf{Compositional representation} & Sasfsf \\
% \textbf{Transfer learning} & Sasfsf \\
% \textbf{Inductive bias} & Sasfsf \\
% \textbf{Event segmentation} & Sasfs f \\
% \textbf{Event segmentation} & Sasfsf \\
% \textbf{Epistemic drive} & Sasfsf 
% \end{tabular}
\rev{
\textbf{Decision-time planning } is a search process over different sequences of potential actions and consequently anticipated changes in the world.
The aim is to determine the best possible sequence of actions and immediate next action to reach a specified goal, to satisfy internal motivational drives, or to maximize a reward or minimize a cost function. 
% , where the agent predicts how the actions change the world. The purpose of decision-time planning is to determine the best possible next action with respect to a specific goal, intention, reward or cost function. 


\noindent \textbf{Background planning} refers to simulating the execution of actions, for the purpose of generating samples for training a behavioural policy. 
In contrast to decision-time planning, background planning does not necessarily happen just-in-time before action execution. It is rather similar to dreaming, in the sense that it simulates action executions to train a behaviour or policy during physically idle times. This reduces the amount of required real-world actions to train a policy, avoids catastrophic forgetting, and fosters selective knowledge consolidation.

\noindent \textbf{Intrinsic motivation}
describes a motivational system that rewards behaviour primarily based on internal goals rather than for some external rewards. 
Here, internal goals refer to all goals that highly depend on subjective, internal representations.
External rewards refer to all rewards found in the environment and are somewhat independent of the subject.
We consider the drive for exploration, curiosity, and playfulness intrinsic motivations. 

% \noindent \textbf{Inference-appropriate state abstraction}
% \noindent \textbf{Inference-fitted state abstraction}
\noindent \textbf{State abstraction}
refers to mapping a lower-level state representation to a higher-level representation.
For instance, high-dimensional raw sensor data are low-level partial state representations, which can be abstracted to high-level discrete symbolic representations\cite{Eppe2019_planning_rl} or low-dimensional continuous vectors produced by convolution and pooling layers in neural networks\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}.


\noindent \textbf{Action abstraction}
refers to the process of generalizing an action representation. 
For example, the index or label of a context-independent behavioural policy or movement primitive (e.g. \concept{grasp(object)} is an abstract action representation because it points to a much more specific low-level action model, namely the actual policy used to execute the context-specific low-level motor-commands. 

\noindent \textbf{Inference-fitted abstraction} is abstraction such that each representational layer is \emph{appropriate for the level of inference} to be performed on that layer. 
Hence, many approaches based on convolutional neural networks are not inference-fitted because the same output of the convolution is passed to all hierarchical RL layers. Therefore, all hierarchical RL layers operate on the same preprocessed state representation, and it is unlikely that the representation is the best fit for all levels of inference.
In contrast, utilizing low-level raw sensor data as appropriate state representations for the low-level reinforcement learning layer and propositional symbolic high-level representations to perform high-level inference  with an action planner is inference-fitted: Here, the low-level control relies on low-level data while the high-level inference performs more effectively with high-level representations, which do not contain all the details of the low-level representation. 

\noindent \textbf{Compositional representations} are data structures that consist of sub-data structures that are subject to semantic rules, which specify how the sub-data structures may be combined. For example, this sentence itself is a data structure that consists of words and grammatical constructions, which are sub-data structures. The sentence is compositional because there exist grammatical rules that are necessary to understand the sentence. Another example for a compositional representation is a disentangled vector representation, where the individual slots of the vector represent individual properties (e.g. angle, colour, rotation or shape of an object). In this case, the semantic rules determine the meaning of each individual slot of the vector. 


\noindent \textbf{Mental simulation}
refers to the general ability to anticipate future states of the agent and its environment, where ``states'' can both refer to concrete observations but also to abstract properties of the environment. Note that the temporal reference ``future'' is relative to an assumed starting point in time and independent of the time when the mental simulation is performed. For example, an agent can perform counter-factual mental simulation to anticipate how a past starting state may have had developed differently if the agent had executed a hypothetical course of actions that is different from the actions it actually applied.

\noindent \textbf{Transfer learning}
is a broad term that generally refers to transferring knowledge acquired in a specific context to a new context. 
The term ``transfer'' is partially misleading in the sense that knowledge is usually not transferred between different agents, but rather re-applied in different contexts. Furthermore, transfer learning usually means that learned knowledge is transferred, and not that the transfer is learned. 
In robotic problem-solving, the context is usually a specific problem, and the knowledge is a computational model that provides a solution to it. In RL, the computational model is usually a learned policy, but it can also be a forward model or other data structures. 
For example, consider a policy that has been successfully trained to solve one or more source problems. If the same policy can be re-applied to solve a new unknown target problem the transfer is successful. 
\citet{Perkins1992} propose a distinction between near and far transfer. 
 Near transfer refers to the transfer of skills in similar domains and situations, e.g. using the knowledge from learning to grasp a glass to grasping other objects. Far transfer typically refers to the transfer of solutions between different situations via abstract analogies.


% We distinguish here between near transfer the 

\noindent \textbf{Inductive bias}
refers to a set of assumptions to constrain a learning algorithm. 
% Typically, there are many possible solutions to a problem. With inductive biases, one can incentivize a learning algorithm ``to prioritize one solution (or interpretation) over another'' \cite{Battaglia:2018}. 
% Ideally, inductive biases encode knowledge about the problem and help the algorithm to generalize better to novel data.
Ideally, inductive biases encode general knowledge that is independent of the specific problem so solve, helping the algorithm to generalize better to novel data.
For example, curiosity and other intrinsic motivation models are inductive behavioural biases that potentially improve the data exploration of an agent. 
On the other hand, structural modularizations, convolution, and attention-based information processing, as well as regularization mechanisms are typical inductive learning biases.

\noindent \textbf{Event segmentation}
describes the process of identifying distinct events from a stream of continuous sensorimotor information. Very generally, an event can be any type of segment that is perceived to have a beginning and an end  \cite{Zacks2001_EventStructure}.
Moreover, an event can be typically characterised by distinct interaction dynamics, including particular spatial-relational, force or motor, and entity-respective properties \cite{Butz2016,Butz:2021} (cf. also \autoref{box:appendix:EST}). 

% \noindent \textbf{Epistemic drive}
% refers to the motivational drive of an agent to gain knowledge about itself and its environment. 

\noindent \textbf{Goal-Directed Behaviour}
refers to behaviour, possibly including the direction of attention and thought itself, towards goals. These goals may be activated by motivations, including extrinsic as well as intrinsic motivations, and related epistemic drives.
Goal-directed behaviour thus naturally influences both background planning and decision-time planning, by selectively reflecting on gathered experiences and actively reasoning and planning to solve current tasks respectively

% \noindent \textbf{Zero-shot, one-shot and few-shot problem-solving and learning}
% In machine learning literature, zero-shot learning usually refers to an architecture that can solve a new problem without any new training data.
% One-shot and few-shot learning requires one or only a few new training examples. 
% We adapt this terminology and use the terms zero-shot and few-shot problem-solving to refer to an agent that can solve a new problem without or with only a few any additional training trials. 

}{E-\ref{rev:editor:form:language}; R2-\ref{rev:r2:realisation_terminology}; R2-\ref{rev:r2:terminology_results}; R2-\ref{rev:r2:semantics:comp_representations}; R2-\ref{rev:r2:terminology}; R2-\ref{rev:r2:terminology2}}
 \end{infobox}

==> v2/hrlFinal.tex <==
\section{Computational realisations}
\label{sec:hrlFinal}

Computational hierarchical reinforcement learning (HRL) mechanisms (cf.~\autoref{fig:hrl}) are less integrated than those of biological agents. 
There are promising novel developments to potentially overcome the existing limitations, \revv{but there are also shortcomings and challenges.}{E-\ref{rev:editor:difficulties:integration}}
We provide an overview of the existing approaches in the supplementary  \autoref{tab:hrl_properties}.
% Herein, we do not explicitly mention reactive policies that map states and goals to actions since these are a general necessary component for solving Markovian decision processes. 
% Herein, we consider a loose definition of ``hierarchical'', and are interested in literature where states and actions are abstracted in some sense, which does not necessarily imply multiple levels of policies (as, e.g., proposed by \citet{Vezhnevets2016_STRAW}). 
% 

% \todo[inline]{TODO: The content of the subsections below is to be elaborated further, based on the literature overview.}

\begin{figure}
    \centering
    %trim={<left> <lower> <right> <upper>}
    %\includegraphics[width=\textwidth,trim={0pt 0pt 0pt 150pt},clip]{pics/HierarchicalArchitecture.pdf}
    \includegraphics[width=\textwidth]{pics/Figure3_smaller.pdf} %TODO use Figure_3_smaller.pdf if there is space
    \caption{A general hierarchical problem-solving architecture with a separate policy $\pi^i$ for each layer of abstraction. 
    Most existing computational HRL approaches focus on two layers, where the high-level action $a^1$ is either a behavioural primitive (an option or sub-policy), or a subgoal.
    Only the low-level actions $a^0$ are motor commands that affect the environment directly. }
    \label{fig:hrl}
\end{figure}

% \input{all_table}

% \subsection{Problem-solving Abilities of Computational Hierarchical Reinforcement Learning Approaches}
% \label{sec:hrl:abilities}

% \subsection{Transfer learning and planning for few-shot problem-solving}
\subsection{Transfer learning and planning for few-shot abilities}
\label{sec:hrl:abilities}
% In comparison to biological agents, the few-shot problem-solving abilities of current reinforcement learning methods are very limited\cite{Butz2017_MindBeing}. 
% So what are the missing computational ingredients that need to be improved further for advanced few-shot problem-solving? 
Our survey of the neurocognitive foundations indicates that two foundational cognitive abilities for few-shot problem-solving are transfer learning and  planning. 

\smallskip
\noindent
\textbf{Transfer learning} denotes the re-use of previously learned skills in new contexts \cite{Perkins1992}.
% , where \emph{near} transfer learning denotes transfer between similar contexts and domains between source and target tasks, while \emph{far} transfer considers stronger dissimilarities \cite{Perkins1992}.
\revv{Transfer learning is natural for hierarchical architectures in the sense that they can potentially re-use general high-level skills and apply them to different low-level use cases, and vice versa. 
For example, a significant fraction of the existing transfer learning approaches build on learning re-usable low-level policies \cite{Eysenbach2019_DiversityFunction,Frans2018_MetaLearningHierarchies,Heess2016_transferModulControl,Jiang2019_HRL_Language_Abstraction,Li2020_SubPolicy,Qureshi2020_CompAgnosticPol,Sharma2020_DADS,Tessler2017_LifelongHRLMinecraft,Vezhnevets2016_STRAW}.
% Transfer learning may also involve the transfer of other data structures, such as predictive forward models\cite{Wu2019_ModelPrimitives}.
}{E-\ref{rev:editor:form:shorten};  R1-\ref{rev:r1:mech_spec_hrl}}
% \citet{Vezhnevets2016_STRAW} build on the automatic discovery of transferable macro-actions (plans) to solve problems in discrete 2D-environments, while  \citet{Jiang2019_HRL_Language_Abstraction} use natural language action representations to perform near transfer learning.
% \citet{Qureshi2020_CompAgnosticPol} build on re-usable low-level policies for goal-conditioned hierarchical reinforcement learning. 
% The policies are transferable between similar tasks, e.g. different locomotion tasks with the same agent.
Research has not only considered transfer learning between different tasks, but also between different robot and agent morphologies\cite{Devin2017_Transfer_RL,Frans2018_MetaLearningHierarchies,Hejna2020_MorphologicalTransfer}. 
% We classify these approaches as \emph{far} transfer because the entire sensorimotor apparatus changes, which places the agent in a far dissimilar context.
% Furthermore, the methods that feature such cross-morphological transfer also perform far transfer learning across different application domains. 
% \revv{
% For example, \citet{Frans2018_MetaLearningHierarchies} transfer navigation skills acquired in a discrete-space environment to a different continuous-space environment.}{R2-\ref{rev:r2:sugg:trans_learn_para}}
% All aforementioned near and far transfer approaches perform skill transfer implicitly, e.g, by re-using pre-trained policies and value functions, but without explicitly representing and learning the analogies between diferent tasks. 
% An exceptional approach that considers the analogies between representations in different tasks explicitly has been presented \citet{Oh2017_Zero-shotTaskGeneralizationDeepRL}. 
% The authors use vector embeddings to represent the representations. 
% The method has been extended in a later paper\cite{Sohn2018_Zero-ShotHRL}, where the high-level layer is implemented as a neural subtask graph solver that reasons over the preconditions, costs and rewards of subtasks to infer the optimal path over subtasks.

% In summary, the transfer-learning capabilities of hierarchical reinforcement learning methods are 
\smallskip
\noindent
\textbf{Planning} \rev{can be categorised into \emph{decision-time planning} and \emph{background planning}, as suggested by \citet{Hamrick2021_MBRL}. 
We refer to decision-time planning as a search over sequences of actions to decide which action to perform next to achieve a specific goal.
The search is realised by simulating the actions with an internal predictive model of the domain dynamics.  
Decision-time planning enables zero-shot problem-solving because the agent only executes the planned actions if an internal prediction model verifies that the actions are successful.
Background planning usually refers to model-based reinforcement learning as introduced by \citet{Sutton1990_Dyna}. It is used to train a policy by simulating actions with a forward model.
This can improve the sampling efficiency, but not to the extent that it enables few-shot problem-solving.}{R2-\ref{rev:r2:terminology}; R2-\ref{rev:r2:papers:hamrick}}

Hierarchical decision-time planning is a well-known paradigm in classical artificial intelligence\cite{Nau2003_SHOP2}, but approaches that integrate it with hierarchical reinforcement learning are rare. 
Some approaches integrate action planning with reinforcement learning by using an action planner for high-level decision-making and a reinforcement learner for low-level motor control\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS}. 
% For example, \citet{Eppe2019_planning_rl} focus on integrating the discrete-space high-level representations for planning with continuous-space low-level representations for motor control. \citet{Ma2020_MultiAgentHRL} focus on multi-agent systems.
These approaches underpin that decision-time planning is especially useful for high-level inference in discrete state-action spaces. 
% However, we are aware of only one recent approach\cite{Botvinick2009_HierarchicalCognitionRL} that exploits predictive models for planning on both the high-level and low-level layer.
% % \footnote{Some approaches use the word ``planning'' to refer to a method that is different from the kind of planning that we consider here.} 
% The authors refer to this architecture as \emph{saltatory} model-based reinforcement learning with planning and they empirically demonstrate significant performance gains with their approach. 
% Additional still unexplored potential synergies become apparent when considering that action planning usually suffers from complexity issues due to the combinatorial explosion of possible state transitions. 
% A reinforcement learning policy can serve as a heuristics to propose candidate plans for a planner, so that the planner does not need to traverse the full search space.


% They either realize one-shot problem-solving by performing a very close transfer between similar problems within the same domain\cite{}, or they only support overly simplistic discrete-space environments\cite{}. 

\subsection{Mechanisms behind transfer learning and planning}
\label{sec:hrl:mechanisms}
Our summary of the cognitive principles behind transfer learning and planning reveals three important mechanisms that are critical for the learning and problem-solving abilities of biological agents, namely compositional sensorimotor abstraction, intrinsic motivation, and mental simulation.

\smallskip
\noindent
\textbf{Compositional sensorimotor abstraction and grounding.}
Hierarchical reinforcement learning (HRL) has a temporal and a representational dimension, and one can distinguish between action and state abstraction. 
The temporal abstraction of actions breaks down complex problems into a hierarchy of simpler problems. 
% The temporal dimension is an innate property of HRL because by definition it beaks down each high-level action or behaviour into low-level actions or behaviours. 
% The representational dimension is less clearly defined. 
% Another dimension of abstraction is representational abstraction. 
% However, temporal abstraction is not the only dimension of abstraction that helps to simplify problems. 
% Here, we are interested in a less investigated form of abstractions, namely representational abstraction. 
% Hierarchical reinforcement learning approaches also involve representational action abstraction. 
% One can distinguish the existing approaches into two different types of representational action abstraction.
The probably most influential method for representational action abstraction builds on behaviour primitives
% \cite{Bacon2017_OptionCritic,Dietterich2000_StateAbstraction_MAXQ,Frans2018_MetaLearningHierarchies,Kulkarni2016_HDQN,Li2020_SubPolicy,Li2017_efficient_learning,Ma2020_MultiAgentHRL,Machado2017_PVF_Laplace_OptionDiscovery,Qiao_2020_HRL-Driving,Shankar2020_MotorPrimitives,Sharma2020_DADS,Tessler2017_LifelongHRLMinecraft,Vezhnevets2020_OPRE}%
\cite{Bacon2017_OptionCritic,Dietterich2000_StateAbstraction_MAXQ,Frans2018_MetaLearningHierarchies,Kulkarni2016_HDQN,Li2020_SubPolicy,Shankar2020_MotorPrimitives,Sharma2020_DADS,Vezhnevets2020_OPRE}
, including options\cite{Sutton1999_options}, sub-policies, or atomic high-level skills.
Such behaviour primitives are represented in an abstract representational space, e.g. in a discrete finite space of action labels or indices (see \autoref{fig:options_behaviour_primitives}, a.). 
Another more recent type of high-level action representations are subgoals in the low-level state-space \cite{Eppe2019_planning_rl,Ghazanfari2020_AssociationRules,Hejna2020_MorphologicalTransfer,Levy2019_Hierarchical,Nachum2018_HIRO,Rafati2019_model-free_rep_learning,Roeder2020_CHAC,Zhang2020_AdjancentSubgoals} (see \autoref{fig:options_behaviour_primitives}, b.).
Subgoals are abstract actions defined in the low-level state space, and the agent achieves the final goal by following a sequence of subgoals.
% There exist also methods that encode high-level actions as continuous vector representations. 
% For example, \citet{Han2020_hierarchicalSelfOrga} use a multi-timescale RNN, where the high-level actions are encoded by the connections between the RNN layers and others use latent vector representations to encode high-level behaviour\cite{Isele2016_FeatureZeroShotTransfer,Shankar2020_MotorPrimitives}. 
% However, some approaches add an abstract context vector to the subgoal specification\cite{Rasmussen2017_NeuralHRL}. 
\begin{figure}
    \centering
    %trim={<left> <lower> <right> <upper>}
    \includegraphics[width=.99\linewidth,trim={20pt 0pt 100pt 40pt},clip]{pics/OptionsSubgoals.pdf}
    {\sf \footnotesize ~~~~~~~ (a.)    behaviour primitives  ~~~~~~~~~~~~ (b.) Subgoals ~~~~~~~~~~~~ }
    \caption{Action abstraction through behaviour primitives (a) vs subgoals (b). With behaviour primitives, the agent determines the path to the final goal by selecting a sequence of high-level actions, but without specifying explicitly to which intermediate state each action leads. With subgoals, the agent determines the intermediate states as subgoals that lead to the final goal, but without specifying the actions to achieve the subgoals.}
    \label{fig:options_behaviour_primitives}
\end{figure}
%

% Overall, there exists a strong implicit focus on action abstraction in HRL.
% , but state abstraction is underrepresented.
Our supplementary \autoref{tab:hrl_properties} shows that  there is considerably less contemporary research on state abstraction than on action abstraction. 
% \citet{Han2020_hierarchicalSelfOrga} perform hierarchical action abstraction with multi-timescale recurrent neural networks.
% However, significant cognitive evidence demonstrates that representational state abstraction is at least as important to realize efficient problem-solving\cite{Butz2017_MindBeing,Lesort2018_state-rep-learning-control}. 
% 
% State abstractions in biological systems range from the mere preprocessing of sensor data, e.g. in the primary visual cortex, to the problem-driven grounding of signals in abstract compositional concept representations \cite{Butz2017_MindBeing,Lesort2018_state-rep-learning-control}. Counterparts for some of these methods can also be found in computational architectures. 
\revv{
Many current reinforcement learning approaches based on visual input use convolutional neural networks to perform a rather generic abstraction of visual sensor data\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}. 
\revv{A problem is that this generic abstraction does not appreciate that \emph{different levels of inference require different levels of abstraction}: For example,  for a transport task, the exact shape and weight of an object is only relevant for the low-level motor control. A high-level planning layer only requires abstract facts, such as whether the object is graspable or transportable.}{R3-\ref{rev:rev3:appreciate_difficulties}} 
Therefore, the representational state abstraction should fit the level of inference it is used for. We refer to such abstractions as \textbf{inference-fitted abstractions}. 
%
% Therefore, we consider only those approaches as representational abstraction methods that involve layer-wise abstraction. 
Inference-fitted abstraction has been tackled in existing HRL approaches, but many of them rely on manually defined abstraction functions\cite{Eppe2019_planning_rl,Kulkarni2016_HDQN,Ma2020_MultiAgentHRL,Toussaint2018}.
There exist only a few exceptions where state abstractions are derived automatically in hierarchical reinforcement learning%
% \cite{Ghosh2019_ActionableRep,Vezhnevets2017_Feudal,Vezhnevets2020_OPRE}
, e.g. through  clustering\cite{Akrour2018_RL_StateAbstraction,Ghazanfari2020_AssociationRules}, with feature representations\cite{Schaul2013_Better_Generalization_with_Forecasts}, or by factorisation \cite{Vezhnevets2020_OPRE}.}{R2-\ref{rev:r2:semantics:comp_representations}}
% Interestingly, non-hierarchical model-based reinforcement learning offers promising alternative prediction-based methods for state abstraction \cite{Hafner2020_Dreamer,Pathak2019_ICML_SelfSuperExploreDisa}, which show parallels to cognitive prediction-based abstraction theories. 
% However, these have not yet been applied in a hierarchical architecture. 

Cognitive science also suggests that \emph{compositionality} is an important property of abstract representations. 
For instance, a symbolic compositional action representation \concept{grasp(glass)} allows for modulating the action \emph{grasp} with the object \emph{glass}.
% In terms of reinforcement learning, compositionality implies that the meaning of a compositional action representation is determined by multiple constituent expressions and a set of rules to combine them. 
% For example, consider an action representation \concept{grasp(glass)}. 
% The expression consists of several sub-expression and symbols, i.e., an action type symbol (``\concept{grasp}'') a semantic patient symbol (``\concept{glass}''), and delimiter symbols (``('',``)''). There exist syntactic rules that determine that the semantic patient of the action is described by the expression within the delimiters and the action type is determined by the expression before the opening delimiter. Hence, the expression \concept{grasp(glass)} is \emph{syntactically compositional}. 
% This syntactic compositionality has the advantage that less atomic symbols are necessary to represent all possible combinations of action types and objects than the number of symbols that would be required if each composed action would be represented by one non-compositional atomic expression like \concept{``graspGlass''}). 
% For example, given $n_a=4$ action types \concept{``grasp'', ``push'', ``move'', ``release''}) and $n_o=4$ object types \concept{``glass'', ``cup'', ``tea pot'', ``spoon''}, the total number of symbols for compositional representations (e.g. \concept{grasp(glass)}) is $n_a + n_o = 8$, whereas the total number of symbols for non-compositional representations (e.g. \concept{graspGlass} is an atomic symbol) is $n_o \cdot n_a = 16$. 
% Similar advantages hold for compositional state representations (e.g. \concept{leftOf(cup,tea pot)}). 
Compositionality is also applicable to distributed numerical expressions, such as vector representations. For example, a vector $v_1$ is a compositional representation if it is composed of other vectors, e.g., $v_2$ and $v_3$, and if there is a vector operation $\circ$ that implements interpretation rules, e.g., $v_1 = v_2 \circ v_3$. 

There is significant cognitive evidence that compositionality improves transfer learning\cite{Colas2020_LanguageGroundingRL}. 
This evidence is computationally plausible when considering that transfer learning relies on exploiting analogies between problems, as described in the supplementary \autoref{box:appendix:compositionality-example}
% This lower number of possible analogy mappings of compositional representations implies better transferability. This has not yet been investigated empirically in reinforcement learning, but 
Other cognitively inspired computational methods, such as concept blending\cite{Eppe2018_AIJ_Blending}, provide further evidence that a lower number of possible analogy mappings improves transferability.
% , where two or more compositional concept representations are transferred into a new representation. 
% \begin{figure}
%     \centering
%     \includegraphics{pics/compTransfer.pdf}
%     \caption{Compositional representations improve transfer learning}
%     \label{fig:compTransfer}
% \end{figure}
Furthermore, the work by \citet{Jiang2019_HRL_Language_Abstraction} provides empirical evidence that compositional representations improve learning transfer. The authors use natural language as an inherently compositional representation to describe high-level actions in hierarchical reinforcement learning, and show that this natural language representation improves transfer learning performance compared to non-compositional representations.
%
% Few other researchers use compositional representations in hierarchical reinforcement learning. \citet{Saxe2017_HRL_Multitask_LMDP} compose high-level actions from concurrent linearly solvable Markov decision processes (LMDPs) to guarantee optimal compositionality. Their method successfully executes compositional policies that it has never executed before, effectively performing zero-shot problem-solving.
% Zero-shot problem-solving has also been demonstrated in other related articles that feature compositional action representations\cite{Isele2016_FeatureZeroShotTransfer,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}, but these works do not draw an explicit link between compositionality and zero-shot problem-solving.
% A few symbolic compositional state representations exist in hierarchical decision-making methods, but these rely on manually defined abstraction functions\cite{Eppe2019_planning_rl,Kulkarni2016_HDQN,Lyu2019_SDRL,Toussaint2018} or they are very general and feature compositionality only as an optional property\cite{Rasmussen2017_NeuralHRL}.
%

% There also exist hierarchical reinforcement learning approaches where sub-symbolic compositional representations are learned\cite{Devin2017_Transfer_RL,Qureshi2020_CompAgnosticPol,Schaul2013_Better_Generalization_with_Forecasts,Vezhnevets2020_OPRE}. 
% The compositionality of these representations is rather implicit and, with one exception \cite{Qureshi2020_CompAgnosticPol}, has not been investigated in the context of transfer learning. The exceptional approach by \citet{Qureshi2020_CompAgnosticPol} considers composable low-level policies and shows that compositionality significantly improves transfer between similar environments. 


\smallskip
\noindent
\textbf{Intrinsic motivation}
is a useful method to stabilise reinforcement learning by supplementing sparse extrinsic rewards with additional  domain-independent intrinsic rewards. 
% Intrinsic motivation is also commonly used to incentivize exploration.  
% Reinforcement learning typically models intrinsic motivation through intrinsic rewards. 
The most common method of HRL with intrinsic motivation is to provide intrinsic rewards when subgoals or subtasks are achieved%
% \cite{Blaes2019_CWYC, Cabi2017_intentionalunintentional,Eppe2019_planning_rl,Haarnoja2018_LatentSpacePoliciesHRL,Jaderberg2017_unreal,Kulkarni2016_HDQN,Lyu2019_SDRL,Oh2017_Zero-shotTaskGeneralizationDeepRL,Qureshi2020_CompAgnosticPol,Rasmussen2017_NeuralHRL,Riedmiller2018_SAC-X,Roeder2020_CHAC,Saxe2017_HRL_Multitask_LMDP,Sohn2018_Zero-ShotHRL,Yamamoto2018_RL_Planning,Yang2018_PEORL}.
\cite{Blaes2019_CWYC,Eppe2019_planning_rl,Haarnoja2018_LatentSpacePoliciesHRL,Kulkarni2016_HDQN,Lyu2019_SDRL,Oh2017_Zero-shotTaskGeneralizationDeepRL,Qureshi2020_CompAgnosticPol,Rasmussen2017_NeuralHRL,Riedmiller2018_SAC-X,Yang2018_PEORL}.

% }$^,$~ \cite{
Other approaches provide intrinsic motivation to identify a collection of behavioural primitives with a high diversity\cite{Blaes2019_CWYC, Eysenbach2019_DiversityFunction,Machado2017_PVF_Laplace_OptionDiscovery} and predictability\cite{Sharma2020_DADS}. 
This includes also the identification of primitives suitable for re-composing high-level tasks\cite{Shankar2020_MotorPrimitives}.

Another prominent intrinsic reward model that is commonly used in non-hierarchical reinforcement learning is based on surprise and curiosity\cite{Oudeyer2007,Pathak2017_forward_model_intrinsic,Schillaci2020_IntrinsicMotivation,Schmidhuber2010}. 
In these approaches, surprise is usually modelled as a function of the prediction error of a forward model, and curiosity is realised by providing intrinsic rewards if the agent is surprised.
However, only \citet{Blaes2019_CWYC}, \citet{Colas2019_CURIOUS}, and \citet{Roeder2020_CHAC} use surprise in a hierarchical setting, showing that hierarchical curiosity leads to a significant improvement of the learning performance.
\revv{Hierarchical curiosity provides potential synergies because a curious high-level layer automatically acts as a curriculum generator for a low-level layer. For example, it can generate ``Goldilocks'' subgoals that are neither too hard nor too easy to achieve for the low-level layer. 
The difficulty is to identify these Goldilocks conditions and to find an appropriate balance between explorative and exploitative subgoals.
}{R1-\ref{rev:r1:mech_spec_hrl}}
%Both approaches train a high-level layer to determine explorative subgoals in hierarchical reinforcement learning. 
% These approaches train a high-level layer to determine explorative subgoals in hierarchical reinforcement learning.
% In addition, \citet{Roeder2020_CHAC} also use surprise to supplement sparse reward for the low-level layer, and they show that hierarchical curiosity leads to a significant improvement of the learning performance.
% An alternative method to model curiosity is to perform hypothesis-testing for option discovery\cite{Chuck2020_HyPe}.

\smallskip
\noindent
\textbf{Mental simulation} enables an agent to anticipate the effects of its own and other actions. Therefore, it is a core mechanism to equip an intelligent agent with the ability to plan ahead. Computational approaches for mental simulation involve model-based reinforcement learning\cite{Sutton1990_Dyna}, action planning\cite{Nau2003_SHOP2}, or a combination of both \cite{Eppe2019_planning_rl,Hafez2020_dual-system}. 
However, even though there is cognitive evidence that mental simulation happens on multiple representational layers\cite{Butz2017_MindBeing,Frankland2020_SearchLoT}, there is a lack of approaches that use hierarchical mental simulation. 
Only a few hierarchical approaches that integrate planning with reinforcement learning build on mental simulation\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS,Yamamoto2018_RL_Planning,Yang2018_PEORL}, though the mental simulation mechanisms of these models are only implemented on the high-level planning layer. 
An exception is the work by \citet{Wu2019_ModelPrimitives}, who use mental simulation on the low-level layer to determine the sub-policies to be executed. 
Another exception is presented by \citet{Li2017_efficient_learning}, who perform mental simulation for planning on multiple task layers. 
\revv{However, we are not aware of any approach that performs hierarchical background planning, i.e., that trains a hierarchical policy by mentally simulating the action execution on multiple levels.
One possible reason for this lack is that high-level background planning requires stable low-level representations, and it is difficult to model a respective stability criterion.}{R1-\ref{rev:r1:mech_spec_hrl}}

% There exist several non-hierarchical model-based reinforcement learning methods\cite{Ha2018_WorldModels,Hafner2020_Dreamer,Sutton1990_Dyna} that perform background planning, i.e., the policy is trained by mentally simulating action execution instead of executing the actions in the real world.

% (e.g.\cite{Sutton1990_Dyna}).

\subsection{Prerequisites for sensorimotor abstraction, intrinsic motivation, and mental simulation}
Reinforcement learning builds on policies or inverse models that predict the actions to be executed in the current state to maximise reward or to achieve a goal state.
% Some approaches learn the policy directly, and others learn a value function that determines the policy. 
In contrast, a forward model predicts a future world state based on the current state and a course of actions. 
% Both kinds of models are critical prerequisites for compositional abstraction, intrinsic motivation, and mental simulation.
Our review shows that the vast majority of hierarchical reinforcement learning methods use inverse models for both the high-level and low-level layers. 
Some approaches exist that use an inverse model only for the low-level layer\cite{Eppe2019_planning_rl,Lyu2019_SDRL,Ma2020_MultiAgentHRL,Sharma2020_DADS,Yamamoto2018_RL_Planning,Yang2018_PEORL} and use decision-time planning to perform high-level decision-making.
Our review also implies that a forward model is required for several additional mechanisms that are necessary or at least highly beneficial for transfer learning, planning, and few-shot problem-solving. 
Some non-hierarchical approaches use a forward model to perform sensorimotor abstraction\cite{Hafner2020_Dreamer,Pathak2017_forward_model_intrinsic}. They achieve this with a self-supervised process, where forward predictions are learned in a latent abstract space. 
However, we are not aware of any hierarchical method that exploits this mechanism. 

A forward model is also useful to model curiosity as an intrinsic motivation mechanism, for example, by rewarding an agent for being surprised, where surprise is a function of the prediction error \cite{Friston2011}. 
% To perform these predictions, a forward model is required.
Curiosity has been demonstrated to alleviate the sparse rewards problem in reinforcement learning\cite{Pathak2017_forward_model_intrinsic,Roeder2020_CHAC}, but with few exceptions\cite{Colas2019_CURIOUS,Roeder2020_CHAC}, there is a lack of approaches that use a hierarchical forward model for generating hierarchical curiosity. 
% The third and most obvious application of a forward model is mental simulation. To simulate the effects of actions, be it for planning or motor imagery, agents must learn a forward model. 

% However, a well-known problem for mental simulation is the model bias\cite{Lesort2020_ContLearnRobo}. 
% A forward model that emulates the dynamics of a real environment is always biased and each predicted state-transition inheres an error.
% Predicting the outcome of a  sequence of actions involves the recursive computation of several state transitions. The error propagates further with each recursion, leading to imprecise mental simulation.
% To address this problem, recent non-hierarchical model-based reinforcement learning methods use Gaussian models that predict also the uncertainty of their predictions\cite{Kupcsik2017}. 
% However, the approach has not yet been applied in a hierarchical reinforcement learning architecture. 





==> v2/intro.tex <==
%\begin{wrapfigure}[12]{r}[34pt]{10cm}
% \section{Introduction}
% \label{sec:intro}
% Some dummy text
% \begin{figure*}
% \centering
%     %trim={<left> <lower> <right> <upper>}
%     % \includegraphics[width=.19\columnwidth,trim={196pt 81pt 167pt 38pt},clip]{pics/1-crow-pickstick.png}
%     % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(1)\end{minipage} 
%     % \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/2-crow-usestick.png}
%     % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(2)\end{minipage} 
%     % \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/3-crow-getstone.png}
%     % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(3)\end{minipage} 
%     % \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/4-crow-usestone.png}
%     % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(4)\end{minipage} 
%     % \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/5-crow-havefood.png}
%     % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(5)\end{minipage}
%     % \includegraphics[width=.19\columnwidth,trim={196pt 81pt 167pt 38pt},clip]{pics/1-crow-pickstick PS1.png}
%     \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-1-clean.pdf}
%     \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{a}\end{minipage} 
%     \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-2-clean.pdf}
%     \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{b}\end{minipage} 
%     \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-3-clean.pdf}
%     \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{c}\end{minipage} 
%     \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-4-clean.pdf}
%     \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{d}\end{minipage} 
%     \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-5-clean.pdf}
%     \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{e}\end{minipage} 
%     \vspace{-10pt}
% \caption{A New Caledonian crow solves a food-access problem:\cite{Gruber2019_CrowMentalRep} \textbf{a,} First, the crow picks a stick. \textbf{b-c,} Then it uses the stick to pull a stone out of a tube. \textbf{d-e,} Finally, it uses the stone to activate a mechanism that releases food. The crow has never solved this problem setup  before. Nevertheless, after a brief inspection phase, it is able to solve the problem, suggesting that the crow develops memorized abstract mental representations to plan ahead. 
%     \rev{This use case of zero-shot problem-solving is a prime example for hierarchical decision-making, based on a composition of several cognitive mechanisms.
%     % These mechanisms involve mental simulation, transfer learning, and representational abstraction.
%     For example, the authors of the study\cite{Gruber2019_CrowMentalRep} reason that the crow must simulate its behaviour to \emph{plan ahead}, because it can only see one side of the cubic setup at a time. 
%     Hence, following the authors' rationale, it must \emph{mentally simulate} the future steps. 
%     There is clearly also \emph{transfer learning} involved: The crow has previously solved individual sub-stages of the problem, and the solutions to the sub-problem are now transferred to the new problem. 
%     The planning and the transfer learning would only be expected if it builds on \emph{abstract compositional mental representations} that involve, for example, the abstract functions and affordances of the tools it uses. 
%     % The crow is motivated to solve the problem because food is involved. However, it 
%     The crow has learned the affordances of the tools previously, when it learned to solve the individual sub-stages.
%     This however, required \emph{intrinsic motivation} to experiment with the tools. 
%     A related study\cite{Kenward2011_tools_crows} concludes that ``heritable action patterns do not provide a complete explanation'' for the problem-solving abilities or crows, suggesting that ``crows are more inclined to object-combination play''. This falls into our category of intrinsic motivation mechanisms.}{R1-\ref{rev:r1:example}}
%     }.
% \label{fig:dummy}
% \end{figure*}
% Link to \autoref{fig:crow_probsolving} and \autoref{fig:cog_prereq} and \autoref{fig:dummy}.

\begin{figure*}[ht]
    \centering
    %trim={<left> <lower> <right> <upper>}
    % \includegraphics[width=.19\columnwidth,trim={196pt 81pt 167pt 38pt},clip]{pics/1-crow-pickstick.png}
    % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(1)\end{minipage} 
    % \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/2-crow-usestick.png}
    % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(2)\end{minipage} 
    % \includegraphics[width=.19\columnwidth,trim={306pt 33pt 0pt 38pt},clip]{pics/3-crow-getstone.png}
    % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(3)\end{minipage} 
    % \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/4-crow-usestone.png}
    % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(4)\end{minipage} 
    % \includegraphics[width=.19\columnwidth,trim={181pt 33pt 125pt 38pt},clip]{pics/5-crow-havefood.png}
    % \hspace{-0.6cm}\begin{minipage}[b][0.4cm][t]{0.5cm}(5)\end{minipage}
    % \includegraphics[width=.19\columnwidth,trim={196pt 81pt 167pt 38pt},clip]{pics/1-crow-pickstick PS1.png}
    \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-1-clean.pdf}
    \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{a}\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-2-clean.pdf}
    \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{b}\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-3-clean.pdf}
    \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{c}\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-4-clean.pdf}
    \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{d}\end{minipage} 
    \includegraphics[width=.19\columnwidth,trim={10.93cm 5.52cm 10.93cm 3.52cm},clip]{pics/crow-5-clean.pdf}
    \hspace{-0.4cm}\begin{minipage}[b][0.3cm][t]{0.3cm}\textbf{e}\end{minipage} 
    \vspace{-10pt}
    % \label{fig:crow_probsolving}
    % \includegraphics[width=.18\textwidth,trim={0pt 0pt 0pt 105pt},clip]{pics/crow4.jpg}
    \rev{}{R1-\ref{rev:r1:example}}
    \caption{A New Caledonian crow solves a food-access problem (images used with permission by R. Gruber and co-authors):\cite{Gruber2019_CrowMentalRep} \textbf{a,} First, the crow picks a stick. \textbf{b-c,} Then it uses the stick to pull a stone out of a tube. \textbf{d-e,} Finally, it uses the stone to activate a mechanism that releases food. 
    Although the crow has never solved this problem setup before, it is able to solve it instantly after a brief inspection phase.
    % , suggesting that the crow develops memorized abstract mental representations to plan ahead. 
    % \rev{
    {\color{revcolor}This use case of zero-shot problem-solving is a prime example for \emph{hierarchical, goal-directed planning} that involves mental simulations and relies on a composition of task-suitable \emph{state- and action-abstractions}.
    % These mechanisms involve mental simulation, transfer learning, and representational abstraction.
    The authors reason that the crow \emph{plans ahead} because it can only see one side of the cubic setup at a time.\cite{Gruber2019_CrowMentalRep} 
    Hence, the crow must \emph{mentally simulate} the future steps. 
    There is clearly also \emph{transfer learning} involved: previously learned solutions to similar sub-problems are transferred and combined to solve the new, more complex problem. 
    Successful planning and transfer learning can be expected to only occur once \emph{abstract compositional mental representations} have developed, which, for example, may encode the abstract manipulation options afforded by the available tools. 
    % The crow is motivated to solve the problem because food is involved. However, it 
    % The crow has learned the affordances of the tools previously, when it learned to solve the individual sub-stages.
    To learn tool affordances and compositional representations, however, the crow relies on its \emph{intrinsic motivation} to acquire knowledge by playing and experimenting with the tools. 
    % A related study\cite{Kenward2011_tools_crows} concludes that ``heritable action patterns do not provide a complete explanation'' for the problem-solving abilities or crows, suggesting that ``crows are more inclined to object-combination play''.
    }
    }.
    % }{R1-\ref{rev:r1:example}}
    \label{fig:crow_probsolving}
\end{figure*}
% \end{wrapfigure}

% \section{Introduction}
% \label{sec:intro}

% \citet{Eppe2015_IJCAI_Blending}
% \citeauthor{Ha2018_WorldModels}

Humans and several other \revv{intelligent animal species}{R3-\ref{rev:r2:sugg:int_animal}} have the ability to break down complex problems into simpler, previously learned sub-problems. This hierarchical approach allows them to solve previously unseen problems in a zero-shot manner, i.e., without any trial and error. 
% What are the mechanisms that are responsible for the capability to unseen solve problems by insight and causal inference in a one-shot manner, without any trial and error?
% Humans and certain intelligent animal species are able to perform \emph{one-shot problem-solving}. They can solve a previously unseen causally non-trivial problem by breaking it down into a hierarchy of previously learned sub-problems. 
For example, \autoref{fig:crow_probsolving} depicts how a crow solves a non-trivial food-access puzzle that consists of three causal steps: It first picks a stick, then uses the stick to access a stone, and then uses the stone to activate a mechanism that releases food \cite{Gruber2019_CrowMentalRep}. 
% Other experiments with crows demonstrate their transfer-learning performance \cite{Taylor2014_CorvidCognition}. 
There exist numerous analogous experiments that attest similar capabilities to primates, octopuses, and, of course,  humans \cite{Butz2017_MindBeing,Perkins1992}.
To develop such problem-solving skills, human and animal cognition research strongly suggests that hierarchical learning and problem-solving is key \cite{Botvinick2009_HierarchicalCognitionRL,Butz2017_MindBeing,Tomov2020}. 
% Yet, little is known about the cognitive mechanisms that are responsible for these capabilities, and even less is known about how these mechanisms can be modelled and verified computationally. 
% It is remarkable that the advanced problem-solving and tool-use abilities of these biological agents have evolved separately and independently from each other multiple times in different species.
This raises the question of how we can equip intelligent artificial agents and robots with similar hierarchical learning and zero-shot problem-solving abilities.

% A common method to illuminate the cognitive processes of biological agents is to model them computationally and to evaluate them with virtual or robotic agents. 
% The currently existing computational systems provide less sophisticated problem-solving mechanisms than intelligent biological agents, but 
% There exist several cognitively inspired computational methods that have the potential to be developed further towards a problem-solving performance that is closer to the abilities of humans or animals.
We address this question from the perspective of reinforcement learning (RL) \cite{Arulkumaran2017_DeepRL,Li2018_DeepRL_Overview,Sutton:2018}. 
Several studies suggest that RL is biologically and cognitively plausible \cite{Neftci2019_RL_BioArtificial_NatureMI,Sutton:2018}. Many existing RL-based methods are aiming at zero-shot problem-solving and transfer learning, but this is currently only possible for minor variations of the same or a similar task \cite{Eppe2019_planning_rl} or in simple synthetic domains, such as 2D grid worlds \cite{Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL}.
A continuous-space problem-solving behaviour that is comparable with the crow's behaviour of \autoref{fig:crow_probsolving} has not yet been accomplished with any artificial system, based on RL or other approaches.
We suggest that the focus on hierarchical learning and problem-solving is largely missing, seeing 
% Therefore, we consider literature in human and animal cognition to identify and discuss the shortcomings and challenges that need to be overcome to further improve RL-based computational systems.
% So what are the critical cognitive prerequisites for learning-based problem-solving and skill transfer? What are the most critical shortcomings of existing RL architectures? And how can we overcome the limitations of existing RL methods?
% , suggesting that decision-making can be modelled with
that research in hierarchical reinforcement learning (HRL) is underrepresented, as suggested by our meta review in \autoref{box:appendix:meta_RL-survey} of the supplementary material.
% We hypothesise that one reason why current machine learning systems fail is that they struggle to leverage the power of learning hierarchical abstractions. 



% This brief meta-review addresses the shortage of hierarchical reinforcement learning by illuminating the finer-grained mechanistic discrepancies between the sophisticated problem-solving behaviour of intelligent biological agents and the limited capabilities of existing computational reinforcement learning agents. 
% We structure this review as follows:

% In this article, we address this shortage and plot ways forward.
% Martin: ich finde diese "roadmap" info wurde im Abstract schon hinreichend gesagt - können wir uns sparen.
%The first part of this article includes a review of human and animal cognition, related to learning, decision-making, and goal-directed behaviour. From this survey, we extract core mechanisms and principles that are suitable and sufficiently understood to be modeled within a computational framework. 
%%% We show that many of these mechanisms are based on hierarchical mental abstraction and sensorimotor prediction using a forward model. 
%
%The second part of this article reviews the state of the art in computational hierarchical reinforcement learning, and relates the contemporary computational methods to the results of our cognitive survey. 
% This review is comprehensive with respect to HRL literature published between January 2017 and May 2020, and we also consider the most important previous work. 

\revv{In this article, we address this gap by both evaluating neurocognitive foundations of hierarchical decision-making and identifying important mechanisms that enable advanced problem-solving skills. 
% odels, suggesting that there should be more focus on predictive forward models in hierarchical RL.
% Furthermore, we exhibit that existing hierarchical RL methods hardly address state abstraction and compositional representations. 
We then review computational hierarchical RL methods and show that the biological mechanisms have mostly been implemented already---but only in isolation and not in an integrative manner. 
% However, we also show that there exist exceptions where isolated relevant cognitive mechanisms including forward models and compositional abstraction have already been implemented, but not in combination with other important mechanisms.
Thus, the AI community already provides many tools for building more intelligent agents, but it is struggling to integrate them properly.
We suggest steps towards combining key methods and mechanisms to overcome the integration challenge for the development of a unifying cognitive architecture.}{E-\ref{rev:editor:review_perspective}; R3-\ref{rev:r3:clarify_contrib}}
\revv{To be as precise as possible, we define the semantics of our terminology in a glossary in the supplementary \autoref{box:appendix:glossary}.}{E-\ref{rev:editor:integrating_difficulties:terms}}
% \input{glossary_box}

%
% In \autoref{sec:conclusion} we conclude and address these limitations by sketching several model-based extensions to existing hierarchical reinforcement learning approaches. 
% Based on the results of the previous review sections, we expect these extensions to improve the sampling-efficiency, the generalization performance, as well as the transfer learning and zero-shot problem-solving capabilities of existing methods. 


% There exist several different subdisciplines within Artificial Intelligence that address hierarchical one-shot problem-solving. As examples consider Task and Motion Planning (e.g. \cite{Toussaint2018}) or hierarchical planning (e.g. \cite{Nau2003_SHOP2}). 
% However, a keyword search in relevant conferences such as IJCAI, AAAI, ICLR reveals that most progress in the past years has been made in the 
% 

% \begin{wrapfigure}{r}{0.5\textwidth} 

% \end{wrapfigure}





==> v2/notes_snippets_manfred.tex <==

% This implies that different intelligent species would conceptualize the world in different ways, ultimately leading to different languages and different self-representations. 
% The theory states that there exist so-called basic concepts that are directly linked to the body. 
% As an example for a basic concept, consider the concept \concept{front}, which is determined by the direction in which we usually move and where most sensory organs are directed to. 
% Other more abstract concepts are hierarchically grounded in basic concepts. 
% For example, consider abstract mathematical concepts, where the front determines the geometric angle of $0^{\circ}$.

\citet{Shapiro2019_EmbodiedCognition} takes a weaker perspective, stating that also agents with different bodies can have shared mental concepts. The grounding of the concepts, however, may be different. He states that even an imaginative spherical being that is capable of omnidirectional movement and sensing in a gravitation-free environment can have a concept for \concept{front} if other objects or agents in its environment have a distinctive side that has certain front-typical features, such as eyes. However, for the spherical being, the \concept{front} concept is not a basic one because it is not directly linked to its body schema. 

Hence, the body schema has a strong influence on higher cognitive functions because it directly influences how we think. 
This becomes evident in natural language, where metaphorical expression involve basic body-related concepts \cite{Eppe2016_GCAI_SemanticParsing,Trott2016}. 
As an example, consider the metaphor \concept{up} \emph{is} \concept{more}. An agent that lives in a gravitation-free environment would not be able to understand a sentence like ``The stock market goes up''.


As an additional example of how body schemas influence our high-level cognitive operations consider recent work on \emph{concept blending} \cite{Eppe2018_AIJ_Blending,Confalonieri2016b,Confalonieri2015}. One pillar of human creativity is the capability of inventing new concepts by means of a serendipitous combinations of known concepts \cite{Fauconnier2002}. This concept blending process strongly depends on body-driven conceptualizations of the world. We conclude that, therefore, creative thought is also a result of the active self. 

What remains open, though, is how we can model grounding of sensorimotor concepts computationally. Several approaches,  including the Theory of Event-Coding \cite{Hommel2015_TEC}, and Event Segmentation Theory \cite{Zacks2007EventPerspective,Gumbsch2019AutonomousPrimitives}, exist. However it is subject to future work to fully integrate these approaches within a unifying computational theory of high-level cognition. Research on the minimal active self fosters the development of such a unifying theory because it allows one to investigate how basic body-related concepts emerge from sensorimotor interaction. 


\subsection{Representational state abstraction}
Cognitive scientists often model abstract mental concepts, such as \emph{path} of \emph{container} in terms of role-filler-based embodied semantic representations, such as semantic frames \cite{Barsalou1992} or image schemas \cite{Lakoff1988,Feldman2009_neural_ECG}. 
For example, a \concept{path} schema has a role \concept{trajector} which is typically filled by an object or agent that moves along the path, and it has roles for \concept{start} and \concept{end}. In our previous work on human-robot dialog, we build on image schemas to perform semantic parsing \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, and show how embodied action-related representations facilitate semantic compositionality for human-robot interaction. 

Role-filler based representations are compatible with action-related semantic representations used in Artificial Intelligence. For example, in action planning, actions are commonly represented by sets of pre- and postconditions (cf. our previous work on action theory \cite{Eppe2015_JAL,Eppe2015_JAL_ASP}): a \concept{move-object} action has the precondition that the agent that moves the object must hold the object, and it has the postcondition that the object is at the target location. In our previous work \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, we have used semantic action templates that link this pre- and postcondition perspective with the role-filler semantics of a semantic language parsing process. 
For example, the \concept{move-object} action inherits structure from the compositional \concept{path} concept: the object to move fills the \concept{trajector} role of the concept, the current object location fills that \concept{start} role and the target location fills the \concept{end} role. 

% , the current object location fills that \concept{start} role, and the target location the \concept{end} role. 

The Neurocognitive and Psychological theories of event coding \cite{Hommel2015_TEC} and ideomotor theory \cite{Stock2004} are in-line with the AI-based pre- and postcondition perspective on actions, as they consider associations between actions and effects at their core. 
However, these and other related theories do not provide a clear consensus on whether conceptual mental action representations are symbolic \cite{Barsalou1999} or distributed \cite{Hommel2015_TEC}. A unifying proposal of modern theories (e.g.~\cite{Hommel2010}) suggests that conceptual compositional representations are distributed, and that language serves as a symbolification mechanism for the underlaying distributed representations. 
\emph{However, there exists no commonly agreed upon mathematical model of learning compositional action- and state representations that is mechanistically compatible to the neurocognitive perspective of distributed representations that are potentially symbolifiable.} 


Humans abstract their sensorimotor data streams and map them to conceptual embodied representations \citet{Barsalou2008_GroundedCognition}. 
High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
For example, on the lowest motor level, an \concept{open hand} action can be modelled as a sequence of continuous finger movements. The opening of the hand may be a semantic primitive within a high-level \concept{grasp} action that consists of \concept{[open hand, move hand to object, close hand]}. The grasp action itself may be a semantic primitive within another higher-level \concept{transport} behavior that consists of \concept{[grasp, move, release]}. 

This divide and conquer approach is also a prominent method to realize learning-based intelligent problem-solving behavior of robots and virtual agents. 

High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
This effectively reduces the branching factor of a problem-solving search process: for the high-level action selection, an agent only has to consider a small set of discrete high-level action primitives and not the large set of their possible low motor-level instantiations. 
This computational problem-solving perspective on sensorimotor abstraction is in-line with



% This article is targeted at researchers in Artificial Intelligence and related fields. Therefore, we can impossibly cover all findings from the life sciences and human sciences that are related to problem-solving, decision-making and mental representations. But how can we obtain an objective overview about the state of the art on learning-based decision-making and problem-solving in cognitive psychology and cognitive neuroscience? 

% In this section, we address this question by performing a meta review of recent survey articles in cognitive psychology and animal cognition. We select and analyze the most cited review articles on learning-based problem-solving from the last three years, which we identify as follows:

% \begin{enumerate}
%     \item 
% \end{enumerate}

% The analysis reveals that there exist several theories related to representational abstraction and predictive forward models for learning-based problem-solving that are largely agreed upon and described well enough to be formalized within a computational framework. 

==> v2/results2.tex <==
\section{Critical discussion and outlook}
\label{sec:results}
% \revv{
\rev{
%In the following, we summarise the state-of-the-art and the shortcomings of hierarchical reinforcement learning, 
Based on our considerations above and the supplementary \autoref{box:appendix:hrl_review} and \autoref{tab:hrl_properties},
we now proceed with summarising the shortcomings of current hierarchical reinforcement learning approaches. 
The shortcomings are consequences of specific challenges that arise from the integration of the different mechanisms (see \autoref{fig:challenges_shortcomings_solutions}). Therefore, we also provide an outlook with suggestions for techniques and methods to partially overcome these shortcomings. 
%
% We present an overview of the relation between the shortcomings, challenges and suggestions for potential partial solutions in 
% }{E-\ref{rev:editor:review_perspective}}
% We present a summary of these results in \autoref{sec:shortcomings_solutions}. 

\begin{figure*}
    \centering
    %\includegraphics[width=.8\textwidth,trim=2.5cm 4cm 2cm 4cm, clip]{pics/Shortcomings_Challenges_Solutions.pdf}
    \includegraphics[width=\textwidth]{pics/illustrations_outlook4.pdf}
    \caption{Our section \nameref{sec:hrlFinal} identifies several shortcomings of contemporary HRL methods. We suppose that these result from at least four central challenges, and we provide three suggestions for key methods that may help to address the challenges.}
    \label{fig:challenges_shortcomings_solutions}
\end{figure*}

\subsection{Shortcomings and challenges of HRL architectures}
\label{sec:results:challenges}
\revv{
% Our computational realizations section and the supplementary \autoref{tab:hrl_properties} provide a comprehensive overview over state-of-the-art computational hierarchical reinforcement learning approaches.
% % , in alignment with our structuring of cognitive prerequisites and mechanisms for the problem-solving abilities of intelligent biological agents (see \autoref{fig:cog_prereq}). 
We identify the following major challenges for current methods:}{E-\ref{rev:editor:difficulties:integration}; R1-\ref{rev:r1:example}; R3-\ref{rev:rev3:appreciate_difficulties}; R3-\ref{rev:r3:structure_not_impression_first_integration}}

\begin{sloppypar}
\noindent \textbf{Hierarchical mental simulation requires stable hierarchical representations and precise predictions.}
\revv{Most current few-shot problem-solving methods build on transfer learning, but they neither leverage decision-time planning nor background planning to exploit hierarchical mental simulation.}{R2-\ref{rev:r2:terminology_results:tautology}}
While numerous non-hierarchical methods show how mental simulation can improve sample efficiency\cite{Deisenroth2011,Ha2018_WorldModels}, our summary in the supplementary \autoref{tab:hrl_properties} shows that reinforcement learning with hierarchical mental simulation on multiple layers is implemented in only one recent method\cite{Li2017_efficient_learning}.
% As a result, inter-dependencies between sub-tasks are hard to detect. 
A major reason for this shortcoming is that the low-level  policy should have already converged before the high-level forward model starts training. 
This problem has been addressed for model-free HRL \cite{Eysenbach2019_DiversityFunction}, but it has not yet been investigated with  predictive forward models. 
% \citet{Eysenbach2019_DiversityFunction} address this issue in a model-free architecture in two steps: first they pre-training low-level policies through an intrinsic reward function based on maximum entropy and once they have converged they use them to learn a high-level policy that composes the low-level policy. .  to pre-train domain-independent low-level policies first, and after convergence 
\end{sloppypar}

% This result is interesting because any approach with a forward model could straight-forwardly be extended to also consider planning\cite{Botvinick2014}.
% , and planning can be leveraged for few-shot problem-solving\cite{Sharma2020_DADS}. 
% Therefore, current model-based approaches do not exploit their full potential.

\begin{sloppypar}
\noindent \textbf{Intrinsic motivation requires forward models with elaborate uncertainty-handling.}
% In our survey, we distinguish between the three most frequently used kinds of intrinsic motivation: curiosity, diversity, and subgoal discovery. 
\revv{Our supplementary \autoref{tab:hrl_properties} show that curiosity and diversity are underrepresented intrinsic motivation methods: they are implemented in only 9 out of 50 surveyed papers, while our section \nameref{sec:cognitive_background} shows significant cognitive evidence that these mechanisms are critical for intelligent behaviour in biological agents\cite{Oudeyer2018_CompuCuriosityLearning}.}{R2-\ref{rev:r2:semantics:intrinsic_underrep}}

A potential reason for this shortcoming is that prediction-based intrinsic motivation suffers from an overly simplistic uncertainty handling of current computational forward models.
This is an issue for noisy observations or chaotic and unpredictable system dynamics. 
For example, \citet{Roeder2020_CHAC} achieve curiosity-driven intrinsic motivation by maximising the prediction error of a forward model. 
This causes the agent to suffer from the so-called \emph{noisy TV problem}, where an agent always strives to encounter unpredictable observations (such as a TV showing only white noise). 
\revv{This problem interferes with the problem of learning hierarchical representations because such a simple curiosity model is not appropriate for high-level representations that have not yet converged.}{R1-\ref{rev:r1:mech_spec_hrl}}
\end{sloppypar}

\noindent \textbf{Compositionality requires elaborate role-filler representations.}
Only a few HRL methods consider compositionality. 
Exceptions include natural language-based representations of actions \cite{Jiang2019_HRL_Language_Abstraction} or symbolic logic-based compositional representations \cite{Oh2017_Zero-shotTaskGeneralizationDeepRL}.
% However, none of these approaches ground these abstractions tightly in sensorimotor experiences. 
% However, as we describe in section \autoref{sec:cognitive_background}, compositionality has many benefits for transfer learning and decision-time planning. 
Since compositional representations generally build on variable-value representations, these need to be researched first on a more foundational level to alleviate this shortcoming. 

\revv{Graph Neural Networks, a class of neural networks that encode entities and their interactions as nodes and edges within a graph \cite{Battaglia:2018}, are a promising approach for compositional representations.
When provided with the underlying graph structure, Graph Neural Networks seem to generalise better and support relational reasoning \cite{Battaglia:2018}.
However, discovering a suitably abstracted graph from data remains an open challenge.}{R2-\ref{rev:r2:papers:battaglia}}

\noindent \textbf{Inference-fitted state abstraction requires a strong learning signal.}
\revv{
Recent HRL approaches \cite{Levy2019_Hierarchical,Roeder2020_CHAC} use the same state representation for each layer in the hierarchy. 
However, it seems cognitively more plausible to fit the level of abstraction to the level of inference needed on each hierarchical level.
For example, a high-level layer may only need to know whether or not an object is graspable, it does not need to consider its precise shape. This more detailed information, however, is relevant for the low-level layer that performs the grasping.
}{R1-\ref{rev:r1:mech_spec_hrl}}
There exist RL-methods that learn state abstractions from visual data with a convolutional autoencoder\cite{Ha2018_WorldModels}. 
%There exist RL-methods, where abstract (aka. latent) representations are generated from visual data with a convolutional autoencoder\cite{Ha2018_WorldModels}. 
However, such representations are optimised for reconstructing the visual input---not for decision-making. 
Furthermore, in the existing recent vision-based architectures\cite{Jiang2019_HRL_Language_Abstraction,Lample2018_PlayingFPSGames,Oh2017_Zero-shotTaskGeneralizationDeepRL,Sohn2018_Zero-ShotHRL,Vezhnevets2017_Feudal,Wulfmeier2020_HierachicalCompositionalPolicies,Yang2018_HierarchicalControl}, all hierarchical layers of the RL agent are provided with the same image embedding. %output of the ConvNet, i.e., with the same level of representational abstraction. 
Therefore, the abstractions are not inference-fitted. 
% There exist a few approaches that perform inference-fitted state abstraction\cite{Vezhnevets2017_Feudal}, and also some that involve compositional state representations\cite{Vezhnevets2020_OPRE}. 
% However, most of these build on hand-crafted abstraction functions that are not learned \cite{Eppe2019_planning_rl}.
A problem for learning inference-fitted abstraction functions is that the reward signal of reinforcement learning is a relatively weak driver for the learning process, compared to other methods like supervised learning. 
%Ideally, behavioral inferences should unfold selectively on the appropriate representational levels dependent on the current goals and motivations of the system.



% \subsection{Central challenges of integrated hierarchical architectures}
% \label{sec:results:challenges}
% We hypothesize that the above shortcomings are the result of several central challenges that occur when integrating the mechanisms depicted in \autoref{fig:cog_prereq} in a unifying hierarchical architecture.  


% % These involve advanced uncertainty models, computational implementations of bidirectional action-effect associations, and inference-fitted abstraction. 


% % \textbf{Uncertainty modelling}

% % \textbf{Bidirectional action-effect models}

% % \textbf{Inference-fitted abstraction}



% \noindent \textbf{Stabilize hierarchical representation learning.} 
% Hierarchical mental simulation demands stable high-level representations to learn a high-level forward model. 
% However, a general problem of hierarchical architectures is that a high-level layer can only learn meaningful behaviour after the lower-level layer has converged. 
% % A naive solution to address this issue is a threshold-based mechanism that detects the convergence of the lower-level to determine when the higher level layer may start training. 
% % This, however, does not consider continual and lifelong learning settings, where an agent's lower level behaviours and representations develop continuously. 
% % In hierarchical decision-making, this problem affects hierarchical mental simulation. 
% In the next subsection, we discuss how learning in hindsight\cite{Andrychowicz2017,Levy2019_Hierarchical} and bi-directional dynamics models\cite{Pathak2017_forward_model_intrinsic,Pathak2019_ICML_SelfSuperExploreDisa} may partially alleviate this problem.

% \noindent \textbf{Alleviate the model bias.}
% A forward model is never perfect, and multiple successive predictions lead to huge accumulated errors that render the predictions unusable. This problem is known as the model bias problem, and it demands for better uncertainty models to make the agent aware of the confidence of its predictions. 
% % Successful non-hierarchical approaches like PILCO \cite{Deisenroth2011} demonstrate the sample-efficiency of uncertainty-aware forward models based on Gaussian Process Models, but these models are only suitable for low-dimensional state and action representations. 
% Another dimension of this problem occurs with noisy observations or chaotic and unpredictable system dynamics, which is an issue for intrinsic motivation methods based on prediction. 
% For example, \citet{Roeder2020_CHAC} achieve curiosity-driven intrinsic motivation by maximizing the prediction error of a forward model. 
% This causes the agent to suffer from the so-called \emph{noisy TV problem}, where an agent always strives to encounter unpredictable observations (such as a TV showing only white noise), instead of searching for predictable situations that it just cannot predict yet. 

% In a hierarchical setting, this problem interferes with the problem of learning hierarchical representations, because high-level representations that are still being learned are hardly predictable at all. 


% \noindent \textbf{Improve variable-value assignment.}
% Abstract compositional representations build on rules to determine the semantics of the composed data structure. 
% These rules require, in one way or another, variable-value pairs, where the variable describes a general semantic property. 
% For example, the disentangled vector representations that occur in variational autoencoders (VAEs) are compositional data structures, where each slot of the vector is a variable that represents a certain object property (e.g. the angle of a visual object).
% In language, the variables are roles of syntactic constructions, and the values are the words that fill these roles. 
% A problem with VAEs is that they do not support dynamic semantic representations with varying variables because the structure of the latent representations fixed, and therefore, also  the set of variables is fixed. They also do not support variables that are assigned to other variables. 
% Variable-value assignment is a particular issue in hierarchical decision-making, where low-level sensorimotor data is abstracted to high-level compositional representations that are used for high-level decision-making. 

% % \citet{Kriete2013_SymbolProc} provide a neurologically plausible model of variable-value assignment where variables are areas in the prefrontal cortex that act like a pointer in computer science, pointing to other areas which represent values. 
% % This is somewhat akin to Transformer neural networks, where Query, Key and Value vectors are used for a self-attention-mechanisms. 



% \noindent \textbf{Strengthen the feedback signal.}
% Learning-based inference-fitted abstraction demands a strong feedback signal to learn the respective abstraction functions. 
% However, in reinforcement learning the reward signal is often relatively weak compared to a supervised loss signal, especially in sparse reward settings where handshaped continuous reward functions are not present.
% In hierarchical reinforcement learning, this problem is even more severe if the goal is to learn also abstraction functions for inference-fitted high-level state representations. 
% Hence, hierarchical reinforcement learning with inference-fitted abstraction demands a stronger feedback signal to stabilize the learning. 
% % In the subsection below, we propose a potential solution to address this problem, based on bi-directional dynamics models. 

\subsection{Outlook: Suggestions for addressing the challenges}
\label{sec:results:solutions}
In the following, we sketch how computational key methods may potentially help to address the above challenges. 
% The methods will not solve all problems related to hierarchical reinforcement learning, but we believe that they are important key mechanisms for future developments. 

\noindent \textbf{Retrospective analysis of experiences.}
% \noindent \textbf{Learning in hindsight.}
% Hierarchical reinforcement learning demands stable high-level representations. 
A central problem of HRL is that stable high-level representations can only emerge once the learning of the lower-level has converged \cite{Eysenbach2019_DiversityFunction}. 
We suggest that a retrospective analysis of experiences can alleviate this issue.
This has been demonstrated for training a policy by learning in hindsight\cite{Andrychowicz2017,Levy2019_Hierarchical}, where the achieved world state of a policy is retrospectively pretended to be the desired goal state. 
% Learning in hindsight\cite{Andrychowicz2017} has been proposed  to alleviate the sparse reward problem in goal-conditioned reinforcement learning. 
% The technique builds on learning from failures, in the sense that an agent gets rewarded even if it fails to achieve a reinforcement learning goal. 
% This is realized by pretending in hindsight that the achieved goal was the actual goal. 
% \citet{Levy2019_Hierarchical} extend the method to hierarchical architectures by also proposing hindsight actions. 
% In their hierarchical framework, high-level actions are subgoals to be achieved by the lower-level layer. 
% Hindsight high-level actions are retrospectively defined as the subgoals that were actually achieved by the low-level layer, regardless of what the original subgoal was. 
% In other words, by pretending in hindsight that the executed action (aka. subgoal) was the intended action, there is no need any more to wait until the low-level behaviour has converged. 
\revv{
We suggest that hindsight learning is a special case of a more general retrospective analysis of memorised experiences. 
For example, it is potentially possible to also learn hierarchical forward models in hindsight, without the high-level layer having to wait for a low-level layer to converge. %that a high-level layer has to wait for a low-level layer to converge.
We hypothesise that re-considering the outcome of past erroneous actions of a not yet fully trained low-level layer as desired outcome can stabilise the high-level representations. 
Such a technique may also help to alleviate the model bias.}{R1-\ref{rev:r1:mech_spec_hrl}}
% , but, of course, there are still many other open ends to address. 





\noindent \textbf{Meta- uncertainty models.}
Prediction errors play an important role in mental simulation and intrinsic motivation. 
In our section \nameref{sec:cognitive_background} we have discussed the free energy principle, which involves two seemingly contradicting mechanisms that build on predictive processing models. 
\revv{
On the one hand, there is active inference \cite{Schwartenbeck2019_CompUncertainExplo}, which seeks to minimise long-term surprise. This can be implemented by minimising a forward model's uncertainty or prediction error. On the other hand, there is active learning, which seeks to maximise information gain. This can be implemented by maximising uncertainty\cite{Haarnoja2018_SAC} or prediction errors \cite{Roeder2020_CHAC} through respective intrinsic reward functions.}{R2-\ref{rev:r2:realisation_terminology}}
\citet{Schwartenbeck2019_CompUncertainExplo} address this contradiction by building on \emph{expected uncertainty}\cite{Yu2005UncertaintyAttention} to unify both mechanisms. 
% Unexpected uncertainty can be understood as meta-uncertainty, i.e., the uncertainty about the uncertainty.
Expected as well as unexpected uncertainty then can be understood as a meta-uncertainty-analysis. 
We suppose that an intrinsic reward for high \emph{meta-}uncertainty may lead to exploratory behaviour, causing the exploration of high short-term but anticipated lower long-term meta-uncertainty. Furthermore, the gained certainty about the uncertainty of forward models can lead to improved predictive processes, which are aware of their own limits\cite{Baldwin:2021}. 

\noindent \textbf{Bi-directional dynamics models.}
\revv{
Bi-directional models involve both forward and backward inference, and we suppose that this combination is beneficial for representational abstraction in
hierarchical architectures.}{R1-\ref{rev:r1:mech_spec_hrl}} 
Our supposition is based on the work by \citet{Pathak2017_forward_model_intrinsic} and by \citet{Hafner2020_Dreamer}, who use a combined forward and inverse model to generate latent representations in a self-supervised manner. 
The bi-directional model operates on a latent space, generated by an abstraction function. 
\revv{
% Their methods learn simultaneously the abstraction function, the forward model and the inverse model. 
By simultaneously performing inverse and backward prediction in the latent space, the abstraction function gains two important features: First, the latent space is de-noised because only the predictable parts of the latent observation determine the forward and backward prediction. Second, the method is self-supervised and, therefore, provides a more stable feedback signal than the comparatively weak reward signal.}{R2-\ref{rev:r2:realisation_terminology}}
This alleviates the prediction error and strengthens the overall learning signal. 
}{E-\ref{rev:editor:review_perspective}}
% The stronger learning signal is also better suited to learn advanced abstraction functions that generate compositional representations, e.g. disentangled state vectors or symbolic compositional representations\cite{Lyu2019_SDRL,Eppe2019_planning_rl}. 
% \noindent \subsection{Challenges remaining}
% The above proposals for addressing the central challenges of hierarchical reinforcement learning are  not sufficient for developing artificial agents that are as smart as the crow of \autoref{fig:crow_probsolving}. 
% The biggest challenge remaining is the integration of the methods, towards a unifying computational framework.
% A problem is the cross-dependencies between the individual methods, as each added component increases the complexity of training and evaluation.
% For example, hindsight learning requires bi-directional abstraction functions to map abstract high-level representation back to the context-specific low-level representations. 
% This is necessary because otherwise the system cannot reward successful high-level hindsight actions with the information from the low-level state representation. Another open question is how to model meta-uncertainty in bidirectional models. 
% % These cross-dependencies are not only conceptually difficult, they also imply software-technological challenges. Each one of the proposed mechanisms comes with its ows variants and hyperparameters TBC...
% It is impossible to foresee all remaining challenges, but we hope that we did present here some useful guidelines for next steps, grounded in cognitive and computational evidence. We encourage attempts to elaborate these further to understand the remaining challenges better.




==> v2/revision.tex <==
\onecolumn

\thispagestyle{empty}%
\vskip-36pt%
{\raggedright\sffamily\bfseries\fontsize{20}{25}\selectfont Response to referees \\[10pt] \Large \newtitle  \par}%
\vskip10pt
{\raggedright\sffamily\fontsize{12}{16}\selectfont  \newauthor \par}
\vskip25pt%

% \section{Statement of revision}

\noindent \textbf{Dear Trenton Jerde, dear anonymous reviewers}\\[0pt]

\noindent In response to the initial submission of our article ``\newtitle'', you provided us with very positive and useful feedback. We highly appreciate that each individual review was very constructive and sophisticated. This led to very interesting and valuable new aspects that significantly improved our article further. In particular, we highly value your comments concerning the appreciation of the contentiousness of the described theories. 

\noindent In this statement of revision, we provide elaborate details about how we have addressed the editor's and reviewers' suggestions. To maximise the convenience for the reviewers, we have marked the relevant rewritten passages in the text in \revv{dark blue colour and we also placed a side note on the article's margin to indicate which of the suggestions is addressed by the revised passage.}{Side notes contain references to the addressed suggestions.}
In the side note, we refer to the suggestion with E (for editor) and R1, R2, R3 for the three reviewers, followed by the item number of the enumeration in the statement of revision below. For example, R3-\ref{rev:r3:controversial_theories:embodiment} refers to item \ref{rev:r3:controversial_theories:embodiment} raised by Reviewer 3.


\subsection{Editor's summary and recommendation}
\label{rev:editor}
The editor reported that our manuscript is very interesting and promising.
His main suggestions for further improvement are to re-submit the revised article as a perspective paper and to further appreciate the computational challenges that arise in the integration of the hierarchical mechanisms we propose. 
We summarise the editor's suggestions and our efforts to address them as follows:

\begin{enumerate}
    \item
    \label{rev:editor:review_perspective}
    \textit{Editor's suggestion:} The editor suggests clarifying whether this is a review or perspective paper. He recommends to ``rewrite the title, abstract and introduction to clarify the purpose and new contributions of the article. At the end of the introduction, [we] should give the readers a brief preview of what the upcoming sections will cover. ''
    
    \textit{Our response:} The reviewers appreciate that our manuscript has a strong focus on reviewing contemporary theories and methods. However, our initial submission also clearly implies propositions for future directions. These future directions refer to the integration of the different mechanisms that we propose. 
    Therefore, we appreciate the suggestion by the editor and re-submit this revision as a perspective article. Yet, we still maintain a strong focus on literature review. 
    As the probably most important part of this revision, we have modified and elaborated the results section and reshaped it towards a critical discussion and outlook. On the one hand, this gives our article more of a perspective character. 
    On the other hand, it provides a structure for addressing another major suggestion by the reviewers, namely the proper and critical appreciation of the difficulties that arise when integrating the different mechanisms we propose. 
    Furthermore, to clarify the contribution of the article early on, we rewrote the title and the relevant parts of the abstract and the introduction as the editor suggests.
    To highlight the new perspective character of this article further, we moved unnecessary parts of the review (e.g. \autoref{tab:hrl_properties}) into the supplementary section. 
    Finally, we shortened some of the lengthy lists of citation numbers throughout the text, reducing unnecessary comprehensiveness in favour of layout and readability.
    
    \item
    \textit{Editor's suggestion:} The editor suggests appreciating further the potential difficulties that arise when integrating all mechanisms and prerequisites in a joint HRL framework. He also suggests using the terminology more carefully. This suggestion is based on the following comments by the reviewers:
        \begin{enumerate}
        \item 
        \label{rev:editor:integrating_difficulties:terms}
        R2 states that the five take-home results stated in the last section depend on the interpretation of the technical terms we use. 
        
        \textit{Our response: } It is indeed a problem that the interdisciplinary terminology we build upon is ambiguous. 
        We take this as an opportunity to propose a clear unifying terminology for the mechanisms, abilities and theories that we discuss. 
        We summarise this terminology in a new glossary in the supplementary \autoref{box:appendix:glossary}, and we also make the definitions more clear throughout the overall text. 
        Herein, we also introduce better terms for the important key concepts, such as \emph{inference-fitted abstraction}, \emph{background planning} and \emph{decision-time planning.}.
        
        
        
        \item
        \label{rev:editor:difficulties:integration}
        R3 states that the individual ideas and theories are not as established as we imply, and the editor suggests being more careful with implying that we have conclusively addressed the challenges of integrating various existing tools with HRL. 
        
        \textit{Our response: } The editor correctly states that there exist many remaining challenges in the integration of the various methods that we summarise in our article. This has also been pointed out by Reviewer 3 (cf. R3-\ref{rev:rev3:appreciate_difficulties}).
        To address this issue, we have significantly elaborated the results section and transformed it into a critical discussion and outlook. 
        The result is a new and dedicated subsection \nameref{sec:results:challenges} that we used to focus more on these difficulties. 
        Furthermore, we sketch solutions to address these problems in the new subsection \nameref{sec:results:solutions}. 
        As the four probably most important potential challenges that occur when integrating our proposed mechanisms, we identified the following ones:
        
        \begin{enumerate}
            \item Stabilise the learning-based hierarchical abstraction.  
             (This point was raised by Reviewer 3, see  R3-\ref{rev:editor:difficulties:abstractions} below). 
            % 
            % The reviewer correctly states that learning abstract representations implies that a high-level reinforcement learning layer or a  forward model operates on changing representations, resulting in very unstable behaviour. We now appreciate this problem better in \autoref{sec:results}. We also very briefly point out that a partial solution to this problem may be hindsight learning. 
            \item Reduce prediction errors and the model bias. 
            % This is a general problem for model-based RL, but it has a unique dimension in hierarchical architectures because, as stated above, prediction errors of high-level forward models occur naturally when the high-level representations are not yet fully learned (converged). As a sketch for a partial potential solution, we propose hindsight learning, modelling meta-uncertainty and bi-directional dynamics models. 
            
            \item Model structured representations with explicit variable-value pairs. 
            % Our review of cognitive literature suggests that compositional representations are important for transfer learning in hierarchical RL. However, to achieve compositional representations one requires mechanisms that structure a knowledge representation that is composed of variables and values. 
            % This is still an open problem in Neural Networks, but disentangled representations or symbolic representations may help. 
            
            \item Strengthen the feedback signal. 
            
            
        \end{enumerate}
        We provide an overview of the shortcomings, underlying challenges and suggestions for improvements in the new \autoref{fig:challenges_shortcomings_solutions}.
        
        % \textit{Our response: } It is true that many of the cognitive theories we discuss are contentious. 
        
        \item 
        \label{rev:editor:difficulties:abstractions} R3 states that state and action abstractions have been around for a long time, and the editor suggests appreciating more the difficulties that arise with these abstractions. 
        
        \textit{Our response: } The reviewer is right in that abstractions are not new. Our point was specifically concerning inference-fitted state abstractions. We now clarify the term, and we argue that these are underrepresented in recent HRL papers (cf. also R2-\ref{rev:r2:semantics:comp_representations}), in the sense that only very few methods use it, as our supplementary overview \autoref{tab:hrl_properties} shows. 
        We also clarify what we mean by ``underrepresented'' in the new section \autoref{sec:results} (cf. also R2-\ref{rev:r2:semantics:intr_motivation}). 
        
        
        
        
        
    \end{enumerate}
    \item The editor recommends reconsidering the following form and layout issues: 
    \label{rev:editor:form}
        \begin{enumerate}
        \item 
        \label{rev:editor:form:shorten}
        The article can be a less comprehensive review and, therefore, be shortened. We should shorten the article to 4,000 - 5,000 words. 
        
        \textit{Our response: } We have now shortened the article to 4739 words (excluding figure captions, references, abstract, section headings, supplementary appendix). 
        We mainly achieved the shortening by focusing less on the unnecessary comprehensiveness of the review sections and by shifting parts of the review into the supplementary section. 
        
        \item 
        \label{rev:editor:form:language}
        We should re-check the use of non-technical language that is accessible to a wide range of readers. 
        
        \textit{Our response: } We use an accessible language targeted towards a broad scientific community. The only abbreviations we use are for reinforcement learning (RL) and hierarchical reinforcement learning (HRL), as these terms occur very often. To further improve comprehensibility, we have added the supplementary glossary in \autoref{box:appendix:glossary}.
        
        \item We should re-check figure resolution and labelling guidelines. 
        
        \textit{Our response: } We double-checked labelling and figure resolution. 
        
        \item We should re-check references, and in particular papers that are not ``accepted by a named publication''.
        
        \textit{Our response: } We avoid publications that have not been peer-reviewed. We made a few exceptions for highly cited and very relevant articles published on ArXiV.
        % \cite{Colas2020_LanguageGroundingRL,Heess2016_transferModulControl,Li2018_DeepRL_Overview,Oudeyer2018_CompuCuriosityLearning}. 
        
    \end{enumerate}
\end{enumerate}





\subsection{Reviewer 1}
\label{rev:r1}
The reviewer agrees with our view that an understanding of biological mechanisms is very important to develop novel computational methods for problem-solving. The reviewer states that there could be an important contribution with this article, but the reviewer had difficulties extracting useful information that are specific to the hierarchical aspects of RL. In the following, we summarise the reviewer's suggestions for improvement and describe how we address them: 

\begin{enumerate}
    \item 
    \label{rev:r1:mech_spec_hrl}
    The reviewer states that most of the mechanisms we summarise in the article are important for RL, but not specific to HRL. 
    As an example, the reviewer mentions that intrinsic motivation is often helpful in RL, but it is unclear how it is related to the hierarchical aspects of HRL. 
    
    \textit{Our response: } The reviewer is right in that several mechanisms are also relevant in non-hierarchical RL, and we may not have pointed out the relevance of hierarchical architectures clearly enough. 
    
    We now address this suggestion by detailing better how a particular mechanism is specific to HRL in the section \nameref{sec:hrlFinal}. 
    For example, we now state more clearly in the section \nameref{sec:hrlFinal} that curiosity is relevant to HRL because it can be used within a high-level layer to serve as a curriculum generator for a low-level layer.
    Furthermore, the new \nameref{sec:results} section also states for each challenge how it affects specifically hierarchical architectures. 
    
    \item The reviewer suggests that \autoref{tab:hrl_properties} and \autoref{fig:hrl} are not helpful. 
    \label{rev:r1:table_figure}
    
    \textit{Our response: } We agree that the detailed  \autoref{tab:hrl_properties} is maybe too detailed for this perspective article, and probably more appropriate for a comprehensive review in a narrower expert journal. 
    We discussed this also with the editor, and he agreed that it would be better to place the table in a supplementary appendix section. We followed this suggestion and the table is now part of the supplementary material.
    
    We also agree that  \autoref{fig:hrl} is trivial for expert readers like the reviewer who is familiar with hierarchical reinforcement learning and related topics. 
    However, \autoref{fig:hrl} requires only little space and contains an important overview to improve the comprehensibility and the overall framing for a broader audience. 
    Since comprehensibility for readers across multiple disciplines is very important to us, we would prefer to keep the figure if possible.
    
    % \item 
    % \label{rev:r1:hierarchical_aspects}
    % The reviewer suggests improving the links between the summarised mechanisms and hierarchical aspects or HRL. 
    % As one possible way of doing this, the reviewer suggests that elements of the results section may be moved to the beginning of the article to set up a motivating structure for how the mechanisms improve hierarchical RL. 
    
    % \textit{Our response: } As discussed already in our response to the editor's comments (cf.   \nameref{rev:editor},  \autoref{rev:editor:difficulties:integration}), we completely agree that the article would benefit from highlighting better the relation between \emph{hierarchical} RL and our proposed mechanisms.
    % We address this issue by highlighting better the relation between our proposed mechanisms and hierarchical architectures in \autoref{sec:hrl} and the new section \autoref{sec:results}.
    
    \item
    \label{rev:r1:example}
    The reviewer suggests to a) describe more clearly the main problems of HRL and b) explain how the mechanisms we summarise could solve them. 
    As one possible way of doing this, the reviewer suggests providing an example of a specific use case where one of our proposed mechanisms solves a previously described HRL problem.  

    \textit{Our response: } 
    The suggestion is a very important contribution, and we agree that a more intense discussion of the general underlying challenges behind HRL would help the article. This is also in-line with the editor's suggestions above.  
    Therefore, we now discuss the main problems of HRL in the new dedicated section \nameref{sec:results:challenges}. 
    We are also most thankful for the reviewer's suggestion to present an example. We address this suggestion by extending the caption of \autoref{fig:crow_probsolving}, which now explains how the individual mechanisms help to solve the problem-solving task performed by the crow. 
    
\end{enumerate}


\subsection{Reviewer 2}
The reviewer appreciates our integrative thinking at a large scale and provides us with very valuable and constructive suggestions for further improvements. Most importantly, the reviewer suggests improving clarity on what the technical terms mean semantically and algorithmically. For example, what is the difference between planning vs. mental simulation, and transfer learning vs. zero-shot problem-solving. 
In the following, we summarise the suggestions by Reviewer 2 and describe how we address them.

\begin{enumerate}
    \item 
    \label{rev:r2:realisation_terminology}
    The reviewer suggests providing more detail on algorithmic realisation and the terminology of the mechanisms that we summarise. For example, the reviewer requests more clarity about the difference between transfer learning and few-shot problem-solving, and about the difference between planning and mental simulation. 
    
    \textit{Our response: } We agree that terminology is an important issue, especially in this interdisciplinary article. We address this suggestion by providing an additional glossary in the supplementary \autoref{box:appendix:glossary}. 
    To address the suggestion concerning the algorithmic realisation, we added more details in the new section  \nameref{sec:results}. For example, we describe more clearly how curiosity could be implemented with meta-uncertainty models to unify active learning and active inference, and we provide more details on bi-directional models. 
    However, we also tried to avoid overly technical details because the journal is targeted at a broad audience. 
    
    \item Our review mainly considers goal-directed processes, and the reviewer suggests elaborating also on habit learning and how habit learning can take advantage of compositional abstraction.
    \label{rev:r2:habits}
    
    \textit{Our response: }  We agree that our description of habit learning was not phrased carefully enough. We rewrote most of the subsection on goal-directed planning and present our points in this subsection more clearly. We now describe the (traditionally considered) difference between planned behaviour and habits and elaborate on how they can be viewed as two ends of a spectrum. We also state how habits can form based on experience with a particular behaviour. 
    % Note by Manfred: From my naive understanding (without being too familiar with the term habit learning) I'd say that habit learning just means to re-use a previously learned low-level policy over and over again. Hence, representations related to a habit are useful if they are compositional, because then they can be transferred to more easily to other new policies and habits.
    
    \item The reviewer suggests elaborating also on immediate stimulus-response pairs that occur, e.g., when humans see a painting and immediately know whether they like it. 
    
    \textit{Our response: } This is definitely an interesting aspect, but we believe that aesthetic or moral judgement is beyond the scope of this shortened version of our article. 
    
    %The reviewer suggests to also consider and elaborate that habit learning can "take advantage of compositionality, analogy, state abstraction, and action abstraction", for example during moral or aesthetic judgement.
    % We agree that our claims on habit learning were not phrased carefully enough. We rewrote most of the subsection on goal-directed planning. Now we present our points in this subsection more in terms of theories. Additionally, we provide more points on how habits can form based on compositional structures and other representational concepts.
    
    \item 
    \label{rev:r2:terminology_results}
    Reviewer 2's most important suggestion is to clarify the semantics of the technical terms that we use. This is particularly important for our claims in the results section of the previous version of this article. In this revised version, the results section has been completely rewritten to pitch the article more towards a perspective paper, and this makes the terminology issue even more important. We address the specific suggestions of the reviewer as follows:
    
    \begin{enumerate}
        \item 
        \label{rev:r2:terminology_results:tautology}
        The reviewer identifies a tautology in our claim ``Most current few-shot problem-solving methods build on transfer learning, but they do not leverage planning''. This is tautologous given our following definition of transfer learning ``Transfer learning allows biological agents to perform few-shot problem-solving by transferring the solution to a previously solved task to novel, previously unseen tasks''
        
        \textit{Our response: } We clarify the terminology in the new glossary in the supplementary \autoref{box:appendix:glossary}, which should also help to communicate better what we mean by transfer learning and planning. Furthermore, in the new rewritten results section, we rephrased the tautologous sentence using our cleanly defined terminology.
    
        \item 
        \label{rev:r2:terminology_results:potential_compositionality}
        The reviewer suggests being more careful with the claim  "Current methods do not exploit the full potential of compositional abstract representations" because the full potential of compositional abstract representations cannot be evaluated. 
        
        \textit{Our response: } It is true that the full potential cannot be evaluated. We removed the sentence in the new section \nameref{sec:results}. 
        
        \item
        \label{rev:r2:semantics:comp_representations}
        The reviewer suggests that our claim ``State abstraction is significantly less researched than action abstraction'' is ``dubious'' when considering that computer vision essentially performs state abstraction. 
        
        \textit{Our response: } 
        This is a very important remark for us because it led us to introduce the concept of \emph{inference-fitted abstraction} in our section \nameref{sec:hrl:mechanisms}. We now also define this term in the new supplementary \autoref{box:appendix:glossary}. 
        
        ConvNets and similar methods for computer vision clearly perform a simple form of abstraction, and our formulations may not have been clear enough. A problem is that in the existing approaches we reviewed, ConvNets and similar methods for visual data use the same latent representations for all hierarchical layers. We claim that this is not ideal because, according to our rationale, the representation on which a hierarchical layer operates should be appropriate for the level of inference it performs. This demands for inference-fitted abstraction, where each level of abstraction is fitted to the particular level of inference. 
        
        \item 
        \label{rev:r2:semantics:intrinsic_underrep}
        The reviewer suggests clarifying the claim ``Curiosity and diversity, as intrinsic motivation methods, are underrepresented.'', in particular to clarify what ``underrepresented'' means. 
        
        \textit{Our response: }
        \label{rev:r2:semantics:intr_motivation}
        We now clarify this in the new section \nameref{sec:results}: By \emph{underrepresented} we mean that only eight out of the 50 approaches we enlist in our comprehensive survey in the supplementary \autoref{tab:hrl_properties} do not feature these types of intrinsic motivation, even though there exist many studies from the cognitive sciences that consider them to be very important. More computational implementations would help to validate the cognitive theories. 
        
        \item The reviewer suggests clarifying our claim ``there is a lack of hierarchical mental simulation methods'' and provides us with several relevant and important references to articles that are inspired by mental simulation. 
        
    \end{enumerate}
    
    \item 
    \label{rev:r2:shorten}
    The reviewer suggests shortening the paper further and phrasing arguments and definitions more compactly.
    
    \textit{Our response: } As suggested also by the editor (E-\ref{rev:editor:form:shorten}), we have re-submitted the article as a perspective paper and shortened it accordingly.
    
    \item The reviewer suggests improving how we discuss the Wolpert and Kawato 1998 paper and how it raises the reader's expectations in the following paragraphs and subsections.  
    \label{rev:r2:wolpert:kawato}
    
    \textit{Our response: } We now avoid this issue by referencing ideomotor theory instead. This also helps to reduce the length and references of our article.
    
    \item 
    \label{rev:r2:terminology}
    The reviewer suggests aligning our terminology ``planning'' and ``model-based RL'' with the terminology ``decision-time planning'' and ``background planning'' by Hamrick et al.
    
    \textit{Our response: } The terminology is indeed a problem, and we thank the reviewer very much for this suggestion. 
    We have addressed it with our glossary in the supplementary \autoref{box:appendix:glossary} and we introduce the different forms of planning now more clearly in section \nameref{sec:hrlFinal}, based on the very interesting and relevant article by Hamrick et al.
    
    \item 
    \label{rev:r2:terminology2}
    The reviewer suggests clarifying the following technical terms before they are used: 
    \begin{enumerate}
        \item state abstraction
        \item compositional representation
        \item transfer learning
        \item inductive bias
        \item event segmentation
        \item intrinsic motivation
        \item epistemic drive
        \item abductive search
    \end{enumerate}
    
    \textit{Our response: } We fully agree that the technical terms are sometimes ambiguous. 
    We have addressed this suggestion with a new supplementary glossary in \autoref{box:appendix:glossary} and we use the terms now more carefully and consistently throughout all sections in the text. We also now avoid using the terms ``abductive search'' and ``epistemic drive''. 
    
    \item The reviewer contributes the following additional suggestions:
    
    \begin{enumerate}
        \item Avoid the term ``higher level intelligent animal species''
        \label{rev:r2:sugg:int_animal}
        
        \textit{Our response: } We reduce this to ``intelligent animal species''. 
        
        \item References: Fix author list of reference 118
        
        \textit{Our response: } Thank you, we fixed the author list.
        
        \item 
        \label{rev:r2:sugg:ref_few_shot}
        Fix the reference [1] for few-shot problem-solving. 
        
        \textit{Our response: } This was a misunderstanding created by unfortunate formatting. The reference $^1$  was indeed pointing to a footnote and not to a reference to the paper [1]. We converted the footnote into an ordinary sentence in the paragraph. 
        
        \item Explain the notation [grasp(object), moveArm(goal), ...]
        
        \textit{Our response: } It is true that the notation is not clearly defined. Given that the reviewers also suggest shortening the article, we removed the example.
        
        \item The statement ``Cognitive theories consider analogical reasoning as a critical cornerstone'' is too strong.
        \label{rev:r2:sugg:analogical_reasoning}
        
        
        \textit{Our response: } We agree and softened the claim.
        
        
        \item 
        \label{rev:r2:sugg:trans_learn_para}
        Improve the last paragraph in the transfer learning section and fix the unfortunate wordings.
        
        \textit{Our response: } We are unsure whether the reviewer refers to the transfer learning section within the section \nameref{sec:hrlFinal} or within the section \nameref{sec:cognitive_background}. We changed the last sentence of the \nameref{sec:cognitive_background} section and removed the last sentence of the \nameref{sec:hrlFinal} section. 
        
        \item The word ``habituated'' was used when ``habitual'' was intended. %Distinguish better between ``habituated'' and ``habitual''. 
        \label{rev:r2:sugg:habitual}
        
        \textit{Our response: } Thank you for pointing this out. We corrected this mistake throughout the manuscript.
        
        \item Be more careful with the statement ``Habituation [sic] of behavior, which is comparable to model-free policy optimization in reinforcement learning, enables an agent to learn one particular skill in a controlled environment. However, complex problem solving in a new or  changing environment requires some form of prospective planning.''. Describe this and related statements not as definitely true but as the viewpoint of some particular theories. 
        \label{rev:r2:sugg:planningclaims}
        
        \textit{Our response: } We agree that the outlined claim and other statements in this section should not be presented as factual truths. We rewrote most of the section on goal-directed planning and removed the sentences in question. In our revised section we present our points more in terms of psychological theories or models instead of positive statements about learning in animals. 
        
        \item The reviewer suggests that ``It is now generally agreed upon... ''  on p.3 is too strong. 
        \label{rev:r2:sugg:agreement}
        
        
        \textit{Our response: } We agree and weakened the claim.
        
        \item Clarify the statement ``Hierarchical abstractions enable automatizing originally planned behaviour'' and relate it to the distinction between habitual and goal-directed behaviour. \label{rev:r2:sugg:automatization}
        
        \textit{Our response: } We clarified the statement and related it to the distinction of habitual and planned behaviour. See also our response in point R2-\ref{rev:r2:habits}.
        
        \item The reviewer suggests to re-think how the following example addresses state abstraction: ``For example, we can tell that a robot arm we have never seen before is grasping an object, even though the anatomy, the unfolding control algorithms, and the involved motor commands may largely vary from our human ones.'' 
        
        \textit{Our response: } We found that this example is not necessary. We followed the suggestion to further shorten the article and removed the example. 
        
        \item Fix the name David Hume
        \label{rev:r2:sugg:hume}
        
        \textit{Our response: } We removed the example mentioning David Hume in this shortened version of the article.
        
        
        \item Re-think how we argue about intrinsic motivation at the end of the intrinsic motivation section on p.4 to not make it sound like a there is intrinsic motivation for scientific hypothesis testing.
        \label{rev:r2:sugg:intrinsic_motivation}
        
        \textit{Our response: } We modified the sentences in question to avoid giving this impression.
        
        \item The definition of transfer learning on p.5 is partly redundant with earlier parts of the paper. 
        
        \textit{Our response: } The reviewer probably refers mainly to the distinction between near and far transfer, which was indeed redundant. While shortening the article, we removed this redundant part. % which is indeed redundant. We included this small overlap on purpose so that a reader who is only interested in one of the two review sections and skips the other one is still able to correctly understand it. 
        %We hope that this small amount of redundancy is appropriate for the journal.
        
    \end{enumerate}
    
    \item
    \label{rev:r2:papers}
    The reviewer suggests considering 13 additional articles. 
    
    \textit{Our response: } 
    We are very thankful for this comprehensive selection of relevant papers. They all provide an important contribution to our article.
    
    \begin{enumerate}
        \item
        \label{rev:r2:papers:thomas}
        Anthony Thomas, Zheng Tian, and David Barber. ``Thinking fast and slow with deep learning and tree search.'' arXiv preprint arXiv:1705.08439 (2017).
    
        $\rightarrow$ The article is indeed interesting as it elegantly exploits how an expert performing decision-time planning is used to train an apprentice's policy by means of imitation learning. However, the article does not present a hierarchical architecture, and we also purposefully avoided the topic of imitation learning because it is immediately linked to social interaction. The whole social dimension on few-shot problem-solving and intelligent behaviour is very important and interesting, but out of scope for this work. Furthermore, the guidelines for submissions have relatively tight constraints for the allowed number of references in this article. Therefore, we decided not to include this proposed paper in our work. 
        

        \item
        \label{rev:r2:papers:barreto}
        Barreto, Andre, et al. "Fast reinforcement learning with generalized policy updates." Proceedings of the National Academy of Sciences 117.48 (2020): 30079-30087.
        
        $\rightarrow$ Barreto et al. generalise policy evaluation and improvement to multiple tasks and policies to achieve transfer learning. Once several policies are learned, a change in the task (here modelled as a change in the reward structure of the task) can be adapted faster than using q-learning from scratch. The authors further propose two ways to learn the reward structure of the task (here, vector of preferences) which effectively implements hierarchical RL. Therefore, we included the approach in Table 1.

        \item 
        \label{rev:r2:papers:battaglia}
        Battaglia, Peter W., et al. "Relational inductive biases, deep learning, and graph networks." arXiv preprint arXiv:1806.01261 (2018).
        
        $\rightarrow$ In their article, Battaglia et al.  provide an excellent review and overview of Graph Neural Networks (GNN). We agree that GNNs are a very promising approach, especially for learning compositional structures, which our article identifies as a key challenge for hierarchical reinforcement learning. We thank the reviewer for this suggestion and included the proposed paper in our outlook section \ref{sec:results:challenges}.

        \item Cobbe, Karl, et al. "Quantifying generalization in reinforcement learning." International Conference on Machine Learning. PMLR, 2019.
        
        $\rightarrow$ Cobbe et al. investigate RL generalisation using supervised learning methods (L2 regularisation dropout, data augmentation and batch normalisation). Extensive studies on zero-shot generalisation to new levels in a platform game are presented; this is a typical case of transfer learning. PPO is used as an RL algorithm with a three-Layer CNN architecture and the IMPALA architecture with three residual blocks. The authors show that all generalisation methods outperform the baseline and perform even better when combined. The paper is a valuable contribution to our position paper, as it shows the importance and value of established methods from supervised learning to solve transfer learning in RT.


        \item Haidt, Jonathan. "The emotional dog and its rational tail: a social intuitionist approach to moral judgment." Psychological review 108.4 (2001): 814.
        
        $\rightarrow$ This article outlines an interesting model for moral judgement. However, in the light of the requests to shorten our article, we believe the topic of moral judgement is beyond the scope of this work. Thus, we decided not to include this paper in our manuscript.  

        \item
        \label{rev:r2:papers:hamrick}
        Hamrick, Jessica B. ``Analogues of mental simulation and imagination in deep learning.'' Current Opinion in Behavioral Sciences 29 (2019): 8-16.
        
        $\rightarrow$ The article provides an excellent analysis of model-based RL, and we now build on it to underpin our the distinction between decision-time planning and background planning. 

        \item Jaderberg, Max, et al. "Human-level performance in 3D multiplayer games with population-based reinforcement learning." Science 364.6443 (2019): 859-865.
        
        $\rightarrow$ Jaderberg et al. suggest an end-to-end approach for a complex multiplayer 3d game environment and reach super-human performance, even after compensating for the artificial agent’s faster reaction time. The approach is based on a population of diverse agents that learn by playing against each other. Each agent is based on a multiple-timescale recurrent neural network and thus realised a hierarchical structure. During training, these agents use a dense internal reward function. While this intrinsic reward drives each agent’s RL training (called inner optimisation), the population of agents is optimised with population-based training, a genetic/evolution algorithm (outer optimisation). Furthermore, the authors show that the agents develop a rich internal representation of the game state: an analysis of embeddings shows clusters and even single neurons representing relevant game states. Though this is a posthoc analysis and not used during learning or evaluation, we report this as a state abstraction in Table 1.

        \item Schaul, Tom, et al. "Universal value function approximators." International conference on machine learning. PMLR, 2015.
        
        $\rightarrow$ The article presents Universal Value Function Approximators (UVFAs), which is indeed very important for goal-conditioned RL and for the hindsight learning we discuss in \autoref{sec:results:solutions}. However, since the articles we cite for hindsight learning already imply UVFAs, we do not see the need here to cite it explicitly. 

        \item Silver, David, et al. "Mastering the game of Go with deep neural networks and tree search." nature 529.7587 (2016): 484-489.
        
        $\rightarrow$ At the core of the approach of Silver et al. for reaching super-human performance in the complex game of Go is a Monte Carlo tree search (MCTS) that is augmented with policy networks and value networks. While this search (or planning) method has been applied to less complex games in the past, the large state space of Go made the problem intractable. The approach uses the value function to avoid expanding the tree to its full depth and the policy function to choose actions, thus reducing search breadth. Both functions are trained over several stages, starting from behavioural cloning for policy networks from human experts over RL optimisation and training of the value function in self-play.  
The approach can be seen as hierarchical, with the policy and value function working on a local level and the MCTS on the high level. However, unlike most hierarchical approaches, where the high control level delegates subtasks to the lower levels, it is actually the low-level functions that help to steer the MCTS and thus reduce the search space.



        \item Silver, David, et al. "Mastering the game of go without human knowledge." nature 550.7676 (2017): 354-359.
        
        $\rightarrow$ The article is relevant but it covers a similar topic as the 2016 article by Silver et al. For brevity, we consider only the more foundational 2016 article. 

        \item Silver, David, et al. "A general reinforcement learning algorithm that masters chess, shogi, and Go through self-play." Science 362.6419 (2018): 1140-1144.
        
        $\rightarrow$ For brevity, we consider only the 2016 article by Silver et al. 

        \item Schrittwieser, Julian, et al. "Mastering atari, go, chess and shogi by planning with a learned model." Nature 588.7839 (2020): 604-609.
        
        $\rightarrow$ This article also builds on the work by Silver et al. to which we already refer.

        \item Sutton, Richard S., et al. "Horde: A scalable real-time architecture for learning knowledge from unsupervised sensorimotor interaction." The 10th International Conference on Autonomous Agents and Multiagent Systems-Volume 2. 2011.
        
        $\rightarrow$ The approach proposed in the paper to learn a set of General Value Functions or demons, which can be divided into two types, control demons and prediction demons, can be seen as using low-level forward and inverse models and mental simulation. The authors indicate that transfer learning is possible.
Though not explicitly a hierarchical approach, we include the paper as it shows the relevance of independent and diverse low-level control and prediction. Thank you very much for the suggestion.

        
    \end{enumerate}
    
    
    
\end{enumerate}

\subsection{Reviewer 3}
\label{rev:r3}
The reviewer has thoroughly assessed our article and considers it an ``excellent review''. However, the reviewer provides three major, highly constructive suggestions to further improve our article. These are that a) the early sections of the article should clarify better the contribution of the review, b) some claims in cognitive sciences are controversial and should not be considered as settled, and c) the true difficulty of HRL should be acknowledged better. 
In the following, we will summarise the reviewer's suggestions in detail and describe our efforts to address them. 

\begin{enumerate}

    \item
    \label{rev:r3:clarify_contrib}
    The reviewer suggests that we should clarify better the first sections of the paper to not provide the reader with the sense that our contribution is to propose the integration of existing methods.
    
    \textit{Our response: }
    It is indeed overly straight-forward and simplistic to just propose the integration of the methods. Therefore, we state now more clearly in the abstract, introduction and conclusion that our contribution lies beyond the straight-forward proposal of integrating the methods. Therefore, we present a scientific rationale consisting of three steps: We first identify cognitively plausible abilities and mechanisms in a neurocognitive survey. Second, we map this survey to computational implementations, and we identify shortcomings in the state-of-the-art by performing a comprehensive review. 
    In this revised version, we now provide a strong additional third contribution with the new section \nameref{sec:results}. Here, we identify the challenges behind the shortcomings of the existing methods, and we provide a concluding outlook towards potential solutions.
    
    \item 
    \label{rev:rev3:appreciate_difficulties}
    The reviewer suggests that we should better describe the difficulties that would arise when integrating the summarised mechanisms into a unifying HRL system. 
    For example, the reviewer mentions the ``moving target'' problem that occurs when high-level predictions are learned while the representations on which they are based have not yet converged. 
    
    \textit{Our response: } The reviewer correctly states that learning abstract representations implies that a high-level reinforcement learning layer or a  forward model operates on changing representations, resulting in very unstable behaviour. We now appreciate this and other problems better in the dedicated new subsection \autoref{sec:results:challenges}. 
    Since the editor suggested submitting our manuscript as a perspective paper, we also sketch potential partial solutions to these problems. 
    
    \item 
    \label{rev:r3:structure_not_impression_first_integration}
    The reviewer suggests using the integration of the summarised mechanisms an organising structure for the review that could be laid out in the introduction. Herein, we should ``avoid giving the impression that this reflects the first time that researchers have considered integrating these mechanisms in an HRL agent.''
    
    \textit{Our response: } We are very aware that researchers have considered integrating these mechanisms before. However, no unifying integrative computational framework exists yet because there exist difficult challenges that need to be addressed. There is a lack of a systematic analysis of these challenges, and our article addresses this lack. 
    The reviewer's valuable suggestion inspired us to use the shortcomings and challenges behind HRL as an organising structure for the new section \nameref{sec:results}. 
    With this new section, the revised version of the article now features the following systematic rationale: 
    1) We provide a dedicated review to identify the core cognitive mechanisms behind hierarchical decision-making. 
    2) we provide a comprehensive review of contemporary HRL methods, which has not been done in recent years, as we discuss with our meta-survey in the supplementary section in \autoref{box:appendix:meta_RL-survey}. 
    Based on the review, we identify shortcomings of the existing methods and link them to the cognitive survey. 
    3) We identify challenges behind the shortcomings, and we propose potential solutions to address the challenges. 
    
    \item The reviewer appreciates the detailed insights we draw from animal cognition, but suggests being less bold when summarising the theoretical claims found in literature on biological and cognitive backgrounds. Our article would improve further if we acknowledge more clearly that these claims are subject to ongoing controversial discussions. 
    \label{rev:r3:bold_claims}
    
    \textit{Our response: } We agree that there is rarely consensus concerning cognitive science accounts, and we appreciate that the reviewer pointed out some controversial points (also listed below) that at first were not presented as such. In our revised manuscript, we now avoid presenting claims about cognition as factual and instead phrase them in terms of theories or models. Additionally, for particular contentious theories, such as the language of thought and the free energy principle, we point to important reference articles that discuss their controversial aspects.
    
    \item 
    \label{rev:r3:circular_inspiration}
    The reviewer suggests that we should be aware of circular reasoning that arises when AI inspires Cognitive Sciences, or when principles and theories from AI are used to model and to make sense of biological processes. Therefore, care should be taken when using cognitive sciences to guide reinforcement learning. 
    
    \textit{Our response: } As the reviewer says, research in AI and CogSci is often interleaved and interdisciplinary. Therefore, circular inference processes are very natural and cannot be avoided completely.
    This makes it sometimes hard to tell whether a particular CogSci theory has been directly or indirectly guided by a mathematical computational theory or vice versa.
    However, in our humble opinion, the influence between AI and CogSci is rather spiralling than circular, such that the spiral's centre is a fixed point where both views converge. 
    % We suggest that our discussed mechanisms are agnostic to the underlying biological or computational hardware. 
    This rationale is also commonly built upon in computational cognitive modelling research. It implies that if our discussed mechanisms have computational advantages they are likely to have also biological cognitive benefits, and vice versa. 
    However, we completely agree with the reviewer that this point should be more explicit. To address the reviewer's suggestion, we now clarify this further in a new dedicated paragraph of the \nameref{sec:conclusion} section.
    
    
    
    \item
    \label{rev:r3:controversial_theories}
    The reviewer reminds us that many of our reviewed cognitive theories are contentious, and suggests appreciating this better. The reviewer gives the following examples of principles, mechanisms and theories that are more controversial than our article implies: 
    
    \begin{enumerate}
        \item Planning.
        \label{rev:r3:controversial_theories:planning}

        \textit{Response: }Indeed, there exists a non-negligible amount of literature that questions whether planning (at least in the way we describe it) is a critical cognitive mechanism. We rewrote most of the section on goal-directed planning and now present our view on goal-directed planning as the combination of different theories and models that were developed over the last century. Thereby, we avoid presenting statements as factual truths. We believe that in our revised manuscript, it is now much clearer that our perspective on planning is just one particular perspective out of many. In addition, we underpin our perspective by the comprehensive article by Hamrick et al., as  suggested by Reviewer 2 in item R2-\ref{rev:r2:terminology}.
        
        \item Embodiment. 
        \label{rev:r3:controversial_theories:embodiment}
        
        \textit{Response: } We agree, and removed statements that present the theory of embodiment as accepted consensus. 
        % Response: We addressed this issue by first clarifying our used terminology better (see x-th par. in Sec. y.). Then we align this terminology with theories that are in favour of and against embodiment.  TODO... 
        
        \item 
        \label{rev:r3:controversial_theories:LoT}
        Language of Thought. 
        
        \textit{Response: } Indeed, language of thought has many contentious aspects, and appreciating this point better will definitely improve our article further. We thank the reviewer also for pointing us to the special issue by Gayler \& Levy. 
        To address this issue, we have rephrased the respective paragraph, and added that the biggest criticism lies in the question about whether knowledge is represented sententially (symbolic) or through neural connections.  
        We then point out that for the cognitive and mechanistic rationale of our perspective article, it is not necessary to go deeper into the connectionist/symbolicist debate. Instead, we immediately connect to neuroscientific connectionist evidence for compositional representations to appreciate both the symbolicist's and the connectionist's view. 
        
    \end{enumerate}
    
    In addition to these examples, we also discuss other mechanisms and theories now more controversially  (see side notes in the article). 
    For example, we acknowledge that discovering analogies is challenging for humans and refer to the functional fixedness phenomenon showcased with Duncker's candle experiment.
    
    
    
    % \item 
    % \label{rev:r3:difficulties}
    % The reviewer suggests appreciating better the true difficulty of the integration that we propose. For example, a problem with learning hierarchical abstractions is that they change over time, so that higher-level decision-making operates on changing representations. The reviewer also points us to difficulties when learning compositional representations with inductive biases. 
    
    % \textit{Response:} The reviewer is right that there are many difficulties in the integration. We address them now properly in the new dedicated section \nameref{sec:results:challenges}. 
    
    \item The reviewer suggests considering also Soar and Soar-RL in the discussion. 
    \label{rev:r3:soar}
    
    \textit{Response:} The Soar architecture is indeed interesting, in particular because of the elaborate memory modelling. This is an important issue, but out of scope for this paper. The Soar-RL extension is relatively old compared to the other papers that we investigate. The submission guidelines admit only a limited number of references, and we would prefer to discuss other more recent articles instead. 
    
\end{enumerate}


